A Comprehensive Survey on Machine Learning Techniques and User Authentication Approaches for Credit Card Fraud Detection

With the increase of credit card usage, the volume of credit card misuse also has significantly increased. As a result, financial organizations are working hard on developing and deploying credit card fraud detection methods, in order to adapt to ever-evolving, increasingly sophisticated defrauding strategies and identifying illicit transactions as quickly as possible to protect themselves and their customers. Compounding on the complex nature of such adverse strategies, credit card fraudulent activities are rare events compared to the number of legitimate transactions. Hence, the challenge to develop fraud detection that are accurate and efficient is substantially intensified and, as a consequence, credit card fraud detection has lately become a very active area of research. In this work, we provide a survey of current techniques most relevant to the problem of credit card fraud detection. We carry out our survey in two main parts. In the first part,we focus on studies utilizing classical machine learning models, which mostly employ traditional transnational features to make fraud predictions. These models typically rely on some static physical characteristics, such as what the user knows (knowledge-based method), or what he/she has access to (object-based method). In the second part of our survey, we review more advanced techniques of user authentication, which use behavioral biometrics to identify an individual based on his/her unique behavior while he/she is interacting with his/her electronic devices. These approaches rely on how people behave (instead of what they do), which cannot be easily forged. By providing an overview of current approaches and the results reported in the literature, this survey aims to drive the future research agenda for the community in order to develop more accurate, reliable and scalable models of credit card fraud detection.

==> LitReview-RBC <==
SyncTeX Version:1
Input:1:C:\Users\ni484792\Desktop\RBC\RBC-Niloo-Litreview\Online-To-Batch.tex
Input:2:C:\Program Files\MiKTeX 2.9\tex\latex\base\article.cls
Input:3:C:\Program Files\MiKTeX 2.9\tex\latex\base\size11.clo
Input:4:C:\Program Files\MiKTeX 2.9\tex\latex\url\url.sty
Input:5:C:\Users\ni484792\Desktop\RBC\RBC-Niloo-Litreview\sty\jmlr2e.sty
Input:6:C:\Program Files\MiKTeX 2.9\tex\latex\graphics\epsfig.sty
Input:7:C:\Program Files\MiKTeX 2.9\tex\latex\graphics\graphicx.sty
Input:8:C:\Program Files\MiKTeX 2.9\tex\latex\graphics\keyval.sty
Input:9:C:\Program Files\MiKTeX 2.9\tex\latex\graphics\graphics.sty
Input:10:C:\Program Files\MiKTeX 2.9\tex\latex\graphics\trig.sty
Input:11:C:\Program Files\MiKTeX 2.9\tex\latex\graphics-cfg\graphics.cfg
Input:12:C:\Program Files\MiKTeX 2.9\tex\latex\graphics-def\pdftex.def
Input:13:C:\Program Files\MiKTeX 2.9\tex\latex\amsfonts\amssymb.sty
Input:14:C:\Program Files\MiKTeX 2.9\tex\latex\amsfonts\amsfonts.sty
Input:15:C:\Program Files\MiKTeX 2.9\tex\latex\natbib\natbib.sty
Input:16:C:\Program Files\MiKTeX 2.9\tex\latex\hyperref\hyperref.sty
Input:17:C:\Program Files\MiKTeX 2.9\tex\generic\oberdiek\hobsub-hyperref.sty
Input:18:C:\Program Files\MiKTeX 2.9\tex\generic\oberdiek\hobsub-generic.sty
Input:19:C:\Program Files\MiKTeX 2.9\tex\generic\ifxetex\ifxetex.sty
Input:20:C:\Program Files\MiKTeX 2.9\tex\latex\oberdiek\auxhook.sty
Input:21:C:\Program Files\MiKTeX 2.9\tex\latex\oberdiek\kvoptions.sty
Input:22:C:\Program Files\MiKTeX 2.9\tex\latex\hyperref\pd1enc.def
Input:23:C:\Program Files\MiKTeX 2.9\tex\latex\00miktex\hyperref.cfg
Input:24:C:\Program Files\MiKTeX 2.9\tex\latex\hyperref\hpdftex.def
Input:25:C:\Program Files\MiKTeX 2.9\tex\latex\oberdiek\rerunfilecheck.sty
Input:26:C:\Program Files\MiKTeX 2.9\tex\latex\enumitem\enumitem.sty
Input:27:C:\Program Files\MiKTeX 2.9\tex\latex\psnfss\times.sty
Input:28:C:\Program Files\MiKTeX 2.9\tex\latex\mathtools\mathtools.sty
Input:29:C:\Program Files\MiKTeX 2.9\tex\latex\tools\calc.sty
Input:30:C:\Program Files\MiKTeX 2.9\tex\latex\mathtools\mhsetup.sty
Input:31:C:\Program Files\MiKTeX 2.9\tex\latex\amsmath\amsmath.sty
Input:32:C:\Program Files\MiKTeX 2.9\tex\latex\amsmath\amstext.sty
Input:33:C:\Program Files\MiKTeX 2.9\tex\latex\amsmath\amsgen.sty
Input:34:C:\Program Files\MiKTeX 2.9\tex\latex\amsmath\amsbsy.sty
Input:35:C:\Program Files\MiKTeX 2.9\tex\latex\amsmath\amsopn.sty
Input:36:C:\Program Files\MiKTeX 2.9\tex\latex\graphics\color.sty
Input:37:C:\Program Files\MiKTeX 2.9\tex\latex\graphics-cfg\color.cfg
Input:38:C:\Users\ni484792\Desktop\RBC\RBC-Niloo-Litreview\sty\options.sty
Input:39:C:\Users\ni484792\Desktop\RBC\RBC-Niloo-Litreview\sty\packages.sty
Input:40:C:\Program Files\MiKTeX 2.9\tex\latex\acronym\acronym.sty
Input:41:C:\Program Files\MiKTeX 2.9\tex\latex\bigfoot\suffix.sty
Input:42:C:\Program Files\MiKTeX 2.9\tex\latex\xstring\xstring.sty
Input:43:C:\Program Files\MiKTeX 2.9\tex\generic\xstring\xstring.tex
Input:44:C:\Users\ni484792\Desktop\RBC\RBC-Niloo-Litreview\sty\macros.sty
Input:45:C:\Program Files\MiKTeX 2.9\tex\latex\microtype\microtype.sty
Input:46:C:\Program Files\MiKTeX 2.9\tex\latex\microtype\microtype-pdftex.def
Input:47:C:\Program Files\MiKTeX 2.9\tex\latex\microtype\microtype.cfg
Input:48:C:\Program Files\MiKTeX 2.9\tex\latex\l3packages\xparse\xparse.sty
Input:49:C:\Program Files\MiKTeX 2.9\tex\latex\l3kernel\expl3.sty
Input:50:C:\Program Files\MiKTeX 2.9\tex\latex\l3kernel\expl3-code.tex
Input:51:C:\Program Files\MiKTeX 2.9\tex\latex\l3kernel\l3pdfmode.def
Input:52:C:\Program Files\MiKTeX 2.9\tex\latex\tcolorbox\tcolorbox.sty
Input:53:C:\Program Files\MiKTeX 2.9\tex\latex\pgf\basiclayer\pgf.sty
Input:54:C:\Program Files\MiKTeX 2.9\tex\latex\pgf\utilities\pgfrcs.sty
Input:55:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\utilities\pgfutil-common.tex
Input:56:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\utilities\pgfutil-common-lists.tex
Input:57:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\utilities\pgfutil-latex.def
Input:58:C:\Program Files\MiKTeX 2.9\tex\latex\ms\everyshi.sty
Input:59:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\utilities\pgfrcs.code.tex
Input:60:C:\Program Files\MiKTeX 2.9\tex\latex\pgf\basiclayer\pgfcore.sty
Input:61:C:\Program Files\MiKTeX 2.9\tex\latex\pgf\systemlayer\pgfsys.sty
Input:62:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\systemlayer\pgfsys.code.tex
Input:63:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\utilities\pgfkeys.code.tex
Input:64:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\utilities\pgfkeysfiltered.code.tex
Input:65:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\systemlayer\pgf.cfg
Input:66:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\systemlayer\pgfsys-pdftex.def
Input:67:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\systemlayer\pgfsys-common-pdf.def
Input:68:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\systemlayer\pgfsyssoftpath.code.tex
Input:69:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\systemlayer\pgfsysprotocol.code.tex
Input:70:C:\Program Files\MiKTeX 2.9\tex\latex\xcolor\xcolor.sty
Input:71:C:\Program Files\MiKTeX 2.9\tex\latex\graphics-cfg\color.cfg
Input:72:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcore.code.tex
Input:73:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmath.code.tex
Input:74:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathcalc.code.tex
Input:75:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathutil.code.tex
Input:76:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathparser.code.tex
Input:77:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfunctions.code.tex
Input:78:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfunctions.basic.code.tex
Input:79:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfunctions.trigonometric.code.tex
Input:80:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfunctions.random.code.tex
Input:81:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfunctions.comparison.code.tex
Input:82:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfunctions.base.code.tex
Input:83:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfunctions.round.code.tex
Input:84:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfunctions.misc.code.tex
Input:85:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfunctions.integerarithmetics.code.tex
Input:86:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\math\pgfmathfloat.code.tex
Input:87:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcorepoints.code.tex
Input:88:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcorepathconstruct.code.tex
Input:89:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcorepathusage.code.tex
Input:90:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcorescopes.code.tex
Input:91:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcoregraphicstate.code.tex
Input:92:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcoretransformations.code.tex
Input:93:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcorequick.code.tex
Input:94:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcoreobjects.code.tex
Input:95:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcorepathprocessing.code.tex
Input:96:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcorearrows.code.tex
Input:97:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcoreshade.code.tex
Input:98:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcoreimage.code.tex
Input:99:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcoreexternal.code.tex
Input:100:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcorelayers.code.tex
Input:101:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcoretransparency.code.tex
Input:102:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\basiclayer\pgfcorepatterns.code.tex
Input:103:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\modules\pgfmoduleshapes.code.tex
Input:104:C:\Program Files\MiKTeX 2.9\tex\generic\pgf\modules\pgfmoduleplot.code.tex
Input:105:C:\Program Files\MiKTeX 2.9\tex\latex\pgf\compatibility\pgfcomp-version-0-65.sty
Input:106:C:\Program Files\MiKTeX 2.9\tex\latex\pgf\compatibility\pgfcomp-version-1-18.sty
Input:107:C:\Program Files\MiKTeX 2.9\tex\latex\tools\verbatim.sty
Input:108:C:\Program Files\MiKTeX 2.9\tex\latex\environ\environ.sty
Input:109:C:\Program Files\MiKTeX 2.9\tex\latex\trimspaces\trimspaces.sty
Input:110:C:\Program Files\MiKTeX 2.9\tex\latex\etoolbox\etoolbox.sty
Input:111:C:\Users\ni484792\Desktop\RBC\RBC-Niloo-Litreview\Online-To-Batch.aux
Input:112:C:\Program Files\MiKTeX 2.9\tex\latex\psnfss\ot1ptm.fd
Input:113:C:\Program Files\MiKTeX 2.9\tex\context\base\supp-pdf.mkii
Input:114:C:\Program Files\MiKTeX 2.9\tex\latex\oberdiek\epstopdf-base.sty
Input:115:C:\Program Files\MiKTeX 2.9\tex\latex\oberdiek\grfext.sty
Input:116:C:\Program Files\MiKTeX 2.9\tex\latex\hyperref\nameref.sty
Input:117:C:\Program Files\MiKTeX 2.9\tex\generic\oberdiek\gettitlestring.sty
Input:118:C:\Users\ni484792\Desktop\RBC\RBC-Niloo-Litreview\Online-To-Batch.out
Input:119:C:\Users\ni484792\Desktop\RBC\RBC-Niloo-Litreview\Online-To-Batch.out
Input:120:C:\Program Files\MiKTeX 2.9\tex\latex\microtype\mt-ptm.cfg
Input:121:C:\Program Files\MiKTeX 2.9\tex\latex\psnfss\omsptm.fd
Input:122:C:\Program Files\MiKTeX 2.9\tex\latex\psnfss\ot1pcr.fd
Input:123:C:\Program Files\MiKTeX 2.9\tex\latex\microtype\mt-cmr.cfg
Input:124:C:\Program Files\MiKTeX 2.9\tex\latex\amsfonts\umsa.fd
Input:125:C:\Program Files\MiKTeX 2.9\tex\latex\microtype\mt-msa.cfg
Input:126:C:\Program Files\MiKTeX 2.9\tex\latex\amsfonts\umsb.fd
Input:127:C:\Program Files\MiKTeX 2.9\tex\latex\microtype\mt-msb.cfg
Output:pdf
Magnification:1000
Unit:1
X Offset:0
Y Offset:0
Content:
!9741
{1
[1,117:4736286,48201563:29601791,43465277,1655174
h1,117:4736286,4736286:0,0,0
[1,117:4736286,4736286:0,0,0
(1,117:4736286,2302362:0,0,0
k1,117:4736286,2302362:-1118290
)
]
[1,117:4736286,48201563:29601791,43465277,1655174
h1,117:4736286,4736286:0,0,0
[1,117:5920357,48201563:28417720,45833420,1655174
[1,117:5920357,3154575:28417720,786432,0
(1,117:5920357,3154575:28417720,357558,113504
(1,117:5920357,3154575:28417720,357558,113504
x1,117:7463846,3154575
g1,117:7594918,3154575
x1,117:8031648,3154575
g1,117:8162720,3154575
x1,117:9997185,3154575
g1,117:10128257,3154575
x1,117:12020923,3154575
g1,117:12151995,3154575
x1,117:14073488,3154575
g1,117:14204560,3154575
x1,117:14728848,3154575
g1,117:14859920,3154575
x1,117:16257668,3154575
g1,117:16388740,3154575
x1,117:17349758,3154575
g1,117:17480830,3154575
k1,117:24694416,3154575:7213586
x1,117:26850262,3154575
g1,117:26981334,3154575
x1,117:28059260,3154575
g1,117:28190332,3154575
x1,117:28772809,3154575
x1,117:29866461,3154575
g1,117:29997533,3154575
x1,117:31075459,3154575
g1,117:31206531,3154575
x1,117:33274826,3154575
g1,117:33405898,3154575
x1,117:34338077,3154575
)
)
]
[1,117:5920357,46235483:28417720,40258437,0
(1,69:5920357,6697942:28417720,541848,11006
k1,69:18666076,6697942:12745719
x1,69:21592358,6697942
k1,69:34338077,6697942:12745719
)
(1,73:5920357,7827265:28417720,440723,133360
g1,73:7231077,7827265
x1,73:7740940,7827265
k1,72:7231077,7827265:-16384
x1,72:8816380,7827265
x1,72:10266019,7827265
g1,72:10469179,7827265
k1,73:33027357,7827265:22558178
g1,73:34338077,7827265
)
(1,77:5920357,9899559:28417720,541848,11006
(1,77:5920357,9899559:668472,541848,11006
g1,77:5920357,9899559
x1,77:6510181,9899559
g1,77:6588829,9899559
)
g1,77:6785437,9899559
x1,77:8139652,9899559
x1,77:11053356,9899559
k1,77:22695716,9899559:11642360
k1,77:34338076,9899559:11642360
)
(1,78:5920357,11282562:28417720,494436,13271
(1,78:5920357,11282562:1255831,494436,10043
g1,78:5920357,11282562
x1,78:6817379,11282562
g1,78:7176188,11282562
)
x1,78:8012924,11282562
x1,78:9156075,11282562
g1,78:9335479,11282562
x1,78:10930015,11282562
g1,78:11109419,11282562
x1,78:13023292,11282562
g1,78:13202696,11282562
x1,78:16111887,11282562
g1,78:16291291,11282562
x1,78:17048373,11282562
x1,78:18909143,11282562
k1,78:26623610,11282562:7714467
k1,78:34338077,11282562:7714467
)
(1,93:5920357,12570818:28417720,489408,155358
x1,93:7678496,12570818
k1,79:7835212,12570818:156716
x1,79:9045522,12570818
k1,79:9202237,12570818:156715
x1,79:10686119,12570818
k1,79:10842835,12570818:156716
x1,79:11311899,12570818
k1,79:11468614,12570818:156715
x1,79:14631869,12570818
k1,79:14788585,12570818:156716
x1,79:15335719,12570818
k1,79:15492435,12570818:156716
x1,79:15844068,12570818
x1,79:17544888,12570818
k1,79:17701603,12570818:156715
x1,79:18209359,12570818
x1,79:19139626,12570818
k1,79:19296342,12570818:156716
x1,79:19647975,12570818
x1,79:20180760,12570818
k1,79:20337475,12570818:156715
x1,79:21313600,12570818
k1,79:21470316,12570818:156716
x1,79:22134195,12570818
k1,79:22290911,12570818:156716
x1,79:24439375,12570818
k1,79:24596090,12570818:156715
x1,79:25728329,12570818
x1,79:27787965,12570818
k1,79:27944681,12570818:156716
x1,79:28530490,12570818
k1,79:28687205,12570818:156715
x1,79:31988295,12570818
k1,80:32149549,12570818:161254
x1,80:34338077,12570818
k1,80:34338077,12570818:0
)
(1,93:5920357,13462108:28417720,489408,155358
x1,93:6480331,13462108
k1,80:6659496,13462108:179165
x1,80:8039280,13462108
k1,80:8218445,13462108:179165
x1,80:11178085,13462108
k1,80:11357249,13462108:179164
x1,80:12775905,13462108
k1,80:12955118,13462108:179213
x1,80:16073124,13462108
k1,80:16252289,13462108:179165
x1,80:17491003,13462108
k1,80:17670167,13462108:179164
x1,80:18709511,13462108
k1,80:18888676,13462108:179165
x1,80:21966389,13462108
k1,80:22145554,13462108:179165
x1,80:23065413,13462108
k1,80:23244578,13462108:179165
x1,80:25323249,13462108
k1,81:25502413,13462108:179164
x1,81:27201061,13462108
k1,81:27423441,13462108:222380
x1,81:30822157,13462108
k1,81:31001322,13462108:179165
x1,81:32520028,13462108
k1,81:32699193,13462108:179165
x1,81:34338077,13462108
k1,81:34338077,13462108:0
)
(1,93:5920357,14353398:28417720,489408,155358
x1,93:7453539,14353398
k1,81:7633394,14353398:179855
x1,81:8753342,14353398
x1,81:10814791,14353398
k1,81:10994645,14353398:179854
x1,81:12794052,14353398
k1,81:12973907,14353398:179855
x1,81:13653366,14353398
x1,81:14155097,14353398
k1,81:14334952,14353398:179855
x1,81:15973844,14353398
k1,81:16153698,14353398:179854
x1,81:17672395,14353398
k1,81:17852250,14353398:179855
x1,81:19251472,14353398
k1,81:19431327,14353398:179855
x1,81:21471126,14353398
k1,82:21650980,14353398:179854
x1,82:24729404,14353398
k1,82:24909259,14353398:179855
x1,82:26468986,14353398
k1,82:26648841,14353398:179855
x1,82:26888522,14353398
x1,82:28000567,14353398
k1,82:28180421,14353398:179854
x1,82:30618977,14353398
k1,82:30798832,14353398:179855
x1,82:34397639,14353398
k1,82:34338077,14353398:0
)
(1,93:5920357,15244688:28417720,489408,155358
x1,93:8260960,15244688
k1,82:8439834,15244688:178874
x1,82:9004834,15244688
k1,82:9183708,15244688:178874
x1,82:10394319,15244688
k1,82:10573193,15244688:178874
x1,82:12650927,15244688
k1,82:12829801,15244688:178874
x1,82:13394801,15244688
k1,82:13573675,15244688:178874
x1,82:15267967,15244688
k1,82:15446841,15244688:178874
x1,82:18149103,15244688
k1,82:18327977,15244688:178874
x1,82:19215418,15244688
k1,82:19394292,15244688:178874
x1,82:22863447,15244688
k1,82:23042321,15244688:178874
x1,82:23647268,15244688
k1,82:23826142,15244688:178874
x1,82:25479741,15244688
k1,83:25658615,15244688:178874
x1,83:27190940,15244688
k1,83:27369814,15244688:178874
x1,83:27934814,15244688
k1,83:28113688,15244688:178874
x1,83:29001129,15244688
k1,83:29180003,15244688:178874
x1,83:30390614,15244688
k1,83:30569488,15244688:178874
x1,83:31295718,15244688
k1,83:31474592,15244688:178874
x1,83:34338077,15244688
k1,83:34338077,15244688:0
)
(1,93:5920357,16135978:28417720,489408,155358
x1,93:7716485,16135978
k1,83:7892202,16135978:175717
x1,83:8751582,16135978
x1,83:9092457,16135978
k1,83:9268174,16135978:175717
x1,83:10790730,16135978
k1,83:10966447,16135978:175717
x1,83:11825827,16135978
k1,83:12001544,16135978:175717
x1,83:15008685,16135978
x1,83:15145037,16135978
k1,83:15366268,16135978:221231
x1,83:17163793,16135978
k1,83:17339510,16135978:175717
x1,83:17925328,16135978
k1,83:18101044,16135978:175716
x1,83:19117242,16135978
k1,83:19292959,16135978:175717
x1,83:20776832,16135978
k1,83:20952549,16135978:175717
x1,83:23803566,16135978
k1,84:23979283,16135978:175717
x1,84:24799286,16135978
k1,84:24975003,16135978:175717
x1,84:26205718,16135978
k1,84:26381435,16135978:175717
x1,84:28413839,16135978
k1,84:28589556,16135978:175717
x1,84:29136690,16135978
k1,84:29312407,16135978:175717
x1,84:30796289,16135978
k1,84:30972006,16135978:175717
x1,84:31519140,16135978
k1,84:31694857,16135978:175717
x1,84:33277205,16135978
k1,84:33453659,16135978:176454
x1,84:33805292,16135978
x1,84:34338077,16135978
k1,84:34338077,16135978:0
)
(1,93:5920357,17027268:28417720,489408,155358
x1,93:6808675,17027268
k1,84:6988605,17027268:179930
x1,84:9249373,17027268
k1,84:9429302,17027268:179929
x1,84:12577679,17027268
k1,84:12757609,17027268:179930
x1,84:15421828,17027268
k1,84:15601757,17027268:179929
x1,84:18023923,17027268
k1,85:18203853,17027268:179930
x1,85:19657749,17027268
k1,85:19837678,17027268:179929
x1,85:20887386,17027268
k1,85:21067316,17027268:179930
x1,85:22521212,17027268
k1,85:22701141,17027268:179929
x1,85:24113586,17027268
k1,85:24293516,17027268:179930
x1,85:24859074,17027268
k1,85:25039003,17027268:179929
x1,85:28188099,17027268
k1,85:28368029,17027268:179930
x1,85:29619094,17027268
k1,85:29799023,17027268:179929
x1,85:31332873,17027268
k1,85:31512803,17027268:179930
x1,85:33592590,17027268
k1,85:33772519,17027268:179929
x1,85:34338077,17027268
k1,85:34338077,17027268:0
)
(1,93:5920357,17918558:28417720,489408,155358
x1,93:8237437,17918558
k1,85:8417403,17918558:179966
x1,85:9436022,17918558
k1,85:9615988,17918558:179966
x1,85:12632331,17918558
k1,86:12812297,17918558:179966
x1,86:13713815,17918558
k1,86:13893780,17918558:179965
x1,86:15931003,17918558
k1,86:16110969,17918558:179966
x1,86:17207880,17918558
k1,86:17432025,17918558:224145
x1,86:19293599,17918558
k1,86:19473705,17918558:180106
x1,86:21374096,17918558
k1,86:21554203,17918558:180107
x1,86:23709225,17918558
k1,86:23889191,17918558:179966
x1,86:27493827,17918558
k1,86:27673792,17918558:179965
x1,86:29162215,17918558
k1,86:29342181,17918558:179966
x1,86:31360373,17918558
k1,86:31540339,17918558:179966
x1,86:32089148,17918558
k1,86:32269114,17918558:179966
x1,86:34463660,17918558
k1,87:34338077,17918558:0
)
(1,93:5920357,18809848:28417720,489408,155358
x1,93:6343152,18809848
x1,87:6649938,18809848
k1,87:6829906,18809848:179968
x1,87:9055810,18809848
k1,87:9235779,18809848:179969
x1,87:10732580,18809848
k1,87:10912548,18809848:179968
x1,87:11924244,18809848
k1,87:12104213,18809848:179969
x1,87:12832586,18809848
x1,87:13189602,18809848
k1,87:13369570,18809848:179968
x1,87:14907165,18809848
k1,87:15087134,18809848:179969
x1,87:15693873,18809848
k1,87:15873841,18809848:179968
x1,87:17410716,18809848
k1,87:17590684,18809848:179968
x1,87:17995650,18809848
k1,87:18175619,18809848:179969
x1,87:18661435,18809848
k1,87:18841403,18809848:179968
x1,87:21672587,18809848
k1,87:21852556,18809848:179969
x1,87:22419230,18809848
k1,87:22599198,18809848:179968
x1,87:24420134,18809848
k1,87:24600102,18809848:179968
x1,87:25490173,18809848
k1,87:25670142,18809848:179969
x1,87:27571909,18809848
k1,87:27751877,18809848:179968
x1,87:28358616,18809848
k1,87:28538585,18809848:179969
x1,87:29428656,18809848
k1,88:29608624,18809848:179968
x1,88:30862157,18809848
k1,88:31042126,18809848:179969
x1,88:33268038,18809848
k1,88:33448006,18809848:179968
x1,88:34338077,18809848
k1,88:34338077,18809848:0
)
(1,93:5920357,19701138:28417720,489408,155358
x1,93:9321574,19701138
k1,88:9499856,19701138:178282
x1,88:10593506,19701138
x1,88:12863462,19701138
k1,88:13085548,19701138:222086
x1,88:14381872,19701138
k1,88:14560154,19701138:178282
x1,88:15046449,19701138
k1,88:15224731,19701138:178282
x1,88:16642097,19701138
k1,88:16820379,19701138:178282
x1,88:17387612,19701138
k1,88:17565894,19701138:178282
x1,88:17930444,19701138
x1,88:19694401,19701138
k1,88:19872683,19701138:178282
x1,88:20399091,19701138
x1,88:21546068,19701138
k1,88:21724575,19701138:178507
x1,88:24479090,19701138
k1,88:24657372,19701138:178282
x1,88:26480104,19701138
k1,89:24657372,19701138:-7175
x1,89:27768523,19701138
k1,89:27946805,19701138:178282
x1,89:29526750,19701138
k1,89:29705032,19701138:178282
x1,89:30393298,19701138
k1,89:30571580,19701138:178282
x1,89:34338077,19701138
k1,89:34338077,19701138:0
)
(1,93:5920357,20592428:28417720,489408,155358
x1,93:7810545,20592428
k1,89:7989969,20592428:179424
x1,89:9053461,20592428
k1,89:9232885,20592428:179424
x1,89:9941891,20592428
x1,89:12287048,20592428
k1,89:12466472,20592428:179424
x1,89:13332867,20592428
k1,89:13512291,20592428:179424
x1,89:15874688,20592428
k1,89:16054112,20592428:179424
x1,89:19402002,20592428
k1,89:19581426,20592428:179424
x1,89:20842032,20592428
k1,89:21021455,20592428:179423
x1,89:21336250,20592428
k1,89:21515674,20592428:179424
x1,89:23288172,20592428
k1,90:23467596,20592428:179424
x1,90:26145488,20592428
k1,90:26324912,20592428:179424
x1,90:27348713,20592428
k1,90:27528137,20592428:179424
x1,90:28866733,20592428
x1,90:29686245,20592428
k1,90:29865669,20592428:179424
x1,90:32544270,20592428
k1,90:32723694,20592428:179424
x1,90:34338077,20592428
k1,90:34338077,20592428:0
)
(1,93:5920357,21483718:28417720,489408,155358
x1,93:7146721,21483718
k1,90:7326284,21483718:179563
x1,90:9186834,21483718
k1,90:9366396,21483718:179562
x1,90:10078990,21483718
k1,90:10258553,21483718:179563
x1,90:12792509,21483718
k1,90:12972071,21483718:179562
x1,90:14080855,21483718
k1,90:14260418,21483718:179563
x1,90:17308152,21483718
k1,90:17487714,21483718:179562
x1,90:20179159,21483718
k1,91:20358721,21483718:179562
x1,91:21743992,21483718
x1,91:23142042,21483718
k1,91:23364978,21483718:222936
x1,91:23879469,21483718
k1,91:24059031,21483718:179562
x1,91:27145953,21483718
k1,91:27325516,21483718:179563
x1,91:28551880,21483718
k1,91:28731442,21483718:179562
x1,91:29206729,21483718
k1,91:29386292,21483718:179563
x1,91:30613369,21483718
k1,91:30792931,21483718:179562
x1,91:32514544,21483718
k1,91:32694146,21483718:179602
x1,91:33287734,21483718
k1,91:33467297,21483718:179563
x1,91:34338077,21483718
k1,91:34338077,21483718:0
)
(1,93:5920357,22375008:28417720,489408,155358
x1,93:7155366,22375008
g1,91:7334770,22375008
x1,91:9208434,22375008
g1,91:9387838,22375008
x1,91:11341884,22375008
g1,91:11521288,22375008
x1,91:12836670,22375008
g1,91:13016074,22375008
x1,91:13852811,22375008
g1,91:14032215,22375008
x1,91:15965473,22375008
g1,92:16144877,22375008
x1,92:17859241,22375008
g1,92:18038645,22375008
x1,92:18636418,22375008
g1,92:18815822,22375008
x1,92:21047586,22375008
g1,92:21226990,22375008
x1,92:24834404,22375008
k1,93:34338077,22375008:9629256
g1,93:34338077,22375008
)
(1,93:5920357,24447302:28417720,541848,11006
(1,93:5920357,24447302:668472,541848,11006
g1,93:5920357,24447302
x1,93:6510181,24447302
g1,93:6588829,24447302
)
g1,93:6785437,24447302
x1,93:7615117,24447302
x1,93:11314435,24447302
k1,93:22826256,24447302:11511821
k1,93:34338077,24447302:11511821
)
(1,94:5920357,25830305:28417720,494436,146029
(1,94:5920357,25830305:1255831,494436,10043
g1,94:5920357,25830305
x1,94:6817379,25830305
g1,94:7176188,25830305
)
x1,94:9847134,25830305
g1,94:10026538,25830305
x1,94:11501229,25830305
x1,94:12846753,25830305
k1,94:23592415,25830305:10745662
k1,94:34338077,25830305:10745662
)
(1,112:5920357,27118561:28417720,489408,155358
x1,112:7036319,27118561
k1,95:7318960,27118561:282641
x1,95:10571794,27118561
k1,95:10854434,27118561:282640
x1,95:11464162,27118561
k1,95:11746803,27118561:282641
x1,95:14226690,27118561
k1,95:14509330,27118561:282640
x1,95:16907970,27118561
k1,95:17190611,27118561:282641
x1,95:20321212,27118561
k1,95:20603853,27118561:282641
x1,95:22799004,27118561
k1,95:23081644,27118561:282640
x1,95:25074046,27118561
k1,96:25356687,27118561:282641
x1,96:28569287,27118561
k1,96:28851927,27118561:282640
x1,96:31616552,27118561
k1,96:31899193,27118561:282641
x1,96:34338077,27118561
k1,96:34338077,27118561:0
)
(1,112:5920357,28009851:28417720,489408,155358
x1,112:8332885,28009851
k1,96:8512325,28009851:179440
x1,96:9817185,28009851
k1,96:9996624,28009851:179439
x1,96:10589606,28009851
k1,96:10769046,28009851:179440
x1,96:12271801,28009851
k1,96:12451241,28009851:179440
x1,96:14883693,28009851
k1,97:15063141,28009851:179448
x1,97:16249122,28009851
k1,97:16428562,28009851:179440
x1,97:19334415,28009851
k1,97:19513864,28009851:179449
x1,97:20185872,28009851
k1,97:20365311,28009851:179439
x1,97:23469058,28009851
k1,97:23648507,28009851:179449
x1,97:27562372,28009851
k1,97:27741812,28009851:179440
x1,97:30174257,28009851
k1,98:30353705,28009851:179448
x1,98:31974624,28009851
k1,98:32154064,28009851:179440
x1,98:34427779,28009851
k1,98:34338077,28009851:0
)
(1,112:5920357,28901141:28417720,489408,155358
x1,112:7209441,28901141
k1,98:7358080,28901141:148639
x1,98:9370105,28901141
k1,98:9524898,28901141:154793
x1,98:11008780,28901141
k1,98:11157420,28901141:148640
x1,98:13911376,28901141
k1,98:14066169,28901141:154793
x1,98:15550745,28901141
k1,98:15699384,28901141:148639
x1,98:17867532,28901141
k1,99:18022325,28901141:154793
x1,99:19037837,28901141
k1,99:19186476,28901141:148639
x1,99:20397489,28901141
x1,99:20738364,28901141
k1,99:20887004,28901141:148640
x1,99:22332202,28901141
k1,99:22480841,28901141:148639
x1,99:26055494,28901141
k1,99:26267699,28901141:212205
x1,99:28728401,28901141
k1,99:28877041,28901141:148640
x1,99:31415813,28901141
k1,99:31564452,28901141:148639
x1,99:33127072,28901141
x1,99:34338077,28901141
k1,100:34338077,28901141:0
)
(1,112:5920357,29792431:28417720,489408,155358
x1,112:8074521,29792431
k1,100:8254519,29792431:179998
x1,100:8986489,29792431
k1,100:9166486,29792431:179997
x1,100:9532471,29792431
x1,100:11592505,29792431
k1,100:11772503,29792431:179998
x1,100:12097493,29792431
k1,100:12277491,29792431:179998
x1,100:14107398,29792431
k1,100:14287396,29792431:179998
x1,100:15710333,29792431
k1,100:15890330,29792431:179997
x1,100:16215320,29792431
x1,100:18359459,29792431
k1,100:18539457,29792431:179998
x1,100:20329103,29792431
k1,100:20509101,29792431:179998
x1,100:21566061,29792431
k1,101:21746059,29792431:179998
x1,101:23332224,29792431
k1,101:23512221,29792431:179997
x1,101:24610158,29792431
k1,101:24790156,29792431:179998
x1,101:25359622,29792431
k1,101:25539620,29792431:179998
x1,101:26800061,29792431
x1,101:27117876,29792431
k1,101:27297874,29792431:179998
x1,101:30550709,29792431
k1,101:30730706,29792431:179997
x1,101:31340434,29792431
k1,101:31520432,29792431:179998
x1,101:34427779,29792431
k1,101:34338077,29792431:0
)
(1,112:5920357,30683721:28417720,489408,155358
x1,112:7578759,30683721
k1,101:7758073,30683721:179314
x1,101:8982679,30683721
k1,101:9161994,30683721:179315
x1,101:10505359,30683721
k1,102:9161994,30683721:-17941
x1,102:11909729,30683721
k1,102:12089043,30683721:179314
x1,102:14064604,30683721
k1,102:14243918,30683721:179314
x1,102:15745140,30683721
k1,102:15924455,30683721:179315
x1,102:18333846,30683721
k1,102:18513160,30683721:179314
x1,102:22009884,30683721
k1,102:22232314,30683721:222430
x1,102:23890725,30683721
k1,102:24070039,30683721:179314
x1,102:24938352,30683721
k1,102:25117667,30683721:179315
x1,102:26342272,30683721
x1,102:26687094,30683721
k1,102:26866408,30683721:179314
x1,102:27419684,30683721
x1,102:29297120,30683721
k1,103:29476434,30683721:179314
x1,103:30977674,30683721
k1,103:31156989,30683721:179315
x1,103:31749382,30683721
k1,103:31928696,30683721:179314
x1,103:34338077,30683721
k1,103:34338077,30683721:0
)
(1,112:5920357,31575011:28417720,489408,155358
x1,112:8318997,31575011
k1,103:8563745,31575011:244748
x1,103:11856117,31575011
k1,103:12100866,31575011:244749
x1,103:12425856,31575011
x1,103:12777492,31575011
x1,103:14710949,31575011
k1,103:14955697,31575011:244748
x1,103:16257124,31575011
k1,103:16501872,31575011:244748
x1,103:17396328,31575011
k1,104:17641077,31575011:244749
x1,104:20528660,31575011
k1,104:20773408,31575011:244748
x1,104:21342874,31575011
k1,104:21587623,31575011:244749
x1,104:22807803,31575011
x1,104:23122035,31575011
k1,104:23366783,31575011:244748
x1,104:27594606,31575011
k1,104:27839354,31575011:244748
x1,104:30746710,31575011
k1,104:31165203,31575011:418493
x1,104:32384658,31575011
k1,104:32629407,31575011:244749
x1,104:33198873,31575011
k1,104:33443621,31575011:244748
x1,104:34338077,31575011
k1,104:34338077,31575011:0
)
(1,112:5920357,32466301:28417720,489408,155358
x1,112:7749531,32466301
k1,105:7968479,32466301:218948
x1,105:8578207,32466301
k1,105:8797155,32466301:218948
x1,105:9854831,32466301
k1,105:10073779,32466301:218948
x1,105:11659944,32466301
k1,105:11878892,32466301:218948
x1,105:13667813,32466301
k1,105:13886761,32466301:218948
x1,105:14415241,32466301
x1,105:15017785,32466301
k1,105:15236733,32466301:218948
x1,105:17513140,32466301
k1,105:17732088,32466301:218948
x1,105:18464058,32466301
k1,105:18683006,32466301:218948
x1,105:20309406,32466301
x1,105:22688281,32466301
k1,105:22917115,32466301:228834
x1,105:23811571,32466301
k1,105:24030519,32466301:218948
x1,105:27080598,32466301
k1,106:27299546,32466301:218948
x1,106:28397483,32466301
k1,106:28616431,32466301:218948
x1,106:29999106,32466301
x1,106:30794374,32466301
k1,106:31013322,32466301:218948
x1,106:31501532,32466301
k1,106:31720480,32466301:218948
x1,106:33387159,32466301
k1,106:33606107,32466301:218948
x1,106:34338077,32466301
k1,106:34338077,32466301:0
)
(1,112:5920357,33357591:28417720,489408,155358
x1,112:6978033,33357591
k1,106:7181861,33357591:203828
x1,106:8828775,33357591
k1,106:9124508,33357591:295733
x1,106:11685644,33357591
k1,106:11889473,33357591:203829
x1,106:14288113,33357591
k1,107:14491941,33357591:203828
x1,107:16118341,33357591
x1,107:18314224,33357591
k1,107:18518052,33357591:203828
x1,107:20183990,33357591
k1,107:20387819,33357591:203829
x1,107:20957285,33357591
k1,107:21161113,33357591:203828
x1,107:22055569,33357591
k1,107:22259397,33357591:203828
x1,107:24454548,33357591
k1,107:24658376,33357591:203828
x1,107:25268104,33357591
k1,107:25471933,33357591:203829
x1,107:27870573,33357591
k1,107:28074401,33357591:203828
x1,107:28643867,33357591
k1,107:28847695,33357591:203828
x1,107:30677594,33357591
k1,108:30881423,33357591:203829
x1,108:33564783,33357591
k1,108:33768611,33357591:203828
x1,108:34338077,33357591
k1,108:34338077,33357591:0
)
(1,112:5920357,34248881:28417720,489408,155358
x1,112:7488674,34248881
x1,112:8900937,34248881
k1,108:9080517,34248881:179580
x1,108:11217950,34248881
k1,108:11440940,34248881:222990
x1,108:11833547,34248881
x1,108:14019551,34248881
x1,108:14149446,34248881
k1,108:14329071,34248881:179625
x1,108:15740619,34248881
k1,108:15920199,34248881:179580
x1,108:16782380,34248881
k1,108:16961961,34248881:179581
x1,108:17550161,34248881
k1,109:16961961,34248881:-17941
x1,109:17885288,34248881
x1,109:18933010,34248881
k1,109:19112590,34248881:179580
x1,109:20603225,34248881
k1,109:20782805,34248881:179580
x1,109:21371014,34248881
k1,109:21550595,34248881:179581
x1,109:23864578,34248881
k1,109:24044158,34248881:179580
x1,109:25338494,34248881
k1,109:25518075,34248881:179581
x1,109:26106275,34248881
k1,109:26285855,34248881:179580
x1,109:29482501,34248881
k1,109:29662126,34248881:179625
x1,109:31231133,34248881
x1,109:34427779,34248881
k1,109:34338077,34248881:0
)
(1,112:5920357,35140171:28417720,489408,155358
x1,112:9886598,35140171
g1,110:10066002,35140171
x1,110:14270479,35140171
g1,110:14449883,35140171
x1,110:17997747,35140171
g1,110:18177151,35140171
x1,110:19213387,35140171
g1,110:19392791,35140171
x1,110:21744400,35140171
g1,110:21923804,35140171
x1,110:22482104,35140171
g1,110:22661508,35140171
x1,110:24096008,35140171
k1,112:34338077,35140171:10242069
g1,112:34338077,35140171
)
(1,113:5920357,36902013:28417720,487261,8965
(1,113:5920357,36902013:1973449,487261,8965
g1,113:5920357,36902013
x1,113:7534997,36902013
g1,113:7893806,36902013
)
x1,113:9937556,36902013
x1,113:11758845,36902013
g1,113:11938249,36902013
x1,113:15243554,36902013
k1,113:24790816,36902013:9547262
k1,113:34338078,36902013:9547262
)
(1,114:5920357,38190270:28417720,487261,8965
(1,114:5920357,38190270:1973449,487261,8965
g1,114:5920357,38190270
x1,114:7534997,38190270
g1,114:7893806,38190270
)
x1,114:10861123,38190270
x1,114:12682412,38190270
g1,114:12861816,38190270
x1,114:16167121,38190270
k1,114:25252599,38190270:9085478
k1,114:34338077,38190270:9085478
)
(1,115:5920357,39504740:28417720,541848,11006
(1,115:5920357,39504740:668472,541848,11006
g1,115:5920357,39504740
x1,115:6510181,39504740
g1,115:6588829,39504740
)
g1,115:6785437,39504740
x1,115:9930339,39504740
x1,115:10265359,39504740
g1,115:10461967,39504740
x1,115:11378939,39504740
x1,115:12895958,39504740
k1,115:23602862,39504740:10735216
k1,115:34338078,39504740:10735216
)
(1,117:5920357,40887743:28417720,489408,155358
x1,117:6570154,40887743
x1,116:6834235,40887743
k1,116:7014046,40887743:179811
x1,116:9024058,40887743
k1,116:9203870,40887743:179812
x1,116:10129232,40887743
k1,116:10309043,40887743:179811
x1,116:11274234,40887743
k1,116:11454046,40887743:179812
x1,116:12700895,40887743
x1,116:13011623,40887743
x1,116:13362903,40887743
k1,116:13542714,40887743:179811
x1,116:14106038,40887743
k1,116:14285849,40887743:179811
x1,116:15009916,40887743
x1,116:15364779,40887743
k1,116:15544591,40887743:179812
x1,116:16992726,40887743
k1,116:17172537,40887743:179811
x1,116:18761139,40887743
k1,116:18984821,40887743:223682
x1,116:19587974,40887743
k1,116:19767786,40887743:179812
x1,116:20652596,40887743
k1,116:20832407,40887743:179811
x1,116:21959048,40887743
k1,116:22138860,40887743:179812
x1,116:23445804,40887743
k1,116:23625717,40887743:179913
x1,116:24469984,40887743
k1,116:24649795,40887743:179811
x1,116:26901654,40887743
k1,116:27081466,40887743:179812
x1,116:27805542,40887743
k1,116:27985353,40887743:179811
x1,116:28870163,40887743
k1,116:29049975,40887743:179812
x1,116:31061425,40887743
k1,116:31241236,40887743:179811
x1,116:34338077,40887743
k1,116:34338077,40887743:0
)
(1,117:5920357,41779033:28417720,489408,155358
x1,117:6814813,41779033
k1,116:6998576,41779033:183763
x1,116:9438211,41779033
k1,116:9621974,41779033:183763
x1,116:10231702,41779033
k1,116:10415465,41779033:183763
x1,116:12082135,41779033
k1,116:12265898,41779033:183763
x1,116:13525606,41779033
k1,116:13709369,41779033:183763
x1,116:15253815,41779033
k1,116:15437578,41779033:183763
x1,116:18120946,41779033
k1,116:18304709,41779033:183763
x1,116:19890874,41779033
k1,116:20074638,41779033:183764
x1,116:22554499,41779033
k1,116:22738262,41779033:183763
(1,116:22738262,41779033:0,0,0
(1,116:22738262,40887743:0,0,0
)
)
x1,116:25299398,41779033
k1,116:25483161,41779033:183763
x1,116:28125553,41779033
k1,116:28309316,41779033:183763
x1,116:28553059,41779033
(1,116:28553059,41779033:1076420,479368,0
x1,116:29629479,41779033
)
x1,116:29873222,41779033
k1,116:30056985,41779033:183763
x1,116:32354613,41779033
k1,116:32590150,41779033:235537
x1,116:34338077,41779033
k1,116:34338077,41779033:0
)
(1,117:5920357,42670323:28417720,489408,155358
x1,117:9167544,42670323
k1,116:9346274,42670323:178730
x1,116:11872972,42670323
k1,116:12051701,42670323:178729
x1,116:13856493,42670323
x1,116:14210280,42670323
k1,116:14389010,42670323:178730
x1,116:17356794,42670323
k1,116:17535524,42670323:178730
x1,116:21224501,42670323
k1,116:21403230,42670323:178729
x1,116:23688087,42670323
k1,116:23866817,42670323:178730
x1,116:25430490,42670323
k1,116:25609220,42670323:178730
x1,116:26210571,42670323
k1,116:26389300,42670323:178729
x1,116:27632442,42670323
k1,116:27811172,42670323:178730
x1,116:28412532,42670323
k1,116:28591262,42670323:178730
x1,116:29473442,42670323
k1,116:29652171,42670323:178729
x1,116:31075071,42670323
k1,116:31253936,42670323:178865
x1,116:32497078,42670323
k1,116:32675807,42670323:178729
x1,116:33277167,42670323
k1,116:33455897,42670323:178730
x1,116:34338077,42670323
k1,116:34338077,42670323:0
)
(1,117:5920357,43561613:28417720,489408,155358
x1,117:9208685,43561613
k1,116:9388843,43561613:180158
x1,116:10884828,43561613
k1,116:11064836,43561613:180008
x1,116:11655435,43561613
k1,116:11835443,43561613:180008
x1,116:12701838,43561613
k1,116:12881845,43561613:180007
x1,116:16170173,43561613
k1,116:16350332,43561613:180159
x1,116:17590366,43561613
k1,116:17814637,43561613:224271
x1,116:18366237,43561613
k1,116:18546244,43561613:180007
x1,116:19767142,43561613
x1,116:20074762,43561613
k1,116:20254770,43561613:180008
x1,116:21750763,43561613
k1,116:21930770,43561613:180007
x1,116:25258806,43561613
k1,116:25483077,43561613:224271
x1,116:26389172,43561613
k1,116:26569180,43561613:180008
x1,116:28026166,43561613
k1,116:28206173,43561613:180007
x1,116:30608970,43561613
k1,116:30788978,43561613:180008
x1,116:31654664,43561613
k1,116:31834671,43561613:180007
x1,116:33449063,43561613
k1,116:33629071,43561613:180008
x1,116:34338077,43561613
k1,116:34338077,43561613:0
)
(1,117:5920357,44452903:28417720,489408,155358
x1,117:7091984,44452903
k1,116:7233740,44452903:141756
x1,116:11218394,44452903
k1,116:11360151,44452903:141757
x1,116:11945969,44452903
k1,116:12087725,44452903:141756
x1,116:13689740,44452903
x1,116:15799511,44452903
k1,116:15941268,44452903:141757
x1,116:18148794,44452903
k1,116:18298080,44452903:149286
x1,116:20016849,44452903
k1,116:20158606,44452903:141757
x1,116:21252171,44452903
k1,116:21393927,44452903:141756
x1,116:22097193,44452903
k1,116:22238950,44452903:141757
x1,116:23723526,44452903
k1,116:23865282,44452903:141756
x1,116:25349840,44452903
k1,116:25491596,44452903:141756
x1,116:26194862,44452903
x1,116:27831968,44452903
k1,116:27973725,44452903:141757
x1,116:32172150,44452903
k1,116:32321437,44452903:149287
x1,116:33610512,44452903
k1,116:33752268,44452903:141756
x1,116:34338077,44452903
k1,116:34338077,44452903:0
)
(1,117:5920357,45344193:28417720,489408,155358
x1,117:7263054,45344193
k1,116:7442266,45344193:179212
x1,116:8302523,45344193
k1,116:8481736,45344193:179213
x1,116:9654558,45344193
k1,116:9833770,45344193:179212
x1,116:10889746,45344193
x1,116:11653921,45344193
k1,116:11833133,45344193:179212
x1,116:13123533,45344193
x1,116:15373103,45344193
x1,116:16976057,45344193
k1,116:17155270,45344193:179213
x1,116:19677622,45344193
k1,116:19856872,45344193:179250
x1,116:20443288,45344193
k1,116:20622501,45344193:179213
x1,116:21991032,45344193
k1,116:22170244,45344193:179212
x1,116:23968899,45344193
k1,116:24148112,45344193:179213
x1,116:25086510,45344193
k1,116:25265722,45344193:179212
x1,116:27063662,45344193
k1,116:27242874,45344193:179212
x1,116:27790567,45344193
k1,116:27969780,45344193:179213
x1,116:30159142,45344193
x1,116:31762096,45344193
k1,116:31941308,45344193:179212
x1,116:34463660,45344193
k1,116:34338077,45344193:0
)
(1,117:5920357,46235483:28417720,489408,155358
x1,117:6793281,46235483
k1,116:6965977,46235483:172696
x1,116:8411166,46235483
k1,116:8583863,46235483:172697
x1,116:9638762,46235483
x1,116:11886021,46235483
k1,116:12058717,46235483:172696
x1,116:12644535,46235483
k1,116:12817231,46235483:172696
x1,116:14770176,46235483
x1,116:16371497,46235483
k1,116:16544193,46235483:172696
x1,116:20528847,46235483
k1,116:20701544,46235483:172697
x1,116:23864808,46235483
k1,116:24037504,46235483:172696
x1,116:24662700,46235483
x1,116:25659918,46235483
k1,116:25832614,46235483:172696
x1,116:27199751,46235483
k1,116:27372447,46235483:172696
x1,116:28036326,46235483
k1,116:28209023,46235483:172697
x1,116:28912289,46235483
x1,116:30425494,46235483
k1,116:30598190,46235483:172696
x1,116:32434399,46235483
x1,116:34427779,46235483
k1,116:34338077,46235483:0
)
]
(1,117:5920357,48201563:28417720,357558,1655174
(1,117:5920357,48201563:28417720,357558,1655174
[1,117:5920357,48201563:28417720,357558,1655174
(1,117:5920357,48201563:28417720,357558,101945
h1,117:5920357,48201563:0,0,0
[1,117:5920357,48201563:557064,254353,101945
(1,117:5920357,48201563:557064,254353,0
g1,117:5920357,48201563
(1,117:5920357,48201563:557064,254353,0
k1,117:6082499,48201563:162142
(1,117:6082499,48185760:232781,238550,6025
x1,117:6315280,48185760
)
k1,117:6477421,48201563:162141
)
g1,117:6477421,48201563
)
(1,117:5920357,48201563:557064,364089,101945
g1,117:5920357,48201563
(1,117:5920357,48201563:557064,364089,101945
x1,117:6477421,48201563
)
g1,117:6477421,48201563
)
]
x1,117:7525997,48201563
g1,117:7657069,48201563
x1,117:9025971,48201563
x1,117:9428096,48201563
g1,117:9559168,48201563
x1,117:9937702,48201563
x1,117:10841043,48201563
x1,117:11263616,48201563
k1,117:22754972,48201563:11583106
k1,117:34338078,48201563:11583106
)
(1,117:5920357,49151835:28417720,357558,113504
h1,117:5920357,49151835:0,0,0
x1,117:7696620,49151835
g1,117:7859148,49151835
x1,117:8733126,49151835
x1,117:9461356,49151835
g1,117:9592428,49151835
x1,117:10378860,49151835
g1,117:10509932,49151835
x1,117:11179437,49151835
g1,117:11310509,49151835
$1,117:11310509,49151835
x1,117:12883374,49151835
g1,117:12883374,49151835
x1,117:13197947,49151835
g1,117:13197947,49151835
x1,117:13512520,49151835
g1,117:13512520,49151835
x1,117:13827093,49151835
g1,117:13827093,49151835
x1,117:18545688,49151835
g1,117:18545688,49151835
x1,117:18860261,49151835
g1,117:18860261,49151835
x1,117:19803980,49151835
g1,117:19803980,49151835
x1,117:20118553,49151835
g1,117:20118553,49151835
x1,117:22635137,49151835
g1,117:22635137,49151835
x1,117:22949710,49151835
g1,117:22949710,49151835
x1,117:23578856,49151835
g1,117:23578856,49151835
x1,117:23893429,49151835
g1,117:23893429,49151835
x1,117:24208002,49151835
g1,117:24208002,49151835
x1,117:24522575,49151835
g1,117:24522575,49151835
x1,117:25151721,49151835
$1,117:25151721,49151835
x1,117:25282793,49151835
g1,117:25445321,49151835
x1,117:26697826,49151835
x1,117:27765269,49151835
g1,117:27896341,49151835
x1,117:30633616,49151835
g1,117:30764688,49151835
x1,117:31404836,49151835
g1,117:31535908,49151835
x1,117:32234782,49151835
x1,117:33391883,49151835
g1,117:33522955,49151835
x1,117:33901483,49151835
k1,117:34338077,49151835:436594
)
(1,117:5920357,49774427:28417720,347600,82310
$1,117:5920357,49774427
x1,117:7178649,49774427
g1,117:7178649,49774427
x1,117:7493222,49774427
g1,117:7493222,49774427
x1,117:7807795,49774427
g1,117:7807795,49774427
x1,117:8122368,49774427
g1,117:8122368,49774427
x1,117:9380660,49774427
g1,117:9380660,49774427
x1,117:9695233,49774427
g1,117:9695233,49774427
x1,117:10638952,49774427
g1,117:10638952,49774427
x1,117:10953525,49774427
g1,117:10953525,49774427
x1,117:12840963,49774427
g1,117:12840963,49774427
x1,117:13155536,49774427
g1,117:13155536,49774427
x1,117:14099255,49774427
g1,117:14099255,49774427
x1,117:14413828,49774427
g1,117:14413828,49774427
x1,117:15042974,49774427
g1,117:15042974,49774427
x1,117:15357547,49774427
(1,117:15357547,49839963:32768,0,0
)
g1,117:15390315,49774427
x1,117:16334034,49774427
g1,117:16334034,49774427
x1,117:16648607,49774427
g1,117:16648607,49774427
x1,117:17906899,49774427
$1,117:17906899,49774427
x1,117:18037971,49774427
k1,117:26142149,49774427:8195928
k1,117:34338077,49774427:8195928
)
]
)
)
]
]
]
!33446
}1
!10
{2
[1,131:4736286,48201563:29601791,43465277,0
[1,131:4736286,4736286:0,0,0
(1,131:4736286,2302362:0,0,0
k1,131:4736286,2302362:-1118290
)
]
[1,131:4736286,48201563:29601791,43465277,0
h1,131:4736286,4736286:0,0,0
[1,131:5920357,48201563:28417720,45833420,0
[1,131:5920357,3154575:28417720,786432,0
(1,131:5920357,3154575:28417720,435811,8188
(1,131:5920357,3154575:28417720,435811,8188
k1,131:18797293,3154575:12876936
x1,131:19303229,3154575
x1,131:20783666,3154575
x1,131:21281738,3154575
g1,131:21461142,3154575
k1,131:34338078,3154575:12876936
)
)
]
[1,131:5920357,46235483:28417720,40258437,0
(1,117:5920357,6697942:28417720,489408,155358
x1,117:7651876,6697942
k1,116:7831491,6697942:179615
x1,116:8311085,6697942
k1,116:8490700,6697942:179615
x1,116:9369372,6697942
k1,116:9548987,6697942:179615
x1,116:9788429,6697942
x1,116:10619654,6697942
k1,116:10799269,6697942:179615
x1,116:11877831,6697942
k1,116:12057446,6697942:179615
x1,116:12976390,6697942
x1,116:13927701,6697942
k1,116:14107316,6697942:179615
x1,116:15105353,6697942
k1,116:15284968,6697942:179615
x1,116:15963750,6697942
k1,116:16143365,6697942:179615
x1,116:18040921,6697942
k1,116:18220589,6697942:179668
x1,116:21136309,6697942
k1,116:21315924,6697942:179615
x1,116:21914893,6697942
k1,116:22094508,6697942:179615
x1,116:24371007,6697942
k1,116:24550622,6697942:179615
x1,116:25269676,6697942
k1,116:25449291,6697942:179615
x1,116:28464242,6697942
k1,116:28687335,6697942:223093
x1,116:31701584,6697942
k1,116:31881252,6697942:179668
x1,116:32920263,6697942
k1,116:33099878,6697942:179615
x1,116:34338077,6697942
k1,116:34338077,6697942:0
)
(1,117:5920357,7589232:28417720,489408,155358
x1,117:6522315,7589232
k1,116:6702376,7589232:180061
x1,116:8790061,7589232
k1,116:8970122,7589232:180061
x1,116:9852455,7589232
k1,116:10032516,7589232:180061
x1,116:10956045,7589232
k1,116:11136106,7589232:180061
x1,116:13343027,7589232
k1,116:13523088,7589232:180061
x1,116:14125046,7589232
k1,116:14305107,7589232:180061
x1,116:18400989,7589232
k1,116:18581050,7589232:180061
x1,116:19263219,7589232
k1,116:19443280,7589232:180061
x1,116:22493519,7589232
k1,116:22673580,7589232:180061
x1,116:23877486,7589232
k1,116:24057547,7589232:180061
x1,116:25462350,7589232
k1,116:25642411,7589232:180061
x1,116:26324580,7589232
k1,116:26504641,7589232:180061
x1,116:29074323,7589232
x1,116:29226285,7589232
k1,116:29406510,7589232:180225
x1,116:30650897,7589232
k1,116:30830958,7589232:180061
x1,116:34363194,7589232
k1,116:34338077,7589232:0
)
(1,117:5920357,8480522:28417720,489408,155358
x1,117:8359250,8480522
k1,116:8540791,8480522:181541
x1,116:9435247,8480522
k1,116:9616789,8480522:181542
x1,116:10552240,8480522
x1,116:11236040,8480522
k1,116:11417581,8480522:181541
x1,116:12027309,8480522
k1,116:12208851,8480522:181542
x1,116:13306806,8480522
x1,116:15402776,8480522
k1,116:15584317,8480522:181541
x1,116:16194045,8480522
k1,116:16375586,8480522:181541
x1,116:17270042,8480522
k1,116:17451584,8480522:181542
x1,116:20541199,8480522
k1,116:20722740,8480522:181541
x1,116:22857149,8480522
k1,116:23086022,8480522:228873
x1,116:23533255,8480522
x1,116:23841835,8480522
k1,116:24023376,8480522:181541
x1,116:25567812,8480522
x1,116:25915856,8480522
x1,116:26230088,8480522
k1,116:26411629,8480522:181541
x1,116:26736619,8480522
k1,116:26918161,8480522:181542
x1,116:28422345,8480522
k1,116:28603886,8480522:181541
x1,116:30149039,8480522
x1,116:31971038,8480522
k1,116:32152580,8480522:181542
x1,116:32681051,8480522
x1,116:33029095,8480522
x1,116:33546808,8480522
k1,116:33728349,8480522:181541
x1,116:34338077,8480522
k1,116:34338077,8480522:0
)
(1,117:5920357,9371812:28417720,489408,155358
x1,117:8162767,9371812
x1,116:8293200,9371812
k1,116:8472752,9371812:179552
x1,116:9928271,9371812
k1,116:10107793,9371812:179522
x1,116:11130557,9371812
x1,116:12764332,9371812
k1,116:12943854,9371812:179522
x1,116:15973171,9371812
k1,116:16152693,9371812:179522
x1,116:16821313,9371812
x1,116:17161108,9371812
x1,116:17464826,9371812
k1,116:17644349,9371812:179523
x1,116:18981589,9371812
k1,116:19161111,9371812:179522
x1,116:21757681,9371812
k1,116:21937203,9371812:179522
x1,116:22763061,9371812
k1,116:22942583,9371812:179522
x1,116:24122577,9371812
k1,116:24302099,9371812:179522
x1,116:30125569,9371812
x1,116:32427481,9371812
k1,116:32607033,9371812:179552
x1,116:34338077,9371812
k1,116:34338077,9371812:0
)
(1,117:5920357,10263102:28417720,489408,155358
x1,117:6896061,10263102
k1,116:7077686,10263102:181625
x1,116:8459636,10263102
x1,116:10152952,10263102
k1,116:10334577,10263102:181625
x1,116:13424908,10263102
k1,116:13606533,10263102:181625
x1,116:14175999,10263102
k1,116:14357623,10263102:181624
x1,116:16634754,10263102
k1,116:16816379,10263102:181625
x1,116:17507354,10263102
k1,116:17688979,10263102:181625
x1,116:18827911,10263102
x1,116:20639877,10263102
k1,116:20821502,10263102:181625
x1,116:22488181,10263102
k1,116:22669806,10263102:181625
x1,116:23401776,10263102
k1,116:23583401,10263102:181625
x1,116:25575795,10263102
k1,116:25757419,10263102:181624
x1,116:27749830,10263102
k1,116:27931455,10263102:181625
x1,116:29313405,10263102
x1,116:30478250,10263102
k1,116:30659875,10263102:181625
x1,116:32286292,10263102
k1,116:32467917,10263102:181625
x1,116:34338077,10263102
k1,116:34338077,10263102:0
)
(1,117:5920357,11154392:28417720,489408,155358
x1,117:6408567,11154392
k1,116:6604572,11154392:196005
x1,116:9735164,11154392
k1,116:9931170,11154392:196006
x1,116:11232597,11154392
k1,116:11428602,11154392:196005
x1,116:13420996,11154392
k1,116:13617001,11154392:196005
x1,116:16503117,11154392
k1,116:16699122,11154392:196005
x1,116:17390097,11154392
x1,116:19059323,11154392
k1,116:19331587,11154392:272264
x1,116:20469795,11154392
k1,116:20665800,11154392:196005
x1,116:22129722,11154392
k1,116:22325728,11154392:196006
x1,116:23382688,11154392
x1,116:25275168,11154392
k1,116:25471173,11154392:196005
x1,116:26080901,11154392
k1,116:26276906,11154392:196005
x1,116:27781081,11154392
k1,116:27977086,11154392:196005
x1,116:31269458,11154392
k1,116:31465464,11154392:196006
x1,116:31953674,11154392
k1,116:32149679,11154392:196005
x1,116:33247616,11154392
k1,116:33443621,11154392:196005
x1,116:34338077,11154392
k1,116:34338077,11154392:0
)
(1,117:5920357,12045682:28417720,491203,155358
x1,117:8192303,12045682
g1,116:8371707,12045682
x1,116:9926035,12045682
g1,116:10105439,12045682
x1,116:10823057,12045682
g1,116:11002461,12045682
x1,116:12198725,12045682
g1,116:12378129,12045682
x1,116:14291283,12045682
g1,116:14470687,12045682
x1,116:15825541,12045682
x1,116:16170001,12045682
x1,116:16477861,12045682
g1,116:16657265,12045682
x1,116:18929211,12045682
g1,116:19108615,12045682
x1,116:19706388,12045682
g1,116:19885792,12045682
x1,116:21281547,12045682
g1,116:21473863,12045682
x1,116:22350781,12045682
x1,116:22698832,12045682
g1,116:22878236,12045682
x1,116:24014222,12045682
g1,116:24193626,12045682
x1,116:25947471,12045682
g1,116:26126875,12045682
x1,116:28040029,12045682
g1,116:28219433,12045682
x1,116:28896860,12045682
g1,116:29076264,12045682
x1,116:30750437,12045682
g1,116:30929841,12045682
x1,116:31766578,12045682
x1,116:32969305,12045682
k1,117:34338077,12045682:1494355
g1,117:34338077,12045682
)
(1,119:5920357,13126741:28417720,489408,155358
h1,118:5920357,13126741:1114112,0,0
x1,118:7623874,13126741
k1,118:7803968,13126741:180094
x1,118:8668609,13126741
k1,118:8848703,13126741:180094
x1,118:10813613,13126741
k1,118:10993707,13126741:180094
x1,118:12093967,13126741
k1,118:12274060,13126741:180093
x1,118:12863465,13126741
k1,118:13043559,13126741:180094
x1,118:13986750,13126741
k1,118:14166844,13126741:180094
x1,118:15385273,13126741
x1,118:15688672,13126741
x1,118:16031700,13126741
x1,118:16161953,13126741
k1,118:16342219,13126741:180266
x1,118:17167240,13126741
k1,118:17347334,13126741:180094
x1,118:17897110,13126741
x1,118:18743810,13126741
x1,118:19236733,13126741
k1,118:19416827,13126741:180094
x1,118:20910492,13126741
k1,118:21090586,13126741:180094
x1,118:21679991,13126741
k1,118:21860085,13126741:180094
x1,118:22724726,13126741
k1,118:22904820,13126741:180094
x1,118:24633394,13126741
k1,118:24813488,13126741:180094
x1,118:26779089,13126741
k1,118:26959182,13126741:180093
x1,118:29985433,13126741
k1,118:30165527,13126741:180094
x1,118:31030168,13126741
k1,118:31210262,13126741:180094
x1,118:33568578,13126741
k1,118:33748672,13126741:180094
x1,118:34338077,13126741
k1,118:34338077,13126741:0
)
(1,119:5920357,14018031:28417720,489408,155358
x1,119:7094374,14018031
k1,118:7274155,14018031:179781
x1,118:11266937,14018031
k1,118:11446718,14018031:179781
x1,118:12973789,14018031
k1,118:13153571,14018031:179782
x1,118:14484037,14018031
x1,118:16113734,14018031
k1,118:16293515,14018031:179781
x1,118:19444891,14018031
k1,118:19668482,14018031:223591
x1,118:20099045,14018031
k1,118:20278826,14018031:179781
x1,118:20748847,14018031
k1,118:20928629,14018031:179782
x1,118:21437421,14018031
x1,118:22565509,14018031
k1,118:22745290,14018031:179781
x1,118:25094740,14018031
k1,118:25274521,14018031:179781
x1,118:26175121,14018031
k1,118:26354902,14018031:179781
x1,118:27411935,14018031
k1,118:27591716,14018031:179781
x1,118:29039853,14018031
k1,118:29219634,14018031:179781
x1,118:30628313,14018031
k1,118:30808095,14018031:179782
x1,118:31747449,14018031
k1,118:31927230,14018031:179781
x1,118:32827830,14018031
k1,118:33007611,14018031:179781
x1,118:34338077,14018031
k1,118:34338077,14018031:0
)
(1,119:5920357,14909321:28417720,489408,155358
x1,119:7290290,14909321
k1,118:7468908,14909321:178618
x1,118:9543541,14909321
k1,118:9722160,14909321:178619
x1,118:11249231,14909321
k1,118:11427849,14909321:178618
x1,118:11976099,14909321
k1,118:12154718,14909321:178619
x1,118:13015851,14909321
k1,118:13194469,14909321:178618
x1,118:14447411,14909321
k1,118:14626030,14909321:178619
x1,118:15213043,14909321
k1,118:15391661,14909321:178618
x1,118:16878570,14909321
k1,118:17057189,14909321:178619
x1,118:19640588,14909321
k1,118:19819206,14909321:178618
x1,118:21346277,14909321
k1,118:21524896,14909321:178619
x1,118:22855362,14909321
x1,118:24485059,14909321
k1,118:24663677,14909321:178618
x1,118:27815053,14909321
k1,118:27993829,14909321:178776
x1,118:28815504,14909321
k1,118:28994122,14909321:178618
x1,118:31185722,14909321
k1,118:31364341,14909321:178619
x1,118:32303704,14909321
k1,118:32482322,14909321:178618
x1,118:33029868,14909321
x1,118:33873060,14909321
x1,118:34363911,14909321
k1,118:34338077,14909321:0
)
(1,119:5920357,15800611:28417720,489408,155358
x1,119:6648021,15800611
k1,118:6828431,15800611:180410
x1,118:8969925,15800611
k1,118:9150334,15800611:180409
x1,118:10362608,15800611
k1,118:10543018,15800611:180410
x1,118:14665914,15800611
k1,118:14846324,15800611:180410
x1,118:18119331,15800611
k1,118:18299741,15800611:180410
x1,118:20118884,15800611
x1,118:21405489,15800611
k1,118:21585898,15800611:180409
x1,118:22959720,15800611
x1,118:24642991,15800611
k1,118:24823401,15800611:180410
x1,118:27895554,15800611
k1,118:28075964,15800611:180410
x1,118:28642080,15800611
k1,118:28822489,15800611:180409
x1,118:31086225,15800611
k1,118:31266635,15800611:180410
x1,118:34338077,15800611
k1,118:34338077,15800611:0
)
(1,119:5920357,16691901:28417720,489408,155358
x1,119:7424533,16691901
k1,118:7606236,16691901:181703
x1,118:9029173,16691901
k1,118:9210876,16691901:181703
x1,118:12281452,16691901
k1,118:12510808,16691901:229356
x1,118:13242769,16691901
k1,118:13424472,16691901:181703
x1,118:14318928,16691901
k1,118:14500631,16691901:181703
x1,118:15740583,16691901
k1,118:15922860,16691901:182277
x1,118:16776330,16691901
k1,118:16958033,16691901:181703
x1,118:17486513,16691901
x1,118:18780774,16691901
k1,118:18962477,16691901:181703
x1,118:19735424,16691901
x1,118:20053239,16691901
k1,118:20234942,16691901:181703
x1,118:20804408,16691901
k1,118:20986110,16691901:181702
x1,118:23385483,16691901
k1,118:23567186,16691901:181703
x1,118:24665123,16691901
k1,118:24846826,16691901:181703
x1,118:26148253,16691901
k1,118:26329956,16691901:181703
x1,118:26898689,16691901
x1,118:27253916,16691901
x1,118:28185050,16691901
k1,118:28366753,16691901:181703
x1,118:28936219,16691901
k1,118:29117922,16691901:181703
x1,118:30012378,16691901
k1,118:30194080,16691901:181702
x1,118:32226744,16691901
k1,118:32408447,16691901:181703
x1,118:33546646,16691901
k1,118:33728349,16691901:181703
x1,118:34338077,16691901
k1,118:34338077,16691901:0
)
(1,119:5920357,17583191:28417720,489408,155358
x1,119:6806044,17583191
k1,118:6985755,17583191:179711
x1,118:8233840,17583191
x1,118:8544886,17583191
x1,118:8896525,17583191
x1,118:9031084,17583191
k1,118:9210871,17583191:179787
x1,118:10055974,17583191
k1,118:10235685,17583191:179711
x1,118:11643946,17583191
k1,118:11823657,17583191:179711
x1,118:13837110,17583191
k1,118:14016820,17583191:179710
x1,118:16994978,17583191
k1,118:17174689,17583191:179711
x1,118:18785170,17583191
k1,118:18964881,17583191:179711
x1,118:19850568,17583191
k1,118:20030278,17583191:179710
x1,118:20594161,17583191
x1,118:22507593,17583191
k1,118:22687304,17583191:179711
x1,118:26793935,17583191
k1,118:26973646,17583191:179711
x1,118:29429212,17583191
k1,118:29608923,17583191:179711
x1,118:30937458,17583191
k1,118:31117168,17583191:179710
x1,118:31681051,17583191
k1,118:31860762,17583191:179711
x1,118:32424645,17583191
x1,118:34338077,17583191
k1,118:34338077,17583191:0
)
(1,119:5920357,18474481:28417720,489408,155358
x1,119:6423003,18474481
x1,118:7859262,18474481
k1,118:8045647,18474481:186385
x1,118:10566529,18474481
k1,118:10751518,18474481:184989
x1,118:12032447,18474481
k1,118:12218832,18474481:186385
x1,118:13072302,18474481
k1,118:13257290,18474481:184988
x1,118:13826023,18474481
x1,118:14702538,18474481
x1,118:15904052,18474481
k1,118:16089041,18474481:184989
x1,118:17146001,18474481
k1,118:17330990,18474481:184989
x1,118:20217124,18474481
k1,118:20402113,18474481:184989
x1,118:22435493,18474481
k1,118:22620481,18474481:184988
x1,118:23189947,18474481
k1,118:23374936,18474481:184989
x1,118:25001345,18474481
k1,118:25186334,18474481:184989
x1,118:25796062,18474481
k1,118:25981051,18474481:184989
x1,118:26550517,18474481
x1,118:28482893,18474481
k1,118:28667881,18474481:184988
x1,118:30049831,18474481
x1,118:31743147,18474481
k1,118:31928136,18474481:184989
x1,118:34427779,18474481
k1,118:34338077,18474481:0
)
(1,119:5920357,19365771:28417720,489408,155358
x1,119:7593821,19365771
g1,118:7773225,19365771
x1,118:9008952,19365771
g1,118:9188356,19365771
x1,118:12416174,19365771
g1,118:12595578,19365771
x1,118:13671987,19365771
g1,118:13851391,19365771
x1,118:14728309,19365771
x1,118:15076360,19365771
g1,118:15255764,19365771
x1,118:16571146,19365771
g1,118:16750550,19365771
x1,118:17587287,19365771
g1,118:17766691,19365771
x1,118:18962228,19365771
g1,118:19141632,19365771
x1,118:23387008,19365771
k1,119:34338077,19365771:11076652
g1,119:34338077,19365771
)
(1,120:5920357,21394071:28417720,494436,146029
(1,120:5920357,21394071:1255831,494436,10043
g1,120:5920357,21394071
x1,120:6817379,21394071
g1,120:7176188,21394071
)
x1,120:9090061,21394071
g1,120:9269465,21394071
x1,120:12178656,21394071
g1,120:12358060,21394071
x1,120:12876178,21394071
x1,120:13974837,21394071
x1,120:15994915,21394071
g1,120:16174319,21394071
x1,120:18008529,21394071
g1,120:18187933,21394071
x1,120:18945733,21394071
g1,120:19125137,21394071
x1,120:19603783,21394071
x1,120:22581143,21394071
g1,120:22760547,21394071
(1,120:22760547,21394071:1156074,482592,0
x1,120:23916621,21394071
)
g1,120:24096025,21394071
x1,120:26328508,21394071
k1,120:30333293,21394071:4004785
k1,120:34338077,21394071:4004784
)
(1,122:5920357,22854041:28417720,489408,155358
x1,122:6320146,22854041
x1,121:6908357,22854041
k1,121:7088121,22854041:179764
x1,121:8127132,22854041
k1,121:8306896,22854041:179764
x1,121:9545096,22854041
x1,121:9853593,22854041
x1,121:10202362,22854041
x1,121:10335486,22854041
k1,121:10515340,22854041:179854
x1,121:11353749,22854041
k1,121:11533513,22854041:179764
x1,121:14048733,22854041
k1,121:14228497,22854041:179764
x1,121:16465464,22854041
k1,121:16645228,22854041:179764
x1,121:19081363,22854041
k1,121:19261126,22854041:179763
x1,121:21777066,22854041
k1,121:21956830,22854041:179764
x1,121:22795241,22854041
k1,121:22975005,22854041:179764
x1,121:24731629,22854041
k1,121:24911393,22854041:179764
x1,121:26788804,22854041
x1,121:27507848,22854041
k1,121:27687612,22854041:179764
x1,121:29564322,22854041
k1,121:29744086,22854041:179764
x1,121:32540460,22854041
k1,121:32720224,22854041:179764
x1,121:33279641,22854041
k1,121:33459405,22854041:179764
x1,121:34338077,22854041
k1,121:34338077,22854041:0
)
(1,122:5920357,23745331:28417720,489408,155358
x1,122:7443616,23745331
x1,121:7979992,23745331
k1,121:8131106,23745331:151114
x1,121:8716924,23745331
k1,121:8868038,23745331:151114
x1,121:10469350,23745331
k1,121:10620465,23745331:151115
x1,121:11830775,23745331
k1,121:11981889,23745331:151114
x1,121:13465771,23745331
k1,121:13616885,23745331:151114
x1,121:16195025,23745331
k1,121:16346139,23745331:151114
x1,121:17870102,23745331
k1,121:18021217,23745331:151115
(1,121:18021217,23745331:1076420,479368,0
x1,121:19097637,23745331
)
k1,121:19248751,23745331:151114
x1,121:21456277,23745331
k1,121:21669307,23745331:213030
x1,121:23739692,23745331
k1,121:23890806,23745331:151114
x1,121:25257943,23745331
k1,121:25409057,23745331:151114
x1,121:27049765,23745331
k1,121:27200880,23745331:151115
x1,121:30247389,23745331
k1,121:30398503,23745331:151114
x1,121:31414015,23745331
k1,121:31565129,23745331:151114
x1,121:34338077,23745331
k1,121:34338077,23745331:0
)
(1,122:5920357,24636621:28417720,489408,155358
x1,122:8887739,24636621
k1,121:9076820,24636621:189081
x1,121:10499023,24636621
k1,121:10688105,24636621:189082
x1,121:11582561,24636621
k1,121:11771642,24636621:189081
x1,121:13195303,24636621
k1,121:13384384,24636621:189081
x1,121:15173297,24636621
k1,121:15362378,24636621:189081
x1,121:15728363,24636621
x1,121:16046178,24636621
x1,121:16929885,24636621
x1,121:18183152,24636621
k1,121:18372234,24636621:189082
x1,121:18941700,24636621
k1,121:19130781,24636621:189081
x1,121:20269722,24636621
k1,121:20458803,24636621:189081
x1,121:21353259,24636621
k1,121:21542341,24636621:189082
x1,121:22639545,24636621
x1,121:22987589,24636621
x1,121:23864104,24636621
k1,121:24053185,24636621:189081
x1,121:26350062,24636621
k1,121:26601554,24636621:251492
x1,121:27211282,24636621
k1,121:27400363,24636621:189081
x1,121:28458039,24636621
k1,121:28647120,24636621:189081
x1,121:30334287,24636621
k1,121:30525788,24636621:191501
x1,121:31257758,24636621
k1,121:31446839,24636621:189081
x1,121:32015572,24636621
x1,121:32892087,24636621
x1,121:34338077,24636621
k1,121:34338077,24636621:0
)
(1,122:5920357,25527911:28417720,489408,155358
x1,122:6814813,25527911
k1,121:7026565,25527911:211752
x1,121:9302954,25527911
k1,121:9514706,25527911:211752
x1,121:10571666,25527911
k1,121:10783417,25527911:211751
x1,121:11922331,25527911
k1,121:12134083,25527911:211752
x1,121:12743811,25527911
k1,121:12955563,25527911:211752
x1,121:13850019,25527911
k1,121:14061771,25527911:211752
x1,121:16704144,25527911
k1,121:16915896,25527911:211752
x1,121:19009310,25527911
k1,121:19229148,25527911:219838
x1,121:20082618,25527911
k1,121:20294370,25527911:211752
x1,121:21961773,25527911
x1,121:23059719,25527911
k1,121:23271471,25527911:211752
x1,121:25568348,25527911
k1,121:25788187,25527911:219839
x1,121:27577108,25527911
k1,121:27788860,25527911:211752
x1,121:28764564,25527911
k1,121:28976315,25527911:211751
(1,121:28976315,25527911:1076420,479368,0
x1,121:30052735,25527911
)
k1,121:30264487,25527911:211752
x1,121:33556859,25527911
k1,121:33768611,25527911:211752
x1,121:34338077,25527911
k1,121:34338077,25527911:0
)
(1,122:5920357,26419201:28417720,489408,155358
x1,122:8055251,26419201
k1,121:8234235,26419201:178984
x1,121:9104138,26419201
k1,121:9283122,26419201:178984
x1,121:11655789,26419201
k1,121:11834773,26419201:178984
x1,121:12427764,26419201
k1,121:12606747,26419201:178983
x1,121:14227666,26419201
k1,121:14406650,26419201:178984
x1,121:15631779,26419201
k1,121:15810763,26419201:178984
x1,121:17312814,26419201
k1,121:17491798,26419201:178984
x1,121:20279476,26419201
k1,121:20501796,26419201:222320
x1,121:21094787,26419201
k1,121:21273771,26419201:178984
x1,121:22143674,26419201
k1,121:22322658,26419201:178984
x1,121:22994666,26419201
x1,121:23537742,26419201
k1,121:23716726,26419201:178984
x1,121:25357580,26419201
k1,121:25536648,26419201:179068
x1,121:27474368,26419201
k1,121:27653351,26419201:178983
x1,121:28365210,26419201
k1,121:28544194,26419201:178984
x1,121:31114033,26419201
k1,121:31293017,26419201:178984
x1,121:33328967,26419201
k1,121:33508035,26419201:179068
x1,121:34338077,26419201
k1,121:34338077,26419201:0
)
(1,122:5920357,27310491:28417720,489408,155358
x1,122:8670966,27310491
g1,121:8850370,27310491
x1,121:9168988,27310491
x1,121:11469648,27310491
g1,121:11649052,27310491
$1,121:11649052,27310491
x1,121:12366672,27310491
$1,121:12366672,27310491
g1,121:12546076,27310491
x1,121:14618513,27310491
g1,121:14797917,27310491
x1,121:17588708,27310491
g1,121:17768112,27310491
x1,121:19082767,27310491
g1,121:19262171,27310491
$1,121:19262171,27310491
x1,121:20697411,27310491
$1,121:20697411,27310491
g1,121:20876815,27310491
x1,121:22152724,27310491
g1,121:22332128,27310491
x1,121:24524437,27310491
g1,121:24703841,27310491
x1,121:25301614,27310491
g1,121:25481018,27310491
x1,121:27912982,27310491
g1,121:28092386,27310491
x1,121:28810004,27310491
g1,121:28989408,27310491
x1,121:30065809,27310491
g1,121:30245213,27310491
x1,121:31480940,27310491
g1,121:31660344,27310491
$1,121:31660344,27310491
x1,121:32377964,27310491
$1,121:32377964,27310491
x1,121:32557368,27310491
k1,122:34338077,27310491:1906292
g1,122:34338077,27310491
)
(1,124:5920357,28391550:28417720,489408,155358
h1,123:5920357,28391550:1114112,0,0
x1,123:8321861,28391550
k1,123:8501648,28391550:179787
x1,123:10552926,28391550
k1,123:10732713,28391550:179787
x1,123:13105478,28391550
k1,123:13285265,28391550:179787
x1,123:13606751,28391550
k1,123:13786538,28391550:179787
x1,123:14349139,28391550
x1,123:15216008,28391550
x1,123:15720848,28391550
k1,123:15900635,28391550:179787
x1,123:16503788,28391550
k1,123:16683575,28391550:179787
x1,123:17568385,28391550
k1,123:17748172,28391550:179787
(1,123:17748172,28391550:1076420,479368,0
x1,123:18824592,28391550
)
k1,123:19004379,28391550:179787
x1,123:22261248,28391550
k1,123:22441035,28391550:179787
x1,123:24733445,28391550
k1,123:24913232,28391550:179787
x1,123:25757500,28391550
k1,123:25937287,28391550:179787
x1,123:28068945,28391550
k1,123:28248732,28391550:179787
x1,123:29536123,28391550
k1,123:29715910,28391550:179787
x1,123:30600720,28391550
k1,123:30780507,28391550:179787
x1,123:33555137,28391550
k1,123:33734924,28391550:179787
x1,123:34338077,28391550
k1,123:34338077,28391550:0
)
(1,124:5920357,29282840:28417720,489408,155358
x1,124:7526570,29282840
k1,123:7706638,29282840:180068
x1,123:8920651,29282840
k1,123:9100718,29282840:180067
x1,123:10589141,29282840
k1,123:10769209,29282840:180068
x1,123:13531593,29282840
k1,123:13756043,29282840:224450
x1,123:16733593,29282840
k1,123:16913661,29282840:180068
x1,123:17462470,29282840
k1,123:17642538,29282840:180068
x1,123:18504548,29282840
k1,123:18684615,29282840:180067
x1,123:21407485,29282840
k1,123:21587719,29282840:180234
x1,123:22841946,29282840
k1,123:23022013,29282840:180067
x1,123:26039055,29282840
k1,123:26219123,29282840:180068
x1,123:27237742,29282840
k1,123:27417809,29282840:180067
x1,123:31140269,29282840
k1,123:31320337,29282840:180068
x1,123:34338077,29282840
k1,123:34338077,29282840:0
)
(1,124:5920357,30174130:28417720,489408,155358
x1,124:6936322,30174130
k1,123:7146065,30174130:209743
x1,123:7837040,30174130
k1,123:8046784,30174130:209744
x1,123:9388473,30174130
k1,123:9598216,30174130:209743
x1,123:10451687,30174130
k1,123:10661431,30174130:209744
x1,123:12328101,30174130
k1,123:12537844,30174130:209743
x1,123:13797552,30174130
k1,123:14007296,30174130:209744
x1,123:15551742,30174130
k1,123:15761485,30174130:209743
x1,123:18627845,30174130
k1,123:18941323,30174130:313478
x1,123:19551051,30174130
k1,123:19760795,30174130:209744
x1,123:20655251,30174130
k1,123:20864994,30174130:209743
x1,123:22247669,30174130
x1,123:23876651,30174130
k1,123:24093979,30174130:217328
x1,123:24947449,30174130
k1,123:25157193,30174130:209744
x1,123:26296116,30174130
k1,123:26505859,30174130:209743
x1,123:28619762,30174130
k1,123:28829506,30174130:209744
x1,123:29520481,30174130
k1,123:29730224,30174130:209743
x1,123:30096209,30174130
x1,123:30451436,30174130
x1,123:31903867,30174130
x1,123:32414406,30174130
k1,123:32624150,30174130:209744
x1,123:33233878,30174130
k1,123:33443621,30174130:209743
x1,123:34338077,30174130
k1,123:34338077,30174130:0
)
(1,124:5920357,31065420:28417720,489408,155358
x1,124:6996048,31065420
x1,123:7336916,31065420
x1,123:8195893,31065420
g1,123:8375297,31065420
x1,123:10368807,31065420
g1,123:10548211,31065420
x1,123:12103275,31065420
g1,123:12282679,31065420
x1,123:13757361,31065420
g1,123:13936765,31065420
x1,123:14654374,31065420
x1,123:15006008,31065420
g1,123:15185412,31065420
x1,123:18413230,31065420
g1,123:18592634,31065420
x1,123:19150934,31065420
g1,123:19330338,31065420
x1,123:21482448,31065420
g1,123:21661852,31065420
x1,123:22538770,31065420
g1,123:22718174,31065420
x1,123:25109974,31065420
g1,123:25289378,31065420
x1,123:25807487,31065420
g1,123:25986891,31065420
x1,123:27561340,31065420
k1,124:34338077,31065420:6902320
g1,124:34338077,31065420
)
(1,125:5920357,32998975:28417720,487261,8965
(1,125:5920357,32998975:1973449,487261,8965
g1,125:5920357,32998975
x1,125:7534997,32998975
g1,125:7893806,32998975
)
x1,125:9937556,32998975
x1,125:11758845,32998975
g1,125:11938249,32998975
(1,125:11938249,32998975:1148181,477213,0
x1,125:13086430,32998975
)
g1,125:13265834,32998975
x1,125:17487530,32998975
g1,125:17666934,32998975
x1,125:18889742,32998975
g1,125:19069146,32998975
x1,125:21450883,32998975
g1,125:21630287,32998975
x1,125:23463063,32998975
g1,125:23642467,32998975
x1,125:24945648,32998975
x1,125:25813957,32998975
g1,125:25993361,32998975
x1,125:29636651,32998975
k1,125:31987364,32998975:2350713
k1,125:34338077,32998975:2350713
)
(1,128:5920357,34458944:28417720,489408,155358
x1,128:8863363,34458944
k1,126:9098950,34458944:235587
x1,126:9993406,34458944
k1,126:10228993,34458944:235587
x1,126:10553983,34458944
x1,126:10905619,34458944
x1,126:13490514,34458944
k1,126:13726101,34458944:235587
x1,126:14335829,34458944
k1,126:14571416,34458944:235587
x1,126:17417288,34458944
k1,126:17652875,34458944:235587
x1,126:21393186,34458944
k1,126:21628773,34458944:235587
x1,126:23031211,34458944
k1,126:23280844,34458944:249633
x1,126:26411446,34458944
k1,126:26647033,34458944:235587
x1,126:29777634,34458944
k1,126:30013221,34458944:235587
x1,126:31029186,34458944
k1,126:31264773,34458944:235587
x1,126:31955748,34458944
k1,126:32191335,34458944:235587
x1,126:33533024,34458944
k1,126:33768611,34458944:235587
x1,126:34338077,34458944
k1,126:34338077,34458944:0
)
(1,128:5920357,35350234:28417720,489408,155358
x1,128:7442804,35350234
x1,126:7792649,35350234
x1,126:8342261,35350234
k1,126:8521945,35350234:179684
x1,126:10805250,35350234
k1,126:10984933,35350234:179683
x1,126:13949043,35350234
k1,126:14128727,35350234:179684
x1,126:14689818,35350234
k1,126:14869501,35350234:179683
x1,126:17152823,35350234
k1,126:17332507,35350234:179684
x1,126:18373924,35350234
k1,126:18553607,35350234:179683
x1,126:21517735,35350234
k1,126:21697419,35350234:179684
x1,126:23700166,35350234
k1,126:23879849,35350234:179683
x1,126:24480611,35350234
k1,126:24660295,35350234:179684
x1,126:28285745,35350234
k1,126:28509043,35350234:223298
x1,126:29630513,35350234
k1,126:29810197,35350234:179684
x1,126:31252591,35350234
k1,126:31432274,35350234:179683
x1,126:32473691,35350234
x1,126:34338077,35350234
k1,126:34338077,35350234:0
)
(1,128:5920357,36241524:28417720,489408,155358
x1,128:6515141,36241524
k1,126:6693778,36241524:178637
x1,126:8161087,36241524
k1,126:8339725,36241524:178638
x1,126:10759548,36241524
k1,126:10938185,36241524:178637
x1,126:11414429,36241524
k1,126:11593067,36241524:178638
x1,126:12664095,36241524
k1,126:12842732,36241524:178637
x1,126:13715266,36241524
x1,126:14061523,36241524
k1,126:14240161,36241524:178638
x1,126:14914201,36241524
x1,126:15256867,36241524
x1,126:15563134,36241524
k1,126:15741771,36241524:178637
x1,126:16297280,36241524
x1,126:16794866,36241524
k1,126:16973504,36241524:178638
x1,126:17211273,36241524
x1,126:18314392,36241524
k1,126:18493029,36241524:178637
x1,126:20080291,36241524
x1,126:20419365,36241524
x1,126:20725632,36241524
k1,126:20904270,36241524:178638
x1,126:23164866,36241524
k1,126:23343503,36241524:178637
x1,126:26754374,36241524
k1,126:26933012,36241524:178638
x1,126:30026160,36241524
k1,126:30204797,36241524:178637
x1,126:30799572,36241524
k1,126:30978210,36241524:178638
x1,126:33000322,36241524
k1,126:33178959,36241524:178637
x1,126:34427779,36241524
k1,126:34338077,36241524:0
)
(1,128:5920357,37132814:28417720,489408,155358
x1,128:7415685,37132814
k1,126:7594367,37132814:178682
x1,126:8483562,37132814
k1,126:8662244,37132814:178682
x1,126:10481387,37132814
k1,126:10660068,37132814:178681
x1,126:11670058,37132814
k1,126:11848740,37132814:178682
x1,126:13303323,37132814
k1,126:13482005,37132814:178682
x1,126:14371200,37132814
k1,126:14549882,37132814:178682
x1,126:14872961,37132814
x1,126:16843605,37132814
k1,126:17022286,37132814:178681
x1,126:18557647,37132814
k1,126:18736329,37132814:178682
x1,126:21403914,37132814
k1,126:21582596,37132814:178682
x1,126:22633339,37132814
k1,126:22812021,37132814:178682
x1,126:25115774,37132814
k1,126:25294455,37132814:178681
x1,126:25860571,37132814
k1,126:26039253,37132814:178682
x1,126:26928448,37132814
k1,126:27107130,37132814:178682
x1,126:27430209,37132814
x1,126:27779692,37132814
x1,126:29701672,37132814
k1,126:29880354,37132814:178682
x1,126:31274544,37132814
k1,126:31496763,37132814:222219
x1,126:34427779,37132814
k1,126:34338077,37132814:0
)
(1,128:5920357,38024104:28417720,489408,155358
x1,128:6942086,38024104
k1,126:7121577,38024104:179491
x1,126:10659401,38024104
k1,126:10838891,38024104:179490
x1,126:11428296,38024104
k1,126:11607787,38024104:179491
x1,126:12472428,38024104
k1,126:12651918,38024104:179490
x1,126:15678169,38024104
k1,126:15857660,38024104:179491
x1,126:19040289,38024104
k1,126:19219779,38024104:179490
x1,126:19691715,38024104
k1,126:19871206,38024104:179491
x1,126:20932545,38024104
k1,126:21112036,38024104:179491
x1,126:21976677,38024104
k1,126:22156167,38024104:179490
x1,126:24474854,38024104
k1,126:24654345,38024104:179491
x1,126:25243750,38024104
k1,126:25423240,38024104:179490
x1,126:26287881,38024104
k1,126:26467372,38024104:179491
x1,126:28236283,38024104
k1,126:28415773,38024104:179490
x1,126:31008973,38024104
k1,126:31188464,38024104:179491
x1,126:31660400,38024104
k1,126:31839890,38024104:179490
x1,126:33451014,38024104
k1,126:33630505,38024104:179491
x1,126:34338077,38024104
k1,126:34338077,38024104:0
)
(1,128:5920357,38915394:28417720,489408,155358
x1,128:6779737,38915394
k1,126:6956529,38915394:176792
x1,126:8949546,38915394
k1,126:9126338,38915394:176792
x1,126:9438584,38915394
x1,126:9775868,38915394
x1,126:11632801,38915394
k1,126:11809593,38915394:176792
x1,126:13293475,38915394
k1,126:13470267,38915394:176792
x1,126:15715774,38915394
k1,126:15893088,38915394:177314
x1,126:18431148,38915394
k1,126:18607940,38915394:176792
x1,126:18998942,38915394
k1,126:19175734,38915394:176792
x1,126:20817136,38915394
k1,126:20993928,38915394:176792
x1,126:21892695,38915394
k1,126:22069487,38915394:176792
x1,126:22733366,38915394
k1,126:22910158,38915394:176792
x1,126:25800537,38915394
k1,126:25977329,38915394:176792
x1,126:26524463,38915394
k1,126:26701255,38915394:176792
x1,126:29552967,38915394
k1,126:29729759,38915394:176792
x1,126:30433025,38915394
x1,126:30773900,38915394
x1,126:31270889,38915394
k1,126:31447681,38915394:176792
x1,126:34338077,38915394
k1,126:34338077,38915394:0
)
(1,128:5920357,39806684:28417720,489408,155358
x1,128:7248115,39806684
x1,126:8640281,39806684
k1,126:8802810,39806684:162529
x1,126:9857691,39806684
k1,126:10020219,39806684:162528
x1,126:11231232,39806684
k1,126:11393761,39806684:162529
x1,126:12292528,39806684
k1,126:12455056,39806684:162528
x1,126:13118935,39806684
x1,126:13456219,39806684
x1,126:13757707,39806684
k1,126:13920236,39806684:162529
x1,126:15247994,39806684
k1,126:15410522,39806684:162528
x1,126:16660210,39806684
k1,126:16822739,39806684:162529
x1,126:17369873,39806684
k1,126:17532401,39806684:162528
x1,126:18391781,39806684
k1,126:18554310,39806684:162529
x1,126:19863069,39806684
k1,126:20079904,39806684:216835
x1,126:21330296,39806684
k1,126:21492824,39806684:162528
x1,126:23134226,39806684
k1,126:23296755,39806684:162529
x1,126:24468381,39806684
k1,126:24630909,39806684:162528
x1,126:25178043,39806684
k1,126:25340572,39806684:162529
x1,126:25652818,39806684
k1,126:25815346,39806684:162528
x1,126:27065746,39806684
k1,126:27228275,39806684:162529
x1,126:27462460,39806684
x1,126:28548841,39806684
k1,126:28711369,39806684:162528
x1,126:29375248,39806684
x1,126:29716123,39806684
x1,126:30415787,39806684
x1,126:30749479,39806684
x1,126:31050967,39806684
k1,126:31213496,39806684:162529
x1,126:34338077,39806684
k1,126:34338077,39806684:0
)
(1,128:5920357,40697974:28417720,489408,155358
x1,128:9392932,40697974
k1,126:9571428,40697974:178496
x1,126:12720534,40697974
k1,126:12899030,40697974:178496
x1,126:13423874,40697974
x1,126:16038075,40697974
k1,126:16216572,40697974:178497
x1,126:17306247,40697974
k1,126:17484743,40697974:178496
x1,126:18050301,40697974
k1,126:18228797,40697974:178496
x1,126:19117115,40697974
k1,126:19295611,40697974:178496
x1,126:20829461,40697974
k1,126:21007958,40697974:178497
x1,126:23713626,40697974
k1,126:23892122,40697974:178496
x1,126:26093284,40697974
k1,126:26315441,40697974:222157
x1,126:28051374,40697974
k1,126:28229870,40697974:178496
x1,126:30693469,40697974
k1,126:30871966,40697974:178497
x1,126:32043059,40697974
k1,126:32221555,40697974:178496
x1,126:33594023,40697974
k1,126:33772519,40697974:178496
x1,126:34338077,40697974
k1,126:34338077,40697974:0
)
(1,128:5920357,41589264:28417720,489408,155358
x1,128:7133825,41589264
k1,126:7312543,41589264:178718
x1,126:8607590,41589264
k1,126:8786307,41589264:178717
x1,126:9676378,41589264
k1,126:9855096,41589264:178718
x1,126:12646223,41589264
k1,126:12824941,41589264:178718
x1,126:13431680,41589264
k1,126:13610397,41589264:178717
x1,126:16846565,41589264
k1,126:17025283,41589264:178718
x1,126:18441226,41589264
k1,126:18619944,41589264:178718
x1,126:20217982,41589264
k1,126:20396837,41589264:178855
x1,126:21003567,41589264
k1,126:21182284,41589264:178717
x1,126:23488325,41589264
k1,126:23667043,41589264:178718
x1,126:27146470,41589264
k1,126:27325188,41589264:178718
x1,126:30035466,41589264
k1,126:30214183,41589264:178717
x1,126:30456731,41589264
x1,126:31015501,41589264
k1,126:31194219,41589264:178718
x1,126:34350277,41589264
k1,126:34338077,41589264:0
)
(1,128:5920357,42480554:28417720,489408,8247
x1,128:6797275,42480554
g1,126:6976679,42480554
x1,126:9926061,42480554
g1,127:10105465,42480554
x1,127:11600251,42480554
k1,128:34338076,42480554:22863408
g1,128:34338076,42480554
)
(1,130:5920357,43561613:28417720,489408,155358
h1,129:5920357,43561613:1114112,0,0
x1,129:8741410,43561613
k1,129:8932877,43561613:191467
x1,129:9421087,43561613
k1,129:9612555,43561613:191468
x1,129:9937545,43561613
k1,129:10129012,43561613:191467
x1,129:10901226,43561613
x1,129:11579288,43561613
k1,129:11770755,43561613:191467
x1,129:14006909,43561613
k1,129:14198377,43561613:191468
x1,129:14808105,43561613
k1,129:14999572,43561613:191467
x1,129:17032952,43561613
k1,129:17224419,43561613:191467
x1,129:18322356,43561613
k1,129:18513824,43561613:191468
x1,129:18838814,43561613
x1,129:21227429,43561613
k1,129:21418896,43561613:191467
x1,129:22313352,43561613
k1,129:22504819,43561613:191467
x1,129:24863198,43561613
k1,129:25054666,43561613:191468
x1,129:25664394,43561613
k1,129:25855861,43561613:191467
x1,129:28986463,43561613
k1,129:29177930,43561613:191467
(1,129:29177930,43561613:1076420,479368,0
x1,129:30254350,43561613
)
k1,129:30445818,43561613:191468
x1,129:33577144,43561613
k1,129:33768611,43561613:191467
x1,129:34338077,43561613
k1,129:34338077,43561613:0
)
(1,130:5920357,44452903:28417720,494436,155358
x1,130:7873302,44452903
k1,129:8030710,44452903:157408
x1,129:8890090,44452903
k1,129:9047498,44452903:157408
x1,129:10648810,44452903
k1,129:10806218,44452903:157408
x1,129:12016528,44452903
k1,129:12173936,44452903:157408
x1,129:15064332,44452903
k1,129:15221740,44452903:157408
x1,129:16237234,44452903
x1,129:17919054,44452903
k1,129:18134182,44452903:215128
(1,129:18134182,44452903:0,0,0
(1,129:18134182,43561613:0,0,0
)
)
x1,129:20566156,44452903
k1,129:20723564,44452903:157408
x1,129:22237727,44452903
x1,129:24059015,44452903
k1,129:24216423,44452903:157408
x1,129:24455387,44452903
(1,129:24455387,44452903:996764,482592,0
x1,129:25452151,44452903
)
x1,129:25691115,44452903
k1,129:25848523,44452903:157408
x1,129:26317587,44452903
k1,129:26474995,44452903:157408
x1,129:26787241,44452903
k1,129:26944649,44452903:157408
x1,129:29093113,44452903
k1,129:29250521,44452903:157408
x1,129:31360283,44452903
k1,129:31517691,44452903:157408
x1,129:34427779,44452903
k1,129:34338077,44452903:0
)
(1,130:5920357,45344193:28417720,489408,155358
x1,130:7683444,45344193
k1,129:7894664,45344193:211220
x1,129:8870368,45344193
k1,129:9081589,45344193:211221
x1,129:10463539,45344193
k1,129:10674759,45344193:211220
x1,129:11690724,45344193
x1,129:12815307,45344193
k1,129:13026528,45344193:211221
x1,129:14368217,45344193
k1,129:14579437,45344193:211220
x1,129:15148903,45344193
k1,129:15360123,45344193:211220
x1,129:17068503,45344193
k1,129:17279724,45344193:211221
x1,129:18824170,45344193
k1,129:19035390,45344193:211220
x1,129:21718758,45344193
k1,129:21929978,45344193:211220
x1,129:24146350,45344193
k1,129:24464260,45344193:317910
x1,129:27229627,45344193
k1,129:27440847,45344193:211220
x1,129:28945022,45344193
k1,129:29156242,45344193:211220
x1,129:31636863,45344193
k1,129:31848084,45344193:211221
x1,129:32741807,45344193
k1,129:32953027,45344193:211220
x1,129:34457202,45344193
k1,130:34338077,45344193:0
)
(1,130:5920357,46235483:28417720,489408,155358
x1,130:9356202,46235483
k1,129:9569766,46235483:213564
x1,129:10870460,46235483
k1,129:11077192,46235483:206732
x1,129:11646658,46235483
k1,129:11853390,46235483:206732
x1,129:14984715,46235483
k1,129:15191447,46235483:206732
x1,129:16248407,46235483
k1,129:16455139,46235483:206732
x1,129:17146114,46235483
x1,129:17497750,46235483
x1,129:17811982,46235483
k1,129:18018714,46235483:206732
x1,129:19279146,46235483
k1,129:19485879,46235483:206733
x1,129:22738705,46235483
k1,129:22945437,46235483:206732
x1,129:24978826,46235483
k1,129:25185558,46235483:206732
x1,129:26486985,46235483
k1,129:26693717,46235483:206732
x1,129:28238163,46235483
k1,129:28444895,46235483:206732
x1,129:31311255,46235483
k1,129:31524819,46235483:213564
x1,129:32419275,46235483
x1,129:32774502,46235483
k1,129:32981234,46235483:206732
x1,129:33672209,46235483
x1,129:34023845,46235483
x1,129:34338077,46235483
k1,129:34338077,46235483:0
)
]
(1,131:5920357,48201563:28417720,446948,0
(1,131:5920357,48201563:28417720,446948,0
k1,131:19965377,48201563:14045020
x1,131:20293057,48201563
k1,131:34338077,48201563:14045020
)
)
]
]
]
!39623
}2
!10
{3
[1,160:4736286,48201563:29601791,43465277,9168
[1,160:4736286,4736286:0,0,0
(1,160:4736286,2302362:0,0,0
k1,160:4736286,2302362:-1118290
)
]
[1,160:4736286,48201563:29601791,43465277,9168
h1,160:4736286,4736286:0,0,0
[1,160:5920357,48201563:28417720,45833420,9168
[1,160:5920357,3154575:28417720,786432,0
(1,160:5920357,3154575:28417720,444988,8188
(1,160:5920357,3154575:28417720,444988,8188
k1,160:13171428,3154575:7251071
x1,160:15265284,3154575
x1,160:16743097,3154575
g1,160:16906937,3154575
x1,160:19925480,3154575
g1,160:20089320,3154575
x1,160:21006160,3154575
x1,160:23981443,3154575
g1,160:24145283,3154575
x1,160:25262002,3154575
g1,160:25425842,3154575
x1,160:26907602,3154575
g1,160:27087006,3154575
k1,160:34338077,3154575:7251071
)
)
]
[1,160:5920357,46235483:28417720,40258437,0
(1,130:5920357,6697942:28417720,489408,155358
x1,130:7972350,6697942
k1,129:8151684,6697942:179334
x1,129:8875760,6697942
x1,129:9943201,6697942
k1,129:10122535,6697942:179334
x1,129:11690878,6697942
k1,129:11870212,6697942:179334
x1,129:14001870,6697942
k1,129:14181204,6697942:179334
x1,129:15468595,6697942
k1,129:15647929,6697942:179334
x1,129:16975158,6697942
x1,129:18623855,6697942
k1,129:18803189,6697942:179334
x1,129:20190504,6697942
k1,129:20369852,6697942:179348
x1,129:22139481,6697942
k1,129:22318815,6697942:179334
x1,129:23565664,6697942
x1,129:24161633,6697942
k1,129:24340967,6697942:179334
x1,129:25789102,6697942
k1,129:25968436,6697942:179334
x1,129:28945076,6697942
k1,129:29124410,6697942:179334
x1,129:29968678,6697942
k1,129:30148012,6697942:179334
x1,129:32279671,6697942
x1,129:32630951,6697942
k1,129:32810285,6697942:179334
x1,129:34338077,6697942
k1,129:34338077,6697942:0
)
(1,130:5920357,7589232:28417720,489408,155358
x1,130:8551111,7589232
g1,129:8730515,7589232
x1,129:11580865,7589232
k1,130:34338078,7589232:22882796
g1,130:34338078,7589232
)
(1,132:5920357,8781002:28417720,494436,155358
h1,131:5920357,8781002:1114112,0,0
(1,131:7034469,8781002:0,0,0
(1,131:7034469,7889712:0,0,0
)
)
x1,131:8309660,8781002
x1,131:9785060,8781002
k1,131:9963957,8781002:178897
x1,131:11199684,8781002
x1,131:12076602,8781002
k1,131:12255499,8781002:178897
x1,131:13331199,8781002
x1,131:13849317,8781002
x1,131:14918560,8781002
k1,131:15097458,8781002:178898
x1,131:15336422,8781002
(1,131:15336422,8781002:1554354,494436,13271
x1,131:16890776,8781002
)
x1,131:17129740,8781002
x1,131:17405257,8781002
k1,131:17584154,8781002:178897
x1,131:18448963,8781002
k1,131:18627860,8781002:178897
x1,131:20083379,8781002
k1,131:20262276,8781002:178897
x1,131:21324708,8781002
x1,131:21678852,8781002
x1,131:22426083,8781002
k1,131:22604981,8781002:178898
x1,131:24021541,8781002
x1,131:25005346,8781002
k1,131:25184243,8781002:178897
x1,131:26246659,8781002
k1,131:26425556,8781002:178897
x1,131:27094176,8781002
x1,131:27433971,8781002
x1,131:27737689,8781002
k1,131:27916586,8781002:178897
x1,131:29253826,8781002
k1,131:29432724,8781002:178898
x1,131:30101344,8781002
x1,131:31517904,8781002
k1,131:31696801,8781002:178897
x1,131:32522659,8781002
k1,131:32701556,8781002:178897
x1,131:33331217,8781002
x1,131:33999837,8781002
x1,131:34235694,8781002
x1,131:34457202,8781002
k1,132:34338077,8781002:0
)
(1,132:5920357,9672292:28417720,489408,155358
x1,132:7447587,9672292
k1,131:7630733,9672292:183146
x1,131:9297403,9672292
k1,131:9480549,9672292:183146
x1,131:10740257,9672292
k1,131:10923403,9672292:183146
x1,131:12467849,9672292
k1,131:12650995,9672292:183146
x1,131:13341970,9672292
x1,131:14195431,9672292
x1,131:15517355,9672292
k1,131:15751041,9672292:233686
x1,131:16970496,9672292
x1,131:17742710,9672292
k1,131:17925857,9672292:183147
x1,131:18820313,9672292
x1,131:19348793,9672292
x1,131:20602060,9672292
k1,131:20785206,9672292:183146
x1,131:21678929,9672292
k1,131:21862075,9672292:183146
x1,131:23732977,9672292
k1,131:23916123,9672292:183146
x1,131:25298073,9672292
x1,131:25705035,9672292
x1,131:26053079,9672292
x1,131:26367311,9672292
k1,131:26550457,9672292:183146
x1,131:27119923,9672292
k1,131:27303069,9672292:183146
x1,131:28563510,9672292
x1,131:29457966,9672292
x1,131:29813193,9672292
k1,131:29996339,9672292:183146
x1,131:31215785,9672292
k1,131:31398931,9672292:183146
x1,131:32821859,9672292
x1,131:34427779,9672292
k1,131:34338077,9672292:0
)
(1,132:5920357,10563582:28417720,489408,155358
x1,132:6652327,10563582
x1,132:7162866,10563582
x1,132:7487856,10563582
x1,132:7835900,10563582
x1,132:8393875,10563582
x1,132:8548169,10563582
k1,131:8740632,10563582:192463
x1,131:9635088,10563582
x1,131:9990315,10563582
k1,131:10180167,10563582:189852
x1,131:10748900,10563582
x1,131:12253084,10563582
k1,131:12442935,10563582:189851
x1,131:13744371,10563582
k1,131:13934223,10563582:189852
x1,131:15194664,10563582
x1,131:15926634,10563582
x1,131:16455105,10563582
x1,131:18122508,10563582
k1,131:18312359,10563582:189851
x1,131:19044329,10563582
x1,131:20123601,10563582
k1,131:20313453,10563582:189852
x1,131:21166924,10563582
k1,131:21356776,10563582:189852
x1,131:22698456,10563582
x1,131:23816899,10563582
k1,131:24009362,10563582:192463
x1,131:25066322,10563582
k1,131:25256173,10563582:189851
x1,131:26150629,10563582
x1,131:26505856,10563582
k1,131:26695708,10563582:189852
x1,131:27589431,10563582
k1,131:27779282,10563582:189851
x1,131:29445970,10563582
k1,131:29635822,10563582:189852
x1,131:30205288,10563582
k1,131:30395139,10563582:189851
x1,131:30964605,10563582
x1,131:31818066,10563582
k1,131:32007918,10563582:189852
x1,131:33146850,10563582
x1,131:34427779,10563582
k1,131:34338077,10563582:0
)
(1,132:5920357,11454872:28417720,489408,155358
x1,132:6279166,11454872
x1,132:6627217,11454872
x1,132:6935077,11454872
x1,132:7174041,11454872
x1,132:7772523,11454872
x1,132:8889123,11454872
g1,131:9068527,11454872
x1,131:10104763,11454872
g1,131:10284167,11454872
x1,131:11978444,11454872
k1,132:34338077,11454872:22485216
g1,132:34338077,11454872
)
(1,137:5920357,12646642:28417720,494436,155358
h1,134:5920357,12646642:1114112,0,0
(1,134:7034469,12646642:0,0,0
(1,134:7034469,11755352:0,0,0
)
)
x1,134:9546824,12646642
k1,134:9759139,12646642:212315
x1,134:10277257,12646642
x1,134:11759121,12646642
k1,134:11971435,12646642:212314
x1,134:14642381,12646642
k1,134:14854696,12646642:212315
x1,134:15093660,12646642
(1,134:15093660,12646642:1594537,494436,13271
x1,134:16688197,12646642
)
x1,134:16927161,12646642
k1,134:17139475,12646642:212314
x1,134:17627685,12646642
k1,134:17840000,12646642:212315
x1,134:20035159,12646642
k1,134:20247473,12646642:212314
x1,134:22483627,12646642
k1,134:22695942,12646642:212315
x1,134:24891834,12646642
k1,134:25104148,12646642:212314
x1,134:26202085,12646642
k1,134:26414400,12646642:212315
x1,134:27390104,12646642
k1,134:27602418,12646642:212314
x1,134:28984368,12646642
k1,134:29196683,12646642:212315
x1,134:31189085,12646642
k1,134:31401399,12646642:212314
x1,134:33556296,12646642
k1,134:33768611,12646642:212315
x1,134:34338077,12646642
k1,134:34338077,12646642:0
)
(1,137:5920357,13537932:28417720,489408,155358
x1,137:7668274,13537932
k1,134:7917594,13537932:249320
x1,134:9746769,13537932
k1,134:9996089,13537932:249320
x1,134:10565555,13537932
k1,134:10814876,13537932:249321
x1,134:11709332,13537932
k1,134:11958652,13537932:249320
x1,134:13625322,13537932
k1,134:13874642,13537932:249320
x1,134:15134350,13537932
k1,134:15383670,13537932:249320
x1,134:17783044,13537932
x1,134:17919397,13537932
k1,134:18351606,13537932:432209
(1,134:18351606,13537932:1555065,489408,10039
x1,134:19906671,13537932
)
x1,134:20191400,13537932
k1,134:20440720,13537932:249320
x1,134:21131695,13537932
x1,134:21483331,13537932
x1,134:21797563,13537932
k1,134:22046883,13537932:249320
x1,134:23428833,13537932
k1,134:23678154,13537932:249321
x1,134:24653867,13537932
x1,134:25009094,13537932
x1,134:25689311,13537932
k1,134:25938631,13537932:249320
x1,134:26508097,13537932
k1,134:26757417,13537932:249320
x1,134:27448392,13537932
k1,134:27697712,13537932:249320
x1,134:30706063,13537932
k1,134:30955384,13537932:249321
x1,134:31524850,13537932
k1,134:31774170,13537932:249320
x1,134:32099160,13537932
k1,134:32348480,13537932:249320
x1,134:32714465,13537932
x1,134:34363194,13537932
k1,134:34338077,13537932:0
)
(1,137:5920357,14429222:28417720,489408,155358
x1,137:6530085,14429222
k1,134:6750611,14429222:220526
x1,134:8377011,14429222
x1,134:10572894,14429222
k1,134:10793421,14429222:220527
x1,134:12257335,14429222
k1,134:12477861,14429222:220526
x1,134:15243219,14429222
k1,134:15463745,14429222:220526
x1,134:17008191,14429222
k1,134:17228717,14429222:220526
x1,134:20095077,14429222
k1,134:20440904,14429222:345827
x1,134:21579112,14429222
k1,134:21799638,14429222:220526
x1,134:24158017,14429222
k1,134:24378544,14429222:220527
x1,134:24988272,14429222
k1,134:25208798,14429222:220526
x1,134:27079693,14429222
k1,134:27300219,14429222:220526
x1,134:29170379,14429222
k1,134:29390905,14429222:220526
x1,134:30813842,14429222
k1,134:31034369,14429222:220527
x1,134:31766330,14429222
x1,134:32125140,14429222
k1,134:32345666,14429222:220526
x1,134:34338077,14429222
k1,134:34338077,14429222:0
)
(1,137:5920357,15320512:28417720,489408,155358
x1,137:8146162,15320512
k1,134:8326329,15320512:180167
x1,134:9185709,15320512
x1,134:9526584,15320512
k1,134:9706751,15320512:180167
x1,134:11992331,15320512
k1,134:12217081,15320512:224750
x1,134:13506842,15320512
k1,134:13687009,15320512:180167
x1,134:14156073,15320512
k1,134:14336240,15320512:180167
x1,134:15625306,15320512
k1,134:15805473,15320512:180167
x1,134:18579114,15320512
k1,134:18759282,15320512:180168
x1,134:19306416,15320512
k1,134:19486583,15320512:180167
x1,134:19994339,15320512
x1,134:20924615,15320512
k1,134:21104782,15320512:180167
x1,134:21651916,15320512
k1,134:21832083,15320512:180167
x1,134:23082483,15320512
k1,134:23262650,15320512:180167
x1,134:26700874,15320512
k1,134:26881041,15320512:180167
x1,134:28833283,15320512
k1,135:29013451,15320512:180168
x1,135:30848948,15320512
k1,135:31029115,15320512:180167
x1,135:33178273,15320512
k1,135:33358440,15320512:180167
x1,135:34022319,15320512
x1,135:34363194,15320512
k1,135:34338077,15320512:0
)
(1,137:5920357,16211802:28417720,489408,155358
x1,137:8733385,16211802
k1,135:8897894,16211802:164509
x1,135:12921935,16211802
k1,135:13086444,16211802:164509
x1,135:15156837,16211802
x1,135:16240347,16211802
x1,135:16369524,16211802
k1,135:16587019,16211802:217495
x1,135:17837411,16211802
k1,135:18001920,16211802:164509
x1,135:18470984,16211802
k1,135:18635494,16211802:164510
x1,135:20119366,16211802
x1,135:20453058,16211802
x1,135:21106179,16211802
k1,135:21270688,16211802:164509
x1,135:21973954,16211802
k1,135:22138463,16211802:164509
x1,135:23662426,16211802
k1,135:23826935,16211802:164509
x1,135:24178568,16211802
x1,135:25577204,16211802
k1,135:25741713,16211802:164509
x1,135:28359241,16211802
k1,135:28523750,16211802:164509
x1,135:29070884,16211802
k1,135:29235394,16211802:164510
x1,135:30446407,16211802
k1,135:30610916,16211802:164509
x1,135:31470296,16211802
k1,135:31634805,16211802:164509
x1,135:32806431,16211802
k1,135:32970940,16211802:164509
x1,135:34338077,16211802
k1,135:34338077,16211802:0
)
(1,137:5920357,17103092:28417720,489408,155358
x1,137:7231785,17103092
k1,135:7410391,17103092:178606
x1,135:9636178,17103092
k1,135:9814784,17103092:178606
x1,135:11285769,17103092
k1,135:11464375,17103092:178606
x1,135:13053403,17103092
k1,135:13232010,17103092:178607
x1,135:13788636,17103092
k1,135:13967242,17103092:178606
x1,135:14284904,17103092
k1,135:14463510,17103092:178606
x1,135:15735602,17103092
k1,135:15914208,17103092:178606
x1,135:19412077,17103092
k1,135:19590683,17103092:178606
x1,135:21576789,17103092
k1,135:21755395,17103092:178606
x1,135:23523289,17103092
k1,135:23702055,17103092:178766
x1,135:26006549,17103092
k1,135:26185155,17103092:178606
x1,135:27059443,17103092
k1,135:27238050,17103092:178607
x1,135:29860906,17103092
k1,135:30039512,17103092:178606
x1,135:30913083,17103092
k1,135:31091689,17103092:178606
x1,135:32561956,17103092
k1,135:32740562,17103092:178606
x1,135:33496081,17103092
x1,135:34363194,17103092
k1,135:34338077,17103092:0
)
(1,137:5920357,17994382:28417720,489408,155358
x1,137:6481448,17994382
k1,135:6661547,17994382:180099
x1,135:7342361,17994382
k1,136:7522460,17994382:180099
x1,136:9725711,17994382
k1,136:9905811,17994382:180100
x1,136:12809351,17994382
k1,136:13033896,17994382:224545
x1,136:14316185,17994382
k1,136:14496285,17994382:180100
x1,136:16939714,17994382
k1,136:17119813,17994382:180099
x1,136:17720575,17994382
k1,136:17900674,17994382:180099
(1,136:17900674,17994382:1555065,489408,10039
x1,136:19455739,17994382
)
x1,136:19736281,17994382
k1,136:19916380,17994382:180099
x1,136:22079249,17994382
k1,136:22259348,17994382:180099
x1,136:24383278,17994382
k1,136:24563378,17994382:180100
x1,136:25885346,17994382
x1,136:27527506,17994382
k1,136:27707605,17994382:180099
x1,136:29310087,17994382
x1,136:31473677,17994382
k1,136:31653776,17994382:180099
x1,136:34338077,17994382
k1,136:34338077,17994382:0
)
(1,137:5920357,18885672:28417720,489408,155358
x1,137:6662992,18885672
x1,136:6968063,18885672
k1,136:7137437,18885672:169374
x1,136:7996817,18885672
k1,136:8166191,18885672:169374
x1,136:9455266,18885672
k1,136:9624639,18885672:169373
x1,136:11538901,18885672
k1,136:11708275,18885672:169374
x1,136:12255409,18885672
k1,136:12424783,18885672:169374
x1,136:13908665,18885672
k1,136:14078039,18885672:169374
x1,136:16831995,18885672
k1,136:17051111,18885672:219116
x1,136:19355698,18885672
k1,136:19525072,18885672:169374
x1,136:21791652,18885672
x1,136:22125344,18885672
x1,136:22426832,18885672
k1,136:22596206,18885672:169374
x1,136:24080773,18885672
x1,136:24925804,18885672
k1,136:25095177,18885672:169373
x1,136:25680995,18885672
k1,136:25850369,18885672:169374
(1,136:25850369,18885672:1555065,489408,10039
x1,136:27405434,18885672
)
x1,136:27678997,18885672
k1,136:27848371,18885672:169374
x1,136:28317435,18885672
k1,136:28486809,18885672:169374
x1,136:29346189,18885672
k1,136:29515562,18885672:169373
x1,136:30023318,18885672
x1,136:30680022,18885672
k1,136:30849396,18885672:169374
x1,136:31708776,18885672
x1,136:32049651,18885672
k1,136:32219025,18885672:169374
x1,136:33702897,18885672
x1,136:34036589,18885672
x1,136:34338077,18885672
k1,136:34338077,18885672:0
)
(1,137:5920357,19776962:28417720,489408,155358
x1,137:7728735,19776962
k1,136:7907719,19776962:178984
x1,136:10520454,19776962
k1,136:10699437,19776962:178983
x1,136:11985553,19776962
k1,136:12164537,19776962:178984
x1,136:13611253,19776962
k1,136:13790236,19776962:178983
x1,136:17888011,19776962
k1,136:18066995,19776962:178984
x1,136:21902933,19776962
k1,136:22125253,19776962:222320
x1,136:24274339,19776962
k1,136:24453406,19776962:179067
x1,136:25498638,19776962
k1,136:25677622,19776962:178984
x1,136:28128344,19776962
k1,136:28307327,19776962:178983
x1,136:28789793,19776962
k1,136:28968777,19776962:178984
x1,136:30013302,19776962
k1,136:30192285,19776962:178983
x1,136:30755051,19776962
k1,136:30934035,19776962:178984
x1,136:31817968,19776962
k1,136:31996951,19776962:178983
x1,136:32237827,19776962
x1,136:33074073,19776962
k1,136:33253057,19776962:178984
x1,136:34338077,19776962
k1,136:34338077,19776962:0
)
(1,137:5920357,20668252:28417720,489408,155358
x1,137:6806044,20668252
k1,136:6984368,20668252:178324
x1,136:10648877,20668252
k1,136:10827201,20668252:178324
x1,136:13242919,20668252
k1,136:13421243,20668252:178324
x1,136:13985126,20668252
k1,136:14163451,20668252:178325
x1,136:15210757,20668252
k1,136:15389081,20668252:178324
x1,136:17079280,20668252
x1,136:17584638,20668252
x1,136:18724809,20668252
k1,136:18903349,20668252:178540
x1,136:21923515,20668252
k1,136:22101839,20668252:178324
x1,136:22786040,20668252
k1,136:22964364,20668252:178324
x1,136:24614713,20668252
k1,136:24793037,20668252:178324
x1,136:26605022,20668252
k1,136:26783347,20668252:178325
x1,136:27387098,20668252
k1,136:27565422,20668252:178324
x1,136:28451109,20668252
k1,136:28629433,20668252:178324
x1,136:32735339,20668252
k1,136:32913663,20668252:178324
x1,136:34321926,20668252
x1,136:34463660,20668252
k1,136:34338077,20668252:0
)
(1,137:5920357,21559542:28417720,489408,155358
x1,137:7174021,21559542
g1,136:7353425,21559542
x1,136:9784698,21559542
g1,136:9964102,21559542
x1,136:11199829,21559542
x1,136:11790418,21559542
g1,136:11969822,21559542
(1,136:11969822,21559542:1555065,489408,10039
x1,136:13524887,21559542
)
g1,136:13704291,21559542
x1,136:15178982,21559542
g1,136:15358386,21559542
x1,136:16314968,21559542
x1,136:17138065,21559542
g1,136:17317469,21559542
x1,136:17875769,21559542
g1,136:18055173,21559542
x1,136:18733301,21559542
g1,136:18912705,21559542
x1,136:21822614,21559542
g1,136:22002018,21559542
x1,136:23337486,21559542
k1,137:34338077,21559542:11126174
g1,137:34338077,21559542
)
(1,140:5920357,22751313:28417720,494436,155358
h1,138:5920357,22751313:1114112,0,0
(1,138:7034469,22751313:0,0,0
(1,138:7034469,21860023:0,0,0
)
)
x1,138:9625751,22751313
k1,138:9874666,22751313:248915
x1,138:10353312,22751313
x1,138:10618826,22751313
x1,138:11243149,22751313
k1,138:11492063,22751313:248914
x1,138:11731027,22751313
(1,138:11731027,22751313:996764,482592,0
x1,138:12727791,22751313
)
x1,138:12966755,22751313
k1,138:13215670,22751313:248915
x1,138:13703880,22751313
k1,138:13952794,22751313:248914
x1,138:16147953,22751313
k1,138:16396868,22751313:248915
x1,138:17657309,22751313
k1,138:17906223,22751313:248914
x1,138:18515951,22751313
k1,138:18764866,22751313:248915
x1,138:20391266,22751313
x1,138:21366970,22751313
x1,138:21521264,22751313
k1,138:21787556,22751313:266292
x1,138:23576477,22751313
k1,138:23825391,22751313:248914
x1,138:24801095,22751313
k1,138:25050010,22751313:248915
x1,138:26431960,22751313
k1,138:26680874,22751313:248914
x1,138:28998275,22751313
k1,138:29247190,22751313:248915
x1,138:29979160,22751313
k1,138:30228075,22751313:248915
x1,138:33519697,22751313
k1,138:33768611,22751313:248914
x1,138:34338077,22751313
k1,138:34338077,22751313:0
)
(1,140:5920357,23642603:28417720,489408,155358
x1,140:6274143,23642603
x1,138:8265032,23642603
k1,138:8444262,23642603:179230
x1,138:9937229,23642603
k1,138:10116459,23642603:179230
x1,138:12710382,23642603
k1,138:12889612,23642603:179230
x1,138:15110653,23642603
k1,138:15333055,23642603:222402
x1,138:17022719,23642603
k1,138:17201949,23642603:179230
x1,138:19599884,23642603
k1,138:19779114,23642603:179230
x1,138:20643047,23642603
k1,138:20822277,23642603:179230
x1,138:22079615,23642603
k1,138:22258845,23642603:179230
x1,138:22809329,23642603
k1,138:22988559,23642603:179230
x1,138:26192399,23642603
k1,138:26371664,23642603:179265
x1,138:28415813,23642603
k1,138:28595043,23642603:179230
x1,138:29616772,23642603
k1,138:29796002,23642603:179230
x1,138:32900801,23642603
k1,138:33080031,23642603:179230
x1,138:34338077,23642603
k1,138:34338077,23642603:0
)
(1,140:5920357,24533893:28417720,489408,155358
x1,140:6484240,24533893
x1,138:6989598,24533893
k1,138:7168878,24533893:179280
x1,138:11316102,24533893
k1,138:11495382,24533893:179280
x1,138:12220176,24533893
x1,138:13288692,24533893
k1,138:13467973,24533893:179281
x1,138:17151337,24533893
k1,138:17373755,24533893:222418
x1,138:19587968,24533893
k1,138:19767249,24533893:179281
x1,138:20652936,24533893
k1,138:20832216,24533893:179280
x1,138:21557001,24533893
x1,138:23640864,24533893
k1,138:23820144,24533893:179280
x1,138:24866742,24533893
k1,138:25046022,24533893:179280
x1,138:29354132,24533893
k1,138:29533413,24533893:179281
x1,138:30137164,24533893
k1,138:30316444,24533893:179280
(1,138:30316444,24533893:956582,479368,0
x1,138:31273026,24533893
)
x1,138:31736161,24533893
k1,138:31915466,24533893:179305
x1,138:32801153,24533893
x1,138:33152792,24533893
k1,138:33332072,24533893:179280
x1,138:34338077,24533893
k1,138:34338077,24533893:0
)
(1,140:5920357,25425183:28417720,489408,155358
x1,140:6588977,25425183
k1,138:6768490,25425183:179513
x1,138:9129187,25425183
k1,138:9308701,25425183:179514
x1,138:10331465,25425183
k1,138:10510978,25425183:179513
x1,138:12321350,25425183
k1,138:12500864,25425183:179514
x1,138:14311212,25425183
x1,138:14647415,25425183
x1,138:14951133,25425183
k1,138:15130646,25425183:179513
x1,138:15681688,25425183
k1,138:15861202,25425183:179514
x1,138:16490863,25425183
x1,138:16798164,25425183
x1,138:17960225,25425183
k1,138:18139738,25425183:179513
x1,138:19516622,25425183
k1,138:19696136,25425183:179514
x1,138:21506492,25425183
x1,138:23400960,25425183
k1,138:23623748,25425183:222788
x1,138:25138761,25425183
k1,138:25318302,25425183:179541
x1,138:26183820,25425183
k1,138:26363334,25425183:179514
x1,138:28881261,25425183
k1,138:29060774,25425183:179513
x1,138:29650775,25425183
k1,138:29830289,25425183:179514
x1,138:32152728,25425183
k1,138:32332241,25425183:179513
x1,138:34338077,25425183
k1,138:34338077,25425183:0
)
(1,140:5920357,26316473:28417720,489408,155358
x1,140:6916402,26316473
g1,138:7095806,26316473
x1,138:8491552,26316473
x1,138:10644379,26316473
g1,138:10823783,26316473
x1,138:11142401,26316473
x1,138:12439115,26316473
g1,139:12618519,26316473
x1,139:13495437,26316473
g1,139:13674841,26316473
x1,139:14989496,26316473
x1,139:15229178,26316473
g1,139:15408582,26316473
x1,139:17003092,26316473
x1,139:19155919,26316473
g1,139:19335323,26316473
x1,139:23140818,26316473
k1,140:34338077,26316473:11322842
g1,140:34338077,26316473
)
(1,144:5920357,27508243:28417720,489408,155358
h1,143:5920357,27508243:1114112,0,0
x1,143:8172677,27508243
k1,143:8372947,27508243:200270
x1,143:11301507,27508243
k1,143:11501776,27508243:200269
x1,143:12558736,27508243
k1,143:12759006,27508243:200270
x1,143:14629882,27508243
x1,143:15750873,27508243
k1,143:15951142,27508243:200269
x1,143:16560870,27508243
k1,143:16761140,27508243:200270
(1,143:16761140,27508243:956582,479368,0
x1,143:17717722,27508243
)
x1,143:18002451,27508243
k1,143:18202721,27508243:200270
x1,143:18893696,27508243
x1,143:19245332,27508243
x1,143:19559564,27508243
k1,143:19759833,27508243:200269
x1,143:21141783,27508243
k1,143:21342053,27508243:200270
x1,143:24228179,27508243
k1,143:24428449,27508243:200270
x1,143:25160419,27508243
k1,143:25360688,27508243:200269
x1,143:27922565,27508243
k1,143:28122835,27508243:200270
x1,143:30887451,27508243
k1,143:31087720,27508243:200269
x1,143:33568341,27508243
k1,143:33768611,27508243:200270
x1,143:34338077,27508243
k1,143:34338077,27508243:0
)
(1,144:5920357,28399533:28417720,494436,120554
x1,144:7667541,28399533
k1,143:7876072,28399533:208531
x1,143:8201062,28399533
k1,143:8409593,28399533:208531
x1,143:10076264,28399533
k1,143:10284795,28399533:208531
x1,143:10894523,28399533
k1,143:11103055,28399533:208532
x1,143:13339209,28399533
k1,143:13547740,28399533:208531
x1,143:15112665,28399533
k1,143:15422506,28399533:309841
(1,143:15422506,28399533:0,0,0
(1,143:15422506,27508243:0,0,0
)
)
x1,143:18053998,28399533
k1,143:18262529,28399533:208531
x1,143:18700993,28399533
x1,143:19360479,28399533
x1,143:20184294,28399533
k1,143:20392825,28399533:208531
x1,143:20631789,28399533
(1,143:20631789,28399533:956582,482592,0
x1,143:21588371,28399533
)
x1,143:21827335,28399533
k1,143:22035866,28399533:208531
x1,143:22524076,28399533
k1,143:22732608,28399533:208532
x1,143:23423583,28399533
k1,143:23632114,28399533:208531
x1,143:26396730,28399533
k1,143:26605261,28399533:208531
x1,143:27214989,28399533
k1,143:27423520,28399533:208531
x1,143:29863146,28399533
k1,143:30071677,28399533:208531
x1,143:31636602,28399533
k1,143:31852415,28399533:215813
x1,143:33641336,28399533
k1,143:33849867,28399533:208531
x1,143:34338077,28399533
k1,143:34338077,28399533:0
)
(1,144:5920357,29290823:28417720,489408,155358
x1,144:7424541,29290823
k1,143:7622031,29290823:197490
x1,143:8597744,29290823
x1,143:9437590,29290823
k1,143:9635081,29290823:197491
x1,143:10204547,29290823
k1,143:10402037,29290823:197490
x1,143:10768022,29290823
x1,143:11123249,29290823
x1,143:11681224,29290823
x1,143:13430608,29290823
k1,143:13628099,29290823:197491
x1,143:14685059,29290823
k1,143:14882549,29290823:197490
x1,143:16427719,29290823
k1,143:16625209,29290823:197490
x1,143:17194675,29290823
k1,143:17392166,29290823:197491
x1,143:18286622,29290823
k1,143:18484112,29290823:197490
x1,143:19886550,29290823
k1,143:20163270,29290823:276720
x1,143:21728937,29290823
k1,143:21930948,29290823:202011
x1,143:22825404,29290823
x1,143:23180631,29290823
k1,143:23378122,29290823:197491
x1,143:24271845,29290823
k1,143:24469335,29290823:197490
x1,143:29227086,29290823
k1,143:29424577,29290823:197491
x1,143:29749567,29290823
x1,143:31987901,29290823
k1,143:32189913,29290823:202012
x1,143:32799632,29290823
k1,143:32997122,29290823:197490
x1,143:34338077,29290823
k1,143:34338077,29290823:0
)
(1,144:5920357,30182113:28417720,489408,155358
x1,144:7010032,30182113
k1,143:7189506,30182113:179474
x1,143:7674365,30182113
k1,143:7853840,30182113:179475
x1,143:10679457,30182113
k1,143:10858931,30182113:179474
x1,143:14977781,30182113
x1,143:15112878,30182113
k1,143:15335550,30182113:222672
x1,143:16223878,30182113
x1,143:17053551,30182113
x1,143:17399084,30182113
x1,143:17953157,30182113
x1,143:18106195,30182113
k1,143:18285687,30182113:179492
x1,143:19174005,30182113
k1,143:19353479,30182113:179474
x1,143:23026712,30182113
k1,143:23206186,30182113:179474
x1,143:23811731,30182113
k1,143:23991206,30182113:179475
x1,143:25485059,30182113
k1,143:25664533,30182113:179474
x1,143:27764658,30182113
k1,143:27944133,30182113:179475
x1,143:29802197,30182113
k1,143:29981671,30182113:179474
x1,143:32363862,30182113
k1,143:32543337,30182113:179475
x1,143:33270285,30182113
k1,143:33449759,30182113:179474
x1,143:34338077,30182113
k1,143:34338077,30182113:0
)
(1,144:5920357,31073403:28417720,489408,155358
x1,144:8186252,31073403
k1,143:8357359,31073403:171107
x1,143:8943177,31073403
k1,143:9114284,31073403:171107
x1,143:10402655,31073403
k1,143:10573762,31073403:171107
x1,143:11627940,31073403
k1,143:11799046,31073403:171106
x1,143:12384855,31073403
k1,143:12555962,31073403:171107
x1,143:13766966,31073403
k1,143:13938073,31073403:171107
x1,143:14523882,31073403
k1,143:14694989,31073403:171107
x1,143:15554369,31073403
k1,143:15725476,31073403:171107
x1,143:18771986,31073403
k1,143:18943093,31073403:171107
x1,143:21286354,31073403
k1,143:21457460,31073403:171106
x1,143:22961017,31073403
k1,143:23180712,31073403:219695
x1,143:24040101,31073403
x1,143:24575774,31073403
x1,143:26256554,31073403
k1,143:26427661,31073403:171107
x1,143:27403786,31073403
k1,143:27574892,31073403:171106
x1,143:29215582,31073403
k1,143:29386689,31073403:171107
x1,143:30948632,31073403
k1,143:31119739,31073403:171107
x1,143:32643007,31073403
k1,143:32814114,31073403:171107
x1,143:34338077,31073403
k1,143:34338077,31073403:0
)
(1,144:5920357,31964693:28417720,489408,155358
x1,144:7384717,31964693
k1,143:7563395,31964693:178678
x1,143:8790472,31964693
k1,143:8969149,31964693:178677
x1,143:9562737,31964693
k1,143:9741415,31964693:178678
x1,143:11978224,31964693
k1,143:12200442,31964693:222218
x1,143:13724665,31964693
k1,143:13903488,31964693:178823
(1,143:13903488,31964693:877637,479368,0
x1,143:14781125,31964693
)
x1,143:15058317,31964693
k1,143:15236994,31964693:178677
x1,143:15909679,31964693
x1,143:16251627,31964693
x1,143:16557257,31964693
k1,143:16735935,31964693:178678
x1,143:18755392,31964693
k1,143:18934070,31964693:178678
x1,143:23169669,31964693
k1,143:23348346,31964693:178677
x1,143:24060940,31964693
x1,143:25111169,31964693
k1,143:25289847,31964693:178678
x1,143:26318829,31964693
k1,143:26497506,31964693:178677
x1,143:27051898,31964693
k1,143:27230576,31964693:178678
x1,143:28101356,31964693
k1,143:28280034,31964693:178678
x1,143:31012085,31964693
k1,143:31190762,31964693:178677
x1,143:31784350,31964693
k1,143:31963028,31964693:178678
x1,143:34338077,31964693
k1,143:34338077,31964693:0
)
(1,144:5920357,32855983:28417720,489408,155358
x1,144:7454598,32855983
g1,143:7634002,32855983
x1,143:9387847,32855983
g1,143:9567251,32855983
x1,143:10802978,32855983
x1,143:11114421,32855983
g1,143:11293825,32855983
x1,143:12011443,32855983
g1,143:12190847,32855983
x1,143:13067765,32855983
g1,143:13247169,32855983
x1,143:16136982,32855983
k1,144:34338077,32855983:18326678
g1,144:34338077,32855983
)
(1,149:5920357,34047753:28417720,494436,155358
h1,148:5920357,34047753:1114112,0,0
(1,148:7034469,34047753:0,0,0
(1,148:7034469,33156463:0,0,0
)
)
x1,148:8110887,34047753
x1,148:8462521,34047753
x1,148:8773964,34047753
k1,148:8960382,34047753:186418
x1,148:10156646,34047753
x1,148:10747235,34047753
k1,148:10933652,34047753:186417
x1,148:11172616,34047753
(1,148:11172616,34047753:996764,482592,13271
x1,148:12169380,34047753
)
x1,148:12408344,34047753
k1,148:12594762,34047753:186418
x1,148:14221162,34047753
x1,148:15481595,34047753
k1,148:15668012,34047753:186417
x1,148:16561735,34047753
k1,148:16748153,34047753:186418
x1,148:18252337,34047753
k1,148:18438754,34047753:186417
x1,148:21570097,34047753
k1,148:21756515,34047753:186418
x1,148:23098204,34047753
k1,148:23284621,34047753:186417
x1,148:24829067,34047753
k1,148:25015485,34047753:186418
x1,148:27698853,34047753
k1,148:27885271,34047753:186418
x1,148:31198864,34047753
k1,148:31387034,34047753:188170
x1,148:33175955,34047753
k1,148:33362373,34047753:186418
x1,148:34338077,34047753
k1,148:34338077,34047753:0
)
(1,149:5920357,34939043:28417720,489408,155358
x1,149:9504807,34939043
k1,148:9684319,34939043:179512
x1,148:11277235,34939043
x1,148:12232851,34939043
k1,148:12412363,34939043:179512
x1,148:14044728,34939043
k1,148:14224240,34939043:179512
x1,148:14941140,34939043
k1,148:15120652,34939043:179512
x1,148:16872734,34939043
k1,148:17052246,34939043:179512
x1,148:20278262,34939043
k1,148:20457774,34939043:179512
x1,148:23604216,34939043
k1,148:23783727,34939043:179511
x1,148:24341469,34939043
k1,148:24520981,34939043:179512
x1,148:26711072,34939043
k1,148:26890584,34939043:179512
x1,148:28203931,34939043
k1,148:28383443,34939043:179512
x1,148:30414392,34939043
k1,148:30593904,34939043:179512
x1,148:31709388,34939043
k1,148:31888900,34939043:179512
x1,148:32764941,34939043
k1,148:32944453,34939043:179512
x1,148:34338077,34939043
k1,148:34338077,34939043:0
)
(1,149:5920357,35830333:28417720,489408,155358
x1,149:7018294,35830333
k1,148:7245124,35830333:226830
x1,148:7652086,35830333
k1,148:7878916,35830333:226830
x1,148:8367126,35830333
k1,148:8593957,35830333:226831
x1,148:10017618,35830333
k1,148:10244448,35830333:226830
x1,148:11017395,35830333
x1,148:11904676,35830333
k1,148:12131506,35830333:226830
x1,148:12700972,35830333
k1,148:12927802,35830333:226830
x1,148:14920213,35830333
k1,148:15147043,35830333:226830
x1,148:15899501,35830333
k1,148:16264240,35830333:364739
x1,148:17402448,35830333
x1,148:17757675,35830333
k1,148:17984505,35830333:226830
x1,148:18878228,35830333
k1,148:19105058,35830333:226830
x1,148:20405752,35830333
k1,148:20632583,35830333:226831
x1,148:21202049,35830333
k1,148:21428879,35830333:226830
x1,148:23908758,35830333
k1,148:24135588,35830333:226830
x1,148:25192548,35830333
k1,148:25419378,35830333:226830
x1,148:25744368,35830333
x1,148:27270497,35830333
x1,148:27618541,35830333
x1,148:28115765,35830333
k1,148:28354452,35830333:238687
x1,148:31281554,35830333
k1,148:31508384,35830333:226830
x1,148:32809811,35830333
k1,148:33036641,35830333:226830
x1,148:34338077,35830333
k1,148:34338077,35830333:0
)
(1,149:5920357,36721623:28417720,489408,155358
x1,149:9498915,36721623
k1,148:9740661,36721623:241746
x1,148:11245578,36721623
k1,148:11487325,36721623:241747
x1,148:12889763,36721623
k1,148:13299250,36721623:409487
x1,148:15250668,36721623
x1,148:15605895,36721623
x1,148:16163870,36721623
x1,148:16318164,36721623
k1,148:16575496,36721623:257332
x1,148:17469952,36721623
x1,148:17825179,36721623
k1,148:18066926,36721623:241747
x1,148:19164863,36721623
x1,148:19675402,36721623
k1,148:19917148,36721623:241746
x1,148:20811604,36721623
k1,148:21053351,36721623:241747
x1,148:22151288,36721623
x1,148:24214180,36721623
k1,148:24455926,36721623:241746
x1,148:25065654,36721623
k1,148:25307401,36721623:241747
x1,148:25632391,36721623
x1,148:27125817,36721623
k1,148:27367563,36721623:241746
x1,148:28465518,36721623
x1,148:30561488,36721623
k1,148:30803235,36721623:241747
x1,148:31372701,36721623
k1,148:31614447,36721623:241746
x1,148:34338077,36721623
k1,148:34338077,36721623:0
)
(1,149:5920357,37612913:28417720,489408,155358
x1,149:9193671,37612913
k1,148:9538907,37612913:345236
x1,148:10677115,37612913
k1,148:10897444,37612913:220329
x1,148:13133580,37612913
x1,148:13481624,37612913
x1,148:13795856,37612913
k1,148:14016185,37612913:220329
x1,148:14748155,37612913
x1,148:15827427,37612913
k1,148:16047756,37612913:220329
x1,148:16657484,37612913
k1,148:16877813,37612913:220329
x1,148:18381988,37612913
k1,148:18602318,37612913:220330
x1,148:20899946,37612913
k1,148:21130506,37612913:230560
x1,148:23346904,37612913
k1,148:23577464,37612913:230560
x1,148:24065674,37612913
k1,148:24286003,37612913:220329
x1,148:26156905,37612913
k1,148:26377234,37612913:220329
x1,148:26702224,37612913
x1,148:28715847,37612913
k1,148:28936177,37612913:220330
x1,148:29668147,37612913
k1,148:29888476,37612913:220329
x1,148:30782932,37612913
k1,148:31003261,37612913:220329
x1,148:34338077,37612913
k1,148:34338077,37612913:0
)
(1,149:5920357,38504203:28417720,489408,155358
x1,149:6530085,38504203
k1,148:6747345,38504203:217260
x1,148:10041174,38504203
k1,148:10258434,38504203:217260
x1,148:13957785,38504203
x1,148:14313012,38504203
k1,148:14530272,38504203:217260
x1,148:16522683,38504203
k1,148:16739944,38504203:217261
x1,148:19056595,38504203
k1,148:19273855,38504203:217260
x1,148:19843321,38504203
k1,148:20060581,38504203:217260
x1,148:20955037,38504203
k1,148:21172297,38504203:217260
x1,148:22574735,38504203
k1,148:22801459,38504203:226724
x1,148:24590380,38504203
k1,148:24807640,38504203:217260
x1,148:26311815,38504203
k1,148:26529075,38504203:217260
x1,148:27098541,38504203
k1,148:27315802,38504203:217261
x1,148:29632470,38504203
k1,148:29849730,38504203:217260
x1,148:32084408,38504203
x1,148:32439635,38504203
k1,148:32656895,38504203:217260
x1,148:33226361,38504203
k1,148:33443621,38504203:217260
x1,148:34338077,38504203
k1,148:34338077,38504203:0
)
(1,149:5920357,39395493:28417720,489408,155358
x1,149:8430557,39395493
g1,148:8609961,39395493
x1,148:9207734,39395493
g1,148:9387138,39395493
x1,148:12256874,39395493
g1,148:12436278,39395493
x1,148:13951142,39395493
x1,148:15272261,39395493
k1,149:34338078,39395493:19191400
g1,149:34338078,39395493
)
(1,151:5920357,40587263:28417720,494436,155358
h1,150:5920357,40587263:1114112,0,0
(1,150:7034469,40587263:0,0,0
(1,150:7034469,39695973:0,0,0
)
)
x1,150:7831733,40587263
x1,150:9345896,40587263
x1,150:10169711,40587263
k1,150:10349620,40587263:179909
x1,150:12143647,40587263
x1,150:13220065,40587263
k1,150:13399974,40587263:179909
x1,150:13638938,40587263
(1,150:13638938,40587263:1594536,482592,13271
x1,150:15233474,40587263
)
x1,150:15472438,40587263
k1,150:15652347,40587263:179909
x1,150:16167866,40587263
x1,150:16881896,40587263
x1,150:18706927,40587263
k1,150:18886835,40587263:179908
x1,150:19560875,40587263
x1,150:19903541,40587263
x1,150:20209808,40587263
k1,150:20389717,40587263:179909
x1,150:21737797,40587263
k1,150:21917706,40587263:179909
x1,150:22869496,40587263
x1,150:24059046,40587263
x1,150:25407833,40587263
k1,150:25587742,40587263:179909
x1,150:26896547,40587263
k1,150:27076456,40587263:179909
x1,150:27631965,40587263
k1,150:27811874,40587263:179909
x1,150:29437696,40587263
k1,150:29617604,40587263:179908
x1,150:30846438,40587263
k1,150:31026347,40587263:179909
x1,150:32532940,40587263
k1,150:32712849,40587263:179909
x1,150:33386889,40587263
x1,150:34219433,40587263
x1,150:34457202,40587263
k1,151:34338077,40587263:0
)
(1,151:5920357,41478553:28417720,490372,155358
x1,151:7190441,41478553
k1,150:7402994,41478553:212553
x1,150:9121755,41478553
k1,150:9271437,41478553:149682
x1,150:9974703,41478553
k1,150:10124385,41478553:149682
x1,150:11140583,41478553
k1,150:11290265,41478553:149682
x1,150:12461891,41478553
x1,150:14200353,41478553
k1,150:14355980,41478553:155627
x1,150:14668226,41478553
k1,150:14817908,41478553:149682
x1,150:15481787,41478553
x1,150:15971602,41478553
k1,150:16121284,41478553:149682
x1,150:16668418,41478553
x1,150:18425853,41478553
k1,150:18575535,41478553:149682
x1,150:20176865,41478553
k1,150:20326547,41478553:149682
x1,150:20795611,41478553
k1,150:20945293,41478553:149682
x1,150:22038849,41478553
x1,150:22507913,41478553
x1,150:23562803,41478553
k1,150:23712485,41478553:149682
x1,150:25313806,41478553
k1,150:25463488,41478553:149682
x1,150:26166754,41478553
k1,150:26316436,41478553:149682
x1,150:26981001,41478553
k1,150:27130683,41478553:149682
$1,150:27130683,41478553
x1,150:27740161,41478553
$1,150:27791490,41478553
k1,150:27941172,41478553:149682
x1,150:28917297,41478553
x1,150:29932792,41478553
k1,150:30082474,41478553:149682
x1,150:31645120,41478553
x1,150:33031950,41478553
k1,150:33244503,41478553:212553
x1,150:34338077,41478553
k1,150:34338077,41478553:0
)
(1,151:5920357,42369843:28417720,489408,155358
x1,151:6238019,42369843
x1,151:7331950,42369843
x1,151:7729736,42369843
x1,151:8069528,42369843
x1,151:8376432,42369843
x1,151:9608445,42369843
k1,150:9788653,42369843:180208
x1,150:10384633,42369843
k1,150:10564842,42369843:180209
x1,150:11598670,42369843
k1,150:11778878,42369843:180208
x1,150:13567524,42369843
k1,150:13747732,42369843:180208
x1,150:14224934,42369843
k1,150:14405142,42369843:180208
x1,150:14961768,42369843
x1,150:15717295,42369843
x1,150:17385747,42369843
k1,150:17565956,42369843:180209
x1,150:18281422,42369843
k1,150:18461630,42369843:180208
x1,150:19335918,42369843
k1,150:19516126,42369843:180208
x1,150:20351061,42369843
x1,150:21860673,42369843
k1,150:22040881,42369843:180208
x1,150:23114061,42369843
x1,150:23868863,42369843
k1,150:24049072,42369843:180209
x1,150:25360509,42369843
k1,150:25540717,42369843:180208
x1,150:26097343,42369843
k1,150:26277551,42369843:180208
x1,150:26834177,42369843
x1,150:27986056,42369843
k1,150:28166264,42369843:180208
x1,150:29040552,42369843
k1,150:29220761,42369843:180209
x1,150:30213818,42369843
x1,150:31246929,42369843
k1,150:31427137,42369843:180208
x1,150:33016891,42369843
x1,150:34427779,42369843
k1,150:34338077,42369843:0
)
(1,151:5920357,43261133:28417720,490372,155358
x1,151:6977317,43261133
k1,150:7185538,43261133:208221
x1,150:8364723,43261133
k1,150:8572944,43261133:208221
x1,150:9467400,43261133
k1,150:9675620,43261133:208220
x1,150:10366595,43261133
x1,150:11504794,43261133
x1,150:11829784,43261133
x1,150:12601998,43261133
k1,150:12810219,43261133:208221
$1,150:12810219,43261133
x1,150:13419697,43261133
$1,150:13471026,43261133
k1,150:13679247,43261133:208221
x1,150:15468168,43261133
k1,150:15676389,43261133:208221
x1,150:16367364,43261133
x1,150:16895835,43261133
x1,150:18888229,43261133
k1,150:19096450,43261133:208221
x1,150:19990906,43261133
k1,150:20199126,43261133:208220
x1,150:21500562,43261133
x1,150:22435280,43261133
k1,150:22643501,43261133:208221
x1,150:23253229,43261133
k1,150:23461450,43261133:208221
x1,150:25087876,43261133
x1,150:26348318,43261133
k1,150:26556539,43261133:208221
x1,150:28629464,43261133
k1,150:28837685,43261133:208221
x1,150:29407151,43261133
k1,150:29615371,43261133:208220
x1,150:30753561,43261133
x1,150:31851499,43261133
k1,150:32059720,43261133:208221
x1,150:32954176,43261133
k1,150:33162397,43261133:208221
x1,150:33853372,43261133
x1,150:34363911,43261133
k1,150:34338077,43261133:0
)
(1,151:5920357,44152423:28417720,489408,155358
x1,151:7076421,44152423
x1,151:8132743,44152423
g1,150:8355203,44152423
x1,150:10028676,44152423
x1,150:11363435,44152423
g1,150:11542839,44152423
x1,150:12419757,44152423
x1,150:13296667,44152423
g1,150:13476071,44152423
x1,150:13994180,44152423
x1,150:14711798,44152423
x1,150:16545999,44152423
g1,150:16725403,44152423
x1,150:17601603,44152423
g1,150:17781007,44152423
x1,150:18099625,44152423
x1,150:18447676,44152423
x1,150:20639967,44152423
g1,150:20819371,44152423
x1,150:21775944,44152423
x1,150:22254581,44152423
x1,150:22653563,44152423
x1,150:22994431,44152423
x1,150:23302291,44152423
g1,150:23481695,44152423
x1,150:24039995,44152423
g1,150:24219399,44152423
x1,150:25913676,44152423
k1,151:34338077,44152423:8549984
g1,151:34338077,44152423
)
(1,157:5920357,45344193:28417720,489408,155358
h1,154:5920357,45344193:1114112,0,0
x1,154:8987414,45344193
k1,154:9156016,45344193:168602
x1,154:10639898,45344193
k1,154:10808499,45344193:168601
x1,154:13386639,45344193
k1,154:13555241,45344193:168602
x1,154:15897791,45344193
k1,154:16066393,45344193:168602
x1,154:17003835,45344193
k1,154:17172437,45344193:168602
x1,154:18500195,45344193
k1,154:18668796,45344193:168601
x1,154:18902981,45344193
x1,154:19442237,45344193
k1,154:19610839,45344193:168602
x1,154:21056037,45344193
k1,154:21224639,45344193:168602
x1,154:21576272,45344193
x1,154:22964142,45344193
k1,154:23132744,45344193:168602
x1,154:23679878,45344193
k1,155:23848479,45344193:168601
x1,155:26231822,45344193
k1,155:26400424,45344193:168602
x1,155:28607950,45344193
k1,155:28778713,45344193:170763
x1,155:31240126,45344193
k1,155:31408727,45344193:168601
x1,155:32268107,45344193
k1,155:32436709,45344193:168602
x1,155:34350277,45344193
k1,155:34338077,45344193:0
)
(1,157:5920357,46235483:28417720,489408,155358
x1,157:8989575,46235483
g1,155:9168979,46235483
x1,155:10045179,46235483
g1,155:10224583,46235483
x1,155:11301693,46235483
g1,155:11481097,46235483
x1,155:13673406,46235483
k1,157:34338078,46235483:20676872
g1,157:34338078,46235483
)
]
(1,160:5920357,48201563:28417720,446948,9168
(1,160:5920357,48201563:28417720,446948,9168
k1,160:19965377,48201563:14045020
x1,160:20293057,48201563
k1,160:34338077,48201563:14045020
)
)
]
]
]
!41812
}3
!10
{4
[1,170:4736286,48201563:29601791,43465277,0
[1,170:4736286,4736286:0,0,0
(1,170:4736286,2302362:0,0,0
k1,170:4736286,2302362:-1118290
)
]
[1,170:4736286,48201563:29601791,43465277,0
h1,170:4736286,4736286:0,0,0
[1,170:5920357,48201563:28417720,45833420,0
[1,170:5920357,3154575:28417720,786432,0
(1,170:5920357,3154575:28417720,435811,8188
(1,170:5920357,3154575:28417720,435811,8188
k1,170:18797293,3154575:12876936
x1,170:19303229,3154575
x1,170:20783666,3154575
x1,170:21281738,3154575
g1,170:21461142,3154575
k1,170:34338078,3154575:12876936
)
)
]
[1,170:5920357,46235483:28417720,40258437,0
(1,158:5920357,6697942:28417720,487261,8965
(1,158:5920357,6697942:1973449,487261,8965
g1,158:5920357,6697942
x1,158:7534997,6697942
g1,158:7893806,6697942
)
x1,158:10861123,6697942
x1,158:12682412,6697942
g1,158:12861816,6697942
(1,158:12861816,6697942:1148181,477213,0
x1,158:14009997,6697942
)
g1,158:14189401,6697942
x1,158:18411097,6697942
g1,158:18590501,6697942
x1,158:19813309,6697942
g1,158:19992713,6697942
x1,158:22374450,6697942
g1,158:22553854,6697942
x1,158:24386630,6697942
g1,158:24566034,6697942
x1,158:25869215,6697942
x1,158:26737524,6697942
g1,158:26916928,6697942
x1,158:30560218,6697942
k1,158:32449148,6697942:1888930
k1,158:34338077,6697942:1888929
)
(1,160:5920357,8034526:28417720,489408,155358
x1,160:6997264,8034526
k1,159:7177200,8034526:179936
x1,159:9140118,8034526
k1,159:9320055,8034526:179937
x1,159:10537247,8034526
k1,159:10717183,8034526:179936
x1,159:11305990,8034526
k1,159:11485927,8034526:179937
x1,159:14665330,8034526
k1,159:14845266,8034526:179936
x1,159:16022870,8034526
k1,159:16202807,8034526:179937
x1,159:17459578,8034526
k1,159:17639514,8034526:179936
x1,159:21369551,8034526
k1,159:21549488,8034526:179937
x1,159:24749383,8034526
k1,159:24929452,8034526:180069
x1,159:26656990,8034526
k1,159:26836927,8034526:179937
x1,159:28524869,8034526
k1,159:28704805,8034526:179936
x1,159:30981562,8034526
k1,159:31161499,8034526:179937
x1,159:31711425,8034526
k1,159:31891361,8034526:179936
x1,159:33225893,8034526
x1,159:34350277,8034526
k1,159:34338077,8034526:0
)
(1,160:5920357,8925816:28417720,489408,155358
x1,160:6527096,8925816
k1,159:6705932,8925816:178836
x1,159:8971909,8925816
k1,159:9150744,8925816:178835
x1,159:12812266,8925816
k1,159:13034537,8925816:222271
x1,159:13641276,8925816
k1,159:13820112,8925816:178836
x1,159:15316913,8925816
k1,159:15495748,8925816:178835
x1,159:18954076,8925816
k1,159:19133026,8925816:178950
x1,159:20023097,8925816
k1,159:20201932,8925816:178835
x1,159:20727812,8925816
x1,159:23104646,8925816
k1,159:23283482,8925816:178836
x1,159:24496951,8925816
k1,159:24675787,8925816:178836
x1,159:26050963,8925816
x1,159:27735907,8925816
k1,159:27914742,8925816:178835
x1,159:29735679,8925816
k1,159:29914515,8925816:178836
x1,159:30400331,8925816
k1,159:30579167,8925816:178836
x1,159:32904866,8925816
k1,159:33083815,8925816:178949
x1,159:34338077,8925816
k1,159:34338077,8925816:0
)
(1,160:5920357,9817106:28417720,489408,155358
x1,160:6949323,9817106
x1,159:8475544,9817106
k1,159:8654513,9817106:178969
x1,159:9921491,9817106
k1,159:10100461,9817106:178970
x1,159:12198334,9817106
k1,159:12377303,9817106:178969
x1,159:15068035,9817106
k1,159:15247004,9817106:178969
x1,159:16632275,9817106
k1,159:16811245,9817106:178970
x1,159:17682025,9817106
k1,159:17860994,9817106:178969
x1,159:19365271,9817106
k1,159:19544241,9817106:178970
x1,159:20019528,9817106
k1,159:20198497,9817106:178969
x1,159:22572833,9817106
k1,159:22751802,9817106:178969
x1,159:23345382,9817106
k1,159:23524352,9817106:178970
x1,159:25483256,9817106
k1,159:25705571,9817106:222315
x1,159:26576359,9817106
k1,159:26755328,9817106:178969
x1,159:27784310,9817106
x1,159:29626222,9817106
k1,159:29805192,9817106:178970
x1,159:30398780,9817106
k1,159:30577749,9817106:178969
x1,159:34338077,9817106
k1,159:34338077,9817106:0
)
(1,160:5920357,10708396:28417720,489408,155358
x1,160:8376658,10708396
k1,159:8556334,10708396:179676
x1,159:9039757,10708396
k1,159:9219432,10708396:179675
x1,159:10306605,10708396
k1,159:10486281,10708396:179676
x1,159:11371968,10708396
x1,159:11723607,10708396
k1,159:11903282,10708396:179675
x1,159:12788244,10708396
k1,159:12967920,10708396:179676
x1,159:14457358,10708396
k1,159:14637034,10708396:179676
x1,159:15361828,10708396
x1,159:17235581,10708396
k1,159:17415256,10708396:179675
x1,159:17979139,10708396
k1,159:18158815,10708396:179676
x1,159:20815876,10708396
k1,159:20995551,10708396:179675
x1,159:21921106,10708396
x1,159:24037662,10708396
k1,159:24217338,10708396:179676
x1,159:26230074,10708396
k1,159:26409750,10708396:179676
x1,159:27939771,10708396
k1,159:28119446,10708396:179675
x1,159:28723197,10708396
k1,159:28902873,10708396:179676
x1,159:30895314,10708396
k1,159:31118589,10708396:223275
x1,159:32668906,10708396
k1,159:32848649,10708396:179743
x1,159:34338077,10708396
k1,159:34338077,10708396:0
)
(1,160:5920357,11599686:28417720,489408,155358
x1,160:6791137,11599686
x1,159:7136676,11599686
k1,159:7315297,11599686:178621
x1,159:8027891,11599686
k1,159:8206513,11599686:178622
x1,159:9117202,11599686
k1,159:9295823,11599686:178621
x1,159:10641193,11599686
k1,159:10819814,11599686:178621
x1,159:12877762,11599686
k1,159:13056384,11599686:178622
x1,159:14421700,11599686
k1,159:14600478,11599686:178778
x1,159:16064838,11599686
k1,159:16243459,11599686:178621
x1,159:18658417,11599686
k1,159:18837038,11599686:178621
x1,159:19826111,11599686
k1,159:20004733,11599686:178622
x1,159:20677418,11599686
k1,159:20856039,11599686:178621
x1,159:22597599,11599686
k1,159:22776220,11599686:178621
x1,159:23330612,11599686
k1,159:23509234,11599686:178622
x1,159:26675966,11599686
k1,159:26854587,11599686:178621
x1,159:28595442,11599686
k1,159:28774063,11599686:178621
x1,159:29486657,11599686
k1,159:29665279,11599686:178622
x1,159:31050550,11599686
k1,159:31229171,11599686:178621
x1,159:32298062,11599686
x1,159:34338077,11599686
k1,159:34338077,11599686:0
)
(1,160:5920357,12490976:28417720,489408,155358
x1,160:6477939,12490976
x1,159:6825990,12490976
x1,159:8655906,12490976
g1,159:8835310,12490976
x1,159:9712228,12490976
g1,159:9891632,12490976
x1,159:12641505,12490976
g1,159:12820909,12490976
x1,159:14813692,12490976
g1,159:14993096,12490976
x1,159:15590869,12490976
g1,159:15770273,12490976
x1,159:17683428,12490976
x1,159:19379851,12490976
g1,159:19559255,12490976
x1,159:20037892,12490976
g1,159:20217296,12490976
x1,159:20535914,12490976
x1,159:20880374,12490976
x1,159:22954973,12490976
k1,160:34338077,12490976:11508687
g1,160:34338077,12490976
)
(1,162:5920357,13448649:28417720,489408,155358
h1,161:5920357,13448649:1114112,0,0
x1,161:8253924,13448649
k1,161:8508119,13448649:254195
x1,161:9117847,13448649
k1,161:9372041,13448649:254194
x1,161:10266497,13448649
k1,161:10520692,13448649:254195
x1,161:11944353,13448649
k1,161:12198548,13448649:254195
x1,161:13296503,13448649
x1,161:14173027,13448649
k1,161:14427222,13448649:254195
x1,161:18289794,13448649
k1,161:18543988,13448649:254194
x1,161:21675314,13448649
k1,161:21929509,13448649:254195
x1,161:23271198,13448649
k1,161:23525393,13448649:254195
x1,161:24094859,13448649
k1,161:24349054,13448649:254195
x1,161:25893500,13448649
k1,161:26147694,13448649:254194
x1,161:28831062,13448649
k1,161:29085257,13448649:254195
x1,161:29573467,13448649
k1,161:29827662,13448649:254195
x1,161:32897504,13448649
k1,161:33344336,13448649:446832
x1,161:33751307,13448649
x1,161:34350277,13448649
k1,161:34338077,13448649:0
)
(1,162:5920357,14339939:28417720,494436,155358
x1,162:6245347,14339939
x1,161:8572478,14339939
k1,161:8861506,14339939:289028
(1,161:8861506,14339939:0,0,0
(1,161:8861506,13448649:0,0,0
)
)
x1,161:9658770,14339939
x1,161:11691762,14339939
k1,161:11958866,14339939:267104
x1,161:12197830,14339939
(1,161:12197830,14339939:1235728,482592,0
x1,161:13433558,14339939
)
x1,161:13672522,14339939
k1,161:13939626,14339939:267104
x1,161:14427836,14339939
k1,161:14694940,14339939:267104
x1,161:15019930,14339939
k1,161:15287034,14339939:267104
x1,161:17239166,14339939
k1,161:17506270,14339939:267104
x1,161:18563230,14339939
k1,161:18830334,14339939:267104
x1,161:19155324,14339939
x1,161:21210666,14339939
k1,161:21477770,14339939:267104
x1,161:24364620,14339939
k1,161:24631723,14339939:267103
x1,161:26827615,14339939
k1,161:27094719,14339939:267104
x1,161:28192656,14339939
k1,161:28459760,14339939:267104
x1,161:31225101,14339939
k1,161:31492205,14339939:267104
x1,161:34338077,14339939
k1,161:34338077,14339939:0
)
(1,162:5920357,15231229:28417720,490372,155358
x1,162:8234797,15231229
k1,161:8413439,15231229:178642
x1,161:9531155,15231229
k1,161:9709797,15231229:178642
$1,161:9709797,15231229
x1,161:10319275,15231229
$1,161:10370604,15231229
k1,161:10549246,15231229:178642
x1,161:12704935,15231229
k1,161:12883577,15231229:178642
x1,161:15078052,15231229
k1,161:15256694,15231229:178642
x1,161:16573392,15231229
k1,161:16752034,15231229:178642
x1,161:17829519,15231229
k1,161:18008161,15231229:178642
x1,161:18885956,15231229
k1,161:19064598,15231229:178642
x1,161:20939436,15231229
k1,161:21118078,15231229:178642
x1,161:21716449,15231229
k1,161:21895091,15231229:178642
x1,161:24249043,15231229
k1,161:24427685,15231229:178642
x1,161:26821158,15231229
k1,161:26999800,15231229:178642
x1,161:27877595,15231229
k1,161:28056237,15231229:178642
x1,161:29812546,15231229
k1,161:29991188,15231229:178642
x1,161:31028461,15231229
k1,161:31207103,15231229:178642
x1,161:33561064,15231229
k1,161:33739706,15231229:178642
x1,161:34338077,15231229
k1,161:34338077,15231229:0
)
(1,162:5920357,16122519:28417720,489408,155358
x1,162:7018294,16122519
k1,161:7214587,16122519:196293
x1,161:9165986,16122519
k1,161:9362280,16122519:196294
x1,161:9850490,16122519
k1,161:10046783,16122519:196293
x1,161:13361100,16122519
k1,161:13634229,16122519:273129
x1,161:16399596,16122519
k1,161:16595889,16122519:196293
(1,161:16595889,16122519:1156074,479368,0
x1,161:17751963,16122519
)
k1,161:17948257,16122519:196294
x1,161:20835107,16122519
k1,161:21031400,16122519:196293
x1,161:24162726,16122519
k1,161:24359020,16122519:196294
x1,161:25252743,16122519
k1,161:25449036,16122519:196293
x1,161:27401168,16122519
k1,161:27597462,16122519:196294
x1,161:28654422,16122519
k1,161:28850715,16122519:196293
x1,161:30151409,16122519
k1,161:30347703,16122519:196294
x1,161:30917169,16122519
k1,161:31113462,16122519:196293
x1,161:34427779,16122519
k1,161:34338077,16122519:0
)
(1,162:5920357,17013809:28417720,489408,155358
x1,162:6814813,17013809
x1,161:7170040,17013809
k1,161:7348604,17013809:178564
x1,161:8242327,17013809
k1,161:8420890,17013809:178563
x1,161:8786875,17013809
x1,161:9710835,17013809
k1,161:9889399,17013809:178564
x1,161:11760275,17013809
x1,161:12108319,17013809
x1,161:12422551,17013809
k1,161:12601114,17013809:178563
x1,161:13170580,17013809
k1,161:13349144,17013809:178564
x1,161:14243600,17013809
k1,161:14422163,17013809:178563
x1,161:16130543,17013809
k1,161:16309107,17013809:178564
x1,161:18260506,17013809
k1,161:18439069,17013809:178563
x1,161:20694969,17013809
k1,161:20873701,17013809:178732
x1,161:22662622,17013809
k1,161:22841185,17013809:178563
x1,161:23734908,17013809
k1,161:23913472,17013809:178564
x1,161:26719092,17013809
k1,161:26897655,17013809:178563
x1,161:29438283,17013809
k1,161:29660463,17013809:222180
x1,161:30961891,17013809
k1,161:31140454,17013809:178563
x1,161:32400895,17013809
x1,161:33003439,17013809
k1,161:33182003,17013809:178564
(1,161:33182003,17013809:1156074,479368,0
x1,161:34338077,17013809
)
k1,161:34338077,17013809:0
)
(1,162:5920357,17905099:28417720,489408,155358
x1,162:8944239,17905099
k1,161:9124032,17905099:179793
x1,161:12107635,17905099
k1,161:12287428,17905099:179793
x1,161:12837354,17905099
k1,161:13017147,17905099:179793
x1,161:15314389,17905099
k1,161:15494280,17905099:179891
x1,161:17221818,17905099
k1,161:17401611,17905099:179793
x1,161:18264669,17905099
k1,161:18444462,17905099:179793
x1,161:21271128,17905099
k1,161:21450921,17905099:179793
x1,161:22510478,17905099
x1,161:22845964,17905099
x1,161:23691788,17905099
k1,161:23871581,17905099:179793
x1,161:24421507,17905099
k1,161:24601300,17905099:179793
x1,161:26092753,17905099
k1,161:26272547,17905099:179794
x1,161:28863842,17905099
k1,161:29043635,17905099:179793
x1,161:30574666,17905099
x1,161:31290547,17905099
k1,161:31514174,17905099:223627
x1,161:33398634,17905099
x1,161:33741303,17905099
x1,161:34279764,17905099
x1,161:34427779,17905099
k1,161:34338077,17905099:0
)
(1,162:5920357,18796389:28417720,490372,155358
x1,162:7929806,18796389
k1,161:8109254,18796389:179448
x1,161:8672020,18796389
k1,161:8851468,18796389:179448
(1,161:8851468,18796389:1554354,479368,8247
x1,161:10405822,18796389
)
k1,161:10585270,18796389:179448
x1,161:13217545,18796389
k1,161:13397004,18796389:179459
x1,161:13959770,18796389
k1,161:14139218,18796389:179448
(1,161:14139218,18796389:1156074,479368,0
x1,161:15295292,18796389
)
x1,161:15576671,18796389
k1,161:15756119,18796389:179448
x1,161:16640052,18796389
k1,161:16819500,18796389:179448
x1,161:19711452,18796389
k1,161:19890899,18796389:179447
$1,161:19890899,18796389
x1,161:20500377,18796389
$1,161:20551706,18796389
k1,161:20731154,18796389:179448
x1,161:22660336,18796389
k1,161:22839784,18796389:179448
x1,161:23522630,18796389
k1,161:23702078,18796389:179448
x1,161:25710828,18796389
k1,161:25890276,18796389:179448
x1,161:29747185,18796389
x1,161:29881385,18796389
k1,161:30060844,18796389:179459
x1,161:31828719,18796389
k1,161:32008167,18796389:179448
x1,161:34338077,18796389
k1,161:34338077,18796389:0
)
(1,162:5920357,19687679:28417720,489408,155358
x1,162:7372159,19687679
k1,161:7551263,19687679:179104
x1,161:8923980,19687679
k1,161:9103083,19687679:179103
x1,161:11221473,19687679
k1,161:11400577,19687679:179104
x1,161:11714097,19687679
x1,161:13605649,19687679
k1,161:13784813,19687679:179164
x1,161:14373022,19687679
k1,161:14552126,19687679:179104
x1,161:14944724,19687679
k1,161:15123828,19687679:179104
x1,161:16613757,19687679
k1,161:16792860,19687679:179103
x1,161:17655747,19687679
k1,161:17834851,19687679:179104
x1,161:18187919,19687679
x1,161:19781435,19687679
k1,161:19960539,19687679:179104
x1,161:20548748,19687679
k1,161:20727852,19687679:179104
x1,161:23552360,19687679
k1,161:23731463,19687679:179103
x1,161:27262107,19687679
k1,161:27441211,19687679:179104
x1,161:27990578,19687679
k1,161:28169682,19687679:179104
x1,161:29268425,19687679
k1,161:29447529,19687679:179104
x1,161:30310416,19687679
k1,161:30489519,19687679:179103
x1,161:32647439,19687679
k1,161:32826543,19687679:179104
x1,161:33179611,19687679
x1,161:34338077,19687679
k1,161:34338077,19687679:0
)
(1,162:5920357,20578969:28417720,490372,155358
x1,162:6518130,20578969
k1,161:6697995,20578969:179865
$1,161:6697995,20578969
x1,161:7307473,20578969
$1,161:7358802,20578969
x1,161:7538206,20578969
k1,161:7762048,20578969:223842
x1,161:10113666,20578969
k1,161:10293530,20578969:179864
x1,161:12167212,20578969
x1,161:14022234,20578969
k1,161:14202099,20578969:179865
x1,161:14799872,20578969
k1,161:14979737,20578969:179865
x1,161:15856655,20578969
k1,161:16036519,20578969:179864
x1,161:18866765,20578969
k1,161:19046630,20578969:179865
x1,161:21658016,20578969
k1,161:21837996,20578969:179980
x1,161:24549132,20578969
k1,161:24728997,20578969:179865
(1,161:24728997,20578969:1156074,479368,0
x1,161:25885071,20578969
)
x1,161:26343621,20578969
k1,161:26523600,20578969:179979
x1,161:27002237,20578969
k1,161:27182102,20578969:179865
x1,161:29931983,20578969
k1,161:30111848,20578969:179865
x1,161:30709621,20578969
k1,161:30889485,20578969:179864
x1,161:33480785,20578969
k1,161:33660650,20578969:179865
x1,161:34338077,20578969
k1,161:34338077,20578969:0
)
(1,162:5920357,21470259:28417720,489408,155358
x1,162:9155677,21470259
k1,161:9335815,21470259:180138
x1,161:11150962,21470259
k1,161:11331100,21470259:180138
x1,161:11883817,21470259
k1,161:12063955,21470259:180138
x1,161:14431118,21470259
k1,161:14611255,21470259:180137
x1,161:15479404,21470259
k1,161:15659542,21470259:180138
x1,161:17987627,21470259
k1,161:18167765,21470259:180138
x1,161:20534936,21470259
k1,161:20715074,21470259:180138
x1,161:22609098,21470259
x1,161:24465988,21470259
k1,161:24690650,21470259:224662
x1,161:25085651,21470259
x1,161:25666688,21470259
k1,161:25846825,21470259:180137
x1,161:26162257,21470259
x1,161:28420628,21470259
k1,161:28600950,21470259:180322
x1,161:28995942,21470259
k1,161:29176080,21470259:180138
x1,161:29649931,21470259
k1,161:29830068,21470259:180137
x1,161:30738006,21470259
k1,161:30918144,21470259:180138
x1,161:31588797,21470259
k1,161:31768935,21470259:180138
x1,161:33031375,21470259
k1,161:33211513,21470259:180138
x1,161:34356017,21470259
k1,161:34338077,21470259:0
)
(1,162:5920357,22361549:28417720,489408,155358
x1,162:6467491,22361549
k1,161:6636496,22361549:169005
x1,161:9058522,22361549
k1,161:9227527,22361549:169005
x1,161:10359766,22361549
x1,161:12301953,22361549
k1,161:12470958,22361549:169005
x1,161:13486470,22361549
k1,161:13655474,22361549:169004
x1,161:16467799,22361549
k1,161:16636804,22361549:169005
x1,161:18121371,22361549
x1,161:19239965,22361549
k1,161:19408970,22361549:169005
x1,161:19956104,22361549
k1,161:20125109,22361549:169005
x1,161:20437355,22361549
k1,161:20606360,22361549:169005
x1,161:22012892,22361549
k1,161:22181897,22361549:169005
x1,161:24955539,22361549
k1,161:25124544,22361549:169005
x1,161:27097173,22361549
k1,161:27268257,22361549:171084
x1,161:28713446,22361549
k1,161:28882451,22361549:169005
x1,161:31148337,22361549
k1,161:31317342,22361549:169005
x1,161:32528355,22361549
k1,161:32697360,22361549:169005
x1,161:34338077,22361549
k1,161:34338077,22361549:0
)
(1,162:5920357,23252839:28417720,489408,155358
x1,162:6469724,23252839
x1,162:8883266,23252839
k1,161:9062069,23252839:178803
x1,161:9768205,23252839
k1,161:9947008,23252839:178803
x1,161:11437643,23252839
k1,161:11616446,23252839:178803
x1,161:13656441,23252839
k1,161:13835244,23252839:178803
x1,161:14423453,23252839
k1,161:14602256,23252839:178803
x1,161:16092882,23252839
x1,161:17216100,23252839
k1,161:17394903,23252839:178803
x1,161:18610858,23252839
k1,161:18789661,23252839:178803
x1,161:19652548,23252839
x1,161:19994858,23252839
k1,161:20173661,23252839:178803
x1,161:20879797,23252839
k1,161:21058600,23252839:178803
x1,161:21764736,23252839
k1,161:21943539,23252839:178803
x1,161:23845849,23252839
k1,161:24068108,23252839:222259
x1,161:25323604,23252839
k1,161:25502407,23252839:178803
x1,161:26718362,23252839
k1,161:26897165,23252839:178803
x1,161:28073572,23252839
k1,161:28252375,23252839:178803
x1,161:28801742,23252839
k1,161:28980545,23252839:178803
x1,161:31805743,23252839
k1,161:31984546,23252839:178803
x1,161:34338077,23252839
k1,161:34338077,23252839:0
)
(1,162:5920357,24144129:28417720,489408,155358
x1,162:6478657,24144129
g1,161:6658061,24144129
x1,161:9727271,24144129
x1,161:11361271,24144129
g1,161:11540675,24144129
x1,161:14152061,24144129
k1,162:34338078,24144129:20311600
g1,162:34338078,24144129
)
(1,165:5920357,25101802:28417720,494436,155358
h1,164:5920357,25101802:1114112,0,0
(1,164:7034469,25101802:0,0,0
(1,164:7034469,24210512:0,0,0
)
)
x1,164:8429497,25101802
x1,164:9306415,25101802
x1,164:11891249,25101802
k1,164:12113937,25101802:222688
x1,164:13549165,25101802
k1,164:13771852,25101802:222687
x1,164:14010816,25101802
(1,164:14010816,25101802:1634719,494436,13271
x1,164:15645535,25101802
)
x1,164:15884499,25101802
k1,164:16107187,25101802:222688
x1,164:16595397,25101802
k1,164:16818084,25101802:222687
x1,164:17509059,25101802
k1,164:17731747,25101802:222688
x1,164:21594319,25101802
k1,164:21817006,25101802:222687
x1,164:23646180,25101802
k1,164:23868868,25101802:222688
x1,164:25291804,25101802
x1,164:26260342,25101802
k1,164:26483030,25101802:222688
x1,164:28881670,25101802
k1,164:29104357,25101802:222687
x1,164:31117256,25101802
k1,164:31350764,25101802:233508
x1,164:33139685,25101802
k1,164:33362373,25101802:222688
x1,164:34338077,25101802
k1,164:34338077,25101802:0
)
(1,165:5920357,25993092:28417720,489408,155358
x1,165:7269793,25993092
k1,164:7449923,25993092:180130
x1,164:8760044,25993092
k1,164:8940174,25993092:180130
x1,164:9496241,25993092
k1,164:9676371,25993092:180130
x1,164:11065828,25993092
k1,164:11245958,25993092:180130
x1,164:13866191,25993092
k1,164:14046321,25993092:180130
x1,164:14999077,25993092
x1,164:16190538,25993092
k1,164:16370668,25993092:180130
x1,164:17402760,25993092
k1,164:17582890,25993092:180130
x1,164:20123778,25993092
k1,164:20303908,25993092:180130
x1,164:23241494,25993092
k1,164:23421624,25993092:180130
x1,164:25863169,25993092
k1,164:26087807,25993092:224638
x1,164:26683189,25993092
k1,164:26863319,25993092:180130
(1,164:26863319,25993092:1555065,489408,10039
x1,164:28418384,25993092
)
x1,164:28597070,25993092
k1,164:28777381,25993092:180311
x1,164:29650792,25993092
k1,164:29830922,25993092:180130
x1,164:32967192,25993092
k1,164:33147322,25993092:180130
x1,164:34338077,25993092
k1,164:34338077,25993092:0
)
(1,165:5920357,26884382:28417720,489408,155358
x1,165:6408567,26884382
k1,164:6611041,26884382:202474
x1,164:9009699,26884382
k1,164:9212174,26884382:202475
x1,164:10351106,26884382
k1,164:10553580,26884382:202474
x1,164:12870981,26884382
k1,164:13073456,26884382:202475
x1,164:14130416,26884382
k1,164:14332890,26884382:202474
x1,164:17341258,26884382
k1,164:17543733,26884382:202475
x1,164:18641662,26884382
k1,164:18844136,26884382:202474
x1,164:21121285,26884382
k1,164:21323760,26884382:202475
x1,164:22218216,26884382
k1,164:22420690,26884382:202474
x1,164:24615841,26884382
k1,164:24818316,26884382:202475
x1,164:25428044,26884382
k1,164:25630518,26884382:202474
x1,164:26931204,26884382
x1,164:27540932,26884382
x1,164:27894004,26884382
x1,164:30756780,26884382
k1,164:30965022,26884382:208242
x1,164:32753943,26884382
k1,164:32956418,26884382:202475
x1,164:33444628,26884382
k1,164:33647102,26884382:202474
x1,164:34338077,26884382
k1,164:34338077,26884382:0
)
(1,165:5920357,27775672:28417720,489408,155358
x1,165:7586152,27775672
x1,164:7925226,27775672
x1,164:8231493,27775672
k1,164:8411052,27775672:179559
x1,164:10236100,27775672
k1,164:10415658,27775672:179558
x1,164:10971167,27775672
k1,164:11150726,27775672:179559
x1,164:12023260,27775672
k1,164:12202819,27775672:179559
x1,164:14424139,27775672
k1,164:14603697,27775672:179558
x1,164:15198481,27775672
k1,164:15378040,27775672:179559
x1,164:17638644,27775672
k1,164:17818203,27775672:179559
x1,164:18373712,27775672
k1,164:18553271,27775672:179559
x1,164:19425805,27775672
k1,164:19605363,27775672:179558
x1,164:20993424,27775672
x1,164:22116555,27775672
k1,164:22339479,27775672:222924
x1,164:22855006,27775672
k1,164:23034565,27775672:179559
x1,164:23708605,27775672
x1,164:24206191,27775672
k1,164:24385749,27775672:179558
x1,164:26587074,27775672
k1,164:26766672,27775672:179598
x1,164:28174728,27775672
k1,164:28354325,27775672:179597
x1,164:28830569,27775672
k1,164:29010128,27775672:179559
x1,164:29921937,27775672
k1,164:30101496,27775672:179559
x1,164:31212514,27775672
k1,164:31392072,27775672:179558
(1,164:31392072,27775672:1555065,489408,10039
x1,164:32947137,27775672
)
x1,164:33145631,27775672
k1,164:33325267,27775672:179636
x1,164:33761530,27775672
k1,164:33941089,27775672:179559
x1,164:34338077,27775672
k1,164:34338077,27775672:0
)
(1,165:5920357,28666962:28417720,489408,155358
x1,165:6391336,28666962
k1,164:6570372,28666962:179036
x1,164:8531977,28666962
k1,164:8711014,28666962:179037
x1,164:9260381,28666962
k1,164:9439417,28666962:179036
x1,164:10145535,28666962
k1,164:10324572,28666962:179037
x1,164:11226301,28666962
x1,164:12738543,28666962
k1,164:12917579,28666962:179036
x1,164:15506233,28666962
k1,164:15685270,28666962:179037
x1,164:17057987,28666962
k1,164:17237023,28666962:179036
x1,164:19472634,28666962
k1,164:19651671,28666962:179037
x1,164:20612704,28666962
k1,164:20791814,28666962:179110
x1,164:21184412,28666962
k1,164:21363448,28666962:179036
x1,164:21834427,28666962
k1,164:22013464,28666962:179037
x1,164:25072416,28666962
k1,164:25251452,28666962:179036
x1,164:25761271,28666962
x1,164:28261483,28666962
k1,164:28440642,28666962:179159
x1,164:29636832,28666962
k1,164:29815942,28666962:179110
x1,164:30247382,28666962
k1,164:30426419,28666962:179037
x1,164:30819017,28666962
k1,164:30998053,28666962:179036
x1,164:31469032,28666962
k1,164:31648069,28666962:179037
x1,164:33609674,28666962
k1,164:33788710,28666962:179036
x1,164:34338077,28666962
k1,164:34338077,28666962:0
)
(1,165:5920357,29558252:28417720,489408,155358
x1,165:6814813,29558252
k1,164:7009881,29558252:195068
x1,164:8189066,29558252
k1,164:8384134,29558252:195068
x1,164:8709124,29558252
x1,164:11137992,29558252
k1,164:11333061,29558252:195069
x1,164:11942789,29558252
k1,164:12137857,29558252:195068
x1,164:15146225,29558252
k1,164:15341293,29558252:195068
x1,164:16622214,29558252
k1,164:16821198,29558252:198984
x1,164:17228160,29558252
k1,164:17423229,29558252:195069
x1,164:17911439,29558252
k1,164:18106507,29558252:195068
x1,164:19732907,29558252
x1,164:20830853,29558252
k1,164:21025921,29558252:195068
x1,164:21635640,29558252
k1,164:21830708,29558252:195068
x1,164:23558146,29558252
k1,164:23827599,29558252:269453
(1,164:23827599,29558252:1555065,489408,10039
x1,164:25382664,29558252
)
x1,164:25667393,29558252
k1,164:25862461,29558252:195068
x1,164:26756184,29558252
k1,164:26951252,29558252:195068
x1,164:27317237,29558252
x1,164:28241197,29558252
k1,164:28436266,29558252:195069
x1,164:28761256,29558252
x1,164:30816598,29558252
k1,164:31011666,29558252:195068
x1,164:31581132,29558252
k1,164:31776200,29558252:195068
x1,164:34338077,29558252
k1,164:34338077,29558252:0
)
(1,165:5920357,30449542:28417720,489408,155358
x1,165:6692571,30449542
x1,164:7370633,30449542
k1,164:7560666,30449542:190033
x1,164:8617626,30449542
k1,164:8807660,30449542:190034
x1,164:10109096,30449542
k1,164:10299129,30449542:190033
x1,164:13877687,30449542
k1,164:14067721,30449542:190034
x1,164:16283359,30449542
k1,164:16476049,30449542:192690
x1,164:17533009,30449542
k1,164:17723043,30449542:190034
x1,164:18292509,30449542
k1,164:18482542,30449542:190033
x1,164:19376998,30449542
k1,164:19567032,30449542:190034
x1,164:23308076,30449542
k1,164:23498109,30449542:190033
x1,164:23741852,30449542
x1,164:26194773,30449542
k1,164:26449122,30449542:254349
x1,164:27343587,30449542
x1,164:28179116,30449542
x1,164:28527160,30449542
x1,164:29085135,30449542
x1,164:29239429,30449542
k1,164:29432119,30449542:192690
x1,164:30326575,30449542
k1,164:30516609,30449542:190034
x1,164:31736055,30449542
k1,164:31926088,30449542:190033
x1,164:32535816,30449542
k1,164:32725850,30449542:190034
x1,164:33050840,30449542
k1,164:33240873,30449542:190033
x1,164:34338077,30449542
k1,164:34338077,30449542:0
)
(1,165:5920357,31340832:28417720,489408,155358
x1,165:7912750,31340832
x1,164:8260794,31340832
x1,164:8575026,31340832
k1,164:8759531,31340832:184505
x1,164:11199166,31340832
k1,164:11383671,31340832:184505
x1,164:12644112,31340832
x1,164:13246656,31340832
k1,164:13431161,31340832:184505
x1,164:13838123,31340832
k1,164:14022628,31340832:184505
x1,164:14592094,31340832
x1,164:16322446,31340832
k1,164:16506951,31340832:184505
x1,164:17076417,31340832
k1,164:17260922,31340832:184505
x1,164:19781071,31340832
k1,164:19965576,31340832:184505
x1,164:20860032,31340832
k1,164:21044537,31340832:184505
x1,164:23403649,31340832
k1,164:23588154,31340832:184505
x1,164:24197882,31340832
k1,164:24382387,31340832:184505
x1,164:24748372,31340832
x1,164:26519344,31340832
k1,164:26703849,31340832:184505
(1,164:26703849,31340832:1555065,489408,10039
x1,164:28258914,31340832
)
k1,164:28443419,31340832:184505
x1,164:30558055,31340832
k1,164:30742560,31340832:184505
x1,164:31433535,31340832
x1,164:32812617,31340832
k1,164:32997122,31340832:184505
x1,164:34338077,31340832
k1,164:34338077,31340832:0
)
(1,165:5920357,32232122:28417720,489408,155358
x1,165:7408320,32232122
x1,164:7549875,32232122
k1,164:7772091,32232122:222216
x1,164:10024657,32232122
k1,164:10203328,32232122:178671
x1,164:11470443,32232122
k1,164:11649261,32232122:178818
x1,164:12413871,32232122
x1,164:12728182,32232122
k1,164:12906853,32232122:178671
x1,164:14394816,32232122
k1,164:14573487,32232122:178671
x1,164:16382936,32232122
k1,164:16561607,32232122:178671
x1,164:17969198,32232122
x1,164:18927214,32232122
k1,164:19105886,32232122:178672
x1,164:20754592,32232122
k1,164:20933263,32232122:178671
x1,164:23206113,32232122
k1,164:23384931,32232122:178818
x1,164:25999551,32232122
k1,164:26178222,32232122:178671
x1,164:27063032,32232122
k1,164:27241703,32232122:178671
x1,164:29454448,32232122
k1,164:29633119,32232122:178671
x1,164:30759035,32232122
k1,164:30937707,32232122:178672
x1,164:31540860,32232122
k1,164:31719531,32232122:178671
x1,164:32604341,32232122
k1,164:32783012,32232122:178671
(1,164:32783012,32232122:1555065,489408,10039
x1,164:34338077,32232122
)
k1,164:34338077,32232122:0
)
(1,165:5920357,33123412:28417720,489408,155358
x1,165:8231776,33123412
g1,164:8411180,33123412
x1,164:8729798,33123412
x1,164:10193731,33123412
g1,164:10373135,33123412
x1,164:11449562,33123412
x1,164:13504084,33123412
g1,164:13683488,33123412
x1,164:15516988,33123412
g1,164:15696392,33123412
x1,164:16015010,33123412
x1,164:17718616,33123412
x1,164:18059484,33123412
x1,164:18367344,33123412
g1,164:18546748,33123412
x1,164:22652911,33123412
g1,164:22832315,33123412
x1,164:23150933,33123412
x1,164:23491801,33123412
x1,164:26244546,33123412
k1,165:34338077,33123412:8219114
g1,165:34338077,33123412
)
(1,166:5920357,35028326:28417720,494436,146029
(1,166:5920357,35028326:1255831,494436,10043
g1,166:5920357,35028326
x1,166:6817379,35028326
g1,166:7176188,35028326
)
x1,166:8610688,35028326
g1,166:8790092,35028326
x1,166:9308210,35028326
x1,166:13339020,35028326
g1,166:13518424,35028326
x1,166:14036542,35028326
x1,166:15135201,35028326
x1,166:17155279,35028326
g1,166:17334683,35028326
x1,166:19168893,35028326
g1,166:19348297,35028326
x1,166:20106097,35028326
g1,166:20285501,35028326
x1,166:21840565,35028326
x1,166:23616651,35028326
g1,166:23796055,35028326
x1,166:27104230,35028326
k1,166:30721154,35028326:3616924
k1,166:34338077,35028326:3616923
)
(1,168:5920357,36364910:28417720,489408,155358
x1,168:7199539,36364910
k1,167:7449962,36364910:250423
x1,167:8588161,36364910
k1,167:8838584,36364910:250423
x1,167:9448312,36364910
k1,167:9698735,36364910:250423
x1,167:10674448,36364910
k1,167:10924871,36364910:250423
x1,167:12185313,36364910
x1,167:12499545,36364910
x1,167:12854772,36364910
k1,167:13105195,36364910:250423
x1,167:13877409,36364910
x1,167:15043681,36364910
k1,167:15294104,36364910:250423
x1,167:16513551,36364910
k1,167:16763974,36364910:250423
x1,167:20911264,36364910
k1,167:21161688,36364910:250424
x1,167:23195068,36364910
k1,167:23445491,36364910:250423
x1,167:25112170,36364910
k1,167:25362593,36364910:250423
x1,167:26094563,36364910
k1,167:26344986,36364910:250423
x1,167:27726936,36364910
x1,167:29420252,36364910
k1,167:29670675,36364910:250423
x1,167:32943998,36364910
k1,167:33379515,36364910:435517
x1,167:34070492,36364910
x1,167:34338077,36364910
k1,167:34338077,36364910:0
)
(1,168:5920357,37256200:28417720,489408,155358
x1,168:6489090,37256200
x1,167:7365605,37256200
x1,167:8567119,37256200
k1,167:8783094,37256200:215975
x1,167:11221254,37256200
k1,167:11437228,37256200:215974
x1,167:13551113,37256200
k1,167:13767088,37256200:215975
x1,167:14336554,37256200
k1,167:14552528,37256200:215974
x1,167:17032424,37256200
k1,167:17248399,37256200:215975
x1,167:19992526,37256200
k1,167:20324698,37256200:332172
x1,167:21626126,37256200
k1,167:21842100,37256200:215974
x1,167:23711527,37256200
k1,167:23927502,37256200:215975
x1,167:24455982,37256200
x1,167:25058526,37256200
k1,167:25274501,37256200:215975
x1,167:26941180,37256200
k1,167:27157154,37256200:215974
x1,167:27889124,37256200
k1,167:28105099,37256200:215975
x1,167:28999555,37256200
k1,167:29215529,37256200:215974
x1,167:32427370,37256200
k1,167:32643345,37256200:215975
x1,167:34350277,37256200
k1,167:34338077,37256200:0
)
(1,168:5920357,38147490:28417720,489408,155358
x1,168:10501531,38147490
k1,167:10679971,38147490:178440
x1,167:11721388,38147490
k1,167:11899829,38147490:178441
x1,167:13702104,38147490
x1,167:15370307,38147490
k1,167:15548747,38147490:178440
x1,167:19214580,38147490
k1,167:19436719,38147490:222139
x1,167:20037481,38147490
k1,167:20215921,38147490:178440
x1,167:21097223,38147490
k1,167:21275664,38147490:178441
x1,167:21956478,38147490
x1,167:22506811,38147490
k1,167:22685251,38147490:178440
x1,167:24507722,38147490
k1,167:24686355,38147490:178633
x1,167:25527275,38147490
k1,167:25705716,38147490:178441
x1,167:27348597,38147490
x1,167:28430397,38147490
k1,167:28608837,38147490:178440
x1,167:29689906,38147490
x1,167:30032568,38147490
x1,167:30895929,38147490
k1,167:31074370,38147490:178441
x1,167:33077847,38147490
k1,167:33256287,38147490:178440
x1,167:34338077,38147490
k1,167:34338077,38147490:0
)
(1,168:5920357,39038780:28417720,489408,155358
x1,168:6980621,39038780
k1,167:7159383,39038780:178762
x1,167:7866228,39038780
x1,167:8212480,39038780
k1,167:8391241,39038780:178761
x1,167:10904068,39038780
k1,167:11082830,39038780:178762
x1,167:13261317,39038780
k1,167:13483563,39038780:222246
x1,167:14956619,39038780
k1,167:15135509,39038780:178890
x1,167:15999274,39038780
k1,167:16178036,39038780:178762
x1,167:18219389,39038780
k1,167:18398150,39038780:178761
x1,167:19418843,39038780
k1,167:19597605,39038780:178762
x1,167:20147531,39038780
k1,167:20326293,39038780:178762
x1,167:20993559,39038780
x1,167:21332637,39038780
x1,167:21635718,39038780
k1,167:21814479,39038780:178761
x1,167:23149011,39038780
k1,167:23327773,39038780:178762
x1,167:26076704,39038780
k1,167:26255466,39038780:178762
x1,167:27550403,39038780
k1,167:27729164,39038780:178761
$1,167:27729164,39038780
x1,167:29164404,39038780
$1,167:29164404,39038780
x1,167:29341117,39038780
k1,167:29563363,39038780:222246
x1,167:31075307,39038780
k1,167:31254197,39038780:178890
x1,167:32117962,39038780
k1,167:32296724,39038780:178762
x1,167:34338077,39038780
k1,167:34338077,39038780:0
)
(1,168:5920357,39930070:28417720,489408,155358
x1,168:6977317,39930070
k1,167:7192252,39930070:214935
x1,167:7761718,39930070
k1,167:7976652,39930070:214934
x1,167:8667627,39930070
x1,167:9019263,39930070
x1,167:9333495,39930070
k1,167:9548430,39930070:214935
x1,167:10442886,39930070
k1,167:10657820,39930070:214934
x1,167:12893974,39930070
k1,167:13108909,39930070:214935
x1,167:13718637,39930070
k1,167:13933571,39930070:214934
x1,167:16414174,39930070
k1,167:16629109,39930070:214935
x1,167:17686069,39930070
x1,167:18041296,39930070
x1,167:18355528,39930070
k1,167:18570463,39930070:214935
$1,167:18570463,39930070
x1,167:19288083,39930070
$1,167:19288083,39930070
x1,167:19471075,39930070
k1,167:19800126,39930070:329051
x1,167:20532087,39930070
k1,167:20747022,39930070:214935
x1,167:21641478,39930070
k1,167:21856413,39930070:214935
x1,167:23096365,39930070
k1,167:23320182,39930070:223817
$1,167:23320182,39930070
x1,167:24037802,39930070
$1,167:24037802,39930070
k1,167:24252736,39930070:214934
x1,167:26366621,39930070
k1,167:26581556,39930070:214935
x1,167:28003759,39930070
k1,167:28218693,39930070:214934
x1,167:30576329,39930070
k1,167:30791264,39930070:214935
x1,167:31644735,39930070
k1,167:31859669,39930070:214934
x1,167:32184659,39930070
k1,167:32399594,39930070:214935
x1,167:34350277,39930070
k1,167:34338077,39930070:0
)
(1,168:5920357,40821360:28417720,489408,155358
x1,168:8461719,40821360
k1,167:8824943,40821360:363224
x1,167:10126371,40821360
k1,167:10352696,40821360:226325
x1,167:12954808,40821360
k1,167:13181134,40821360:226326
x1,167:13709614,40821360
x1,167:14312158,40821360
k1,167:14538483,40821360:226325
x1,167:15961428,40821360
k1,167:16187753,40821360:226325
x1,167:16919723,40821360
k1,167:17146049,40821360:226326
x1,167:18040505,40821360
k1,167:18266830,40821360:226325
x1,167:18835563,40821360
x1,167:19712078,40821360
x1,167:21035093,40821360
x1,167:21280358,40821360
k1,167:21506684,40821360:226326
x1,167:24475523,40821360
k1,167:24791825,40821360:316302
x1,167:27312707,40821360
k1,167:27539033,40821360:226326
x1,167:27986257,40821360
k1,167:28212582,40821360:226325
x1,167:29107038,40821360
k1,167:29333363,40821360:226325
x1,167:31771523,40821360
k1,167:31997849,40821360:226326
x1,167:33623542,40821360
k1,167:33849867,40821360:226325
x1,167:34338077,40821360
k1,167:34338077,40821360:0
)
(1,168:5920357,41712650:28417720,489408,155358
x1,168:8399349,41712650
k1,167:8579164,41712650:179815
x1,167:8893640,41712650
k1,167:9073455,41712650:179815
x1,167:9781743,41712650
x1,167:10125129,41712650
x1,167:10802817,41712650
k1,167:10982734,41712650:179917
x1,167:13973084,41712650
k1,167:14152899,41712650:179815
x1,167:15175663,41712650
k1,167:15355478,41712650:179815
x1,167:16417185,41712650
x1,167:16753388,41712650
x1,167:17600965,41712650
k1,167:17780780,41712650:179815
x1,167:20553713,41712650
k1,167:20733631,41712650:179918
x1,167:22464675,41712650
k1,167:22644490,41712650:179815
x1,167:23627586,41712650
k1,167:23807401,41712650:179815
x1,167:24476021,41712650
k1,167:24655836,41712650:179815
x1,167:24970312,41712650
x1,167:27201980,41712650
k1,167:27381794,41712650:179814
x1,167:27932836,41712650
k1,167:28112651,41712650:179815
x1,167:28978169,41712650
k1,167:29157984,41712650:179815
x1,167:30376929,41712650
k1,167:30556744,41712650:179815
x1,167:31146745,41712650
k1,167:31326560,41712650:179815
x1,167:32939309,41712650
k1,167:33119124,41712650:179815
x1,167:34338077,41712650
k1,167:34338077,41712650:0
)
(1,168:5920357,42603940:28417720,489408,8247
x1,168:7434521,42603940
g1,167:7613925,42603940
x1,167:10424083,42603940
k1,168:34338076,42603940:24039576
g1,168:34338076,42603940
)
(1,170:5920357,43561613:28417720,489408,155358
h1,169:5920357,43561613:1114112,0,0
x1,169:10043570,43561613
k1,169:10289387,43561613:245817
x1,169:12158814,43561613
k1,169:12404630,43561613:245816
x1,169:13461590,43561613
k1,169:13707407,43561613:245817
x1,169:15902548,43561613
k1,169:16148365,43561613:245817
x1,169:17367812,43561613
k1,169:17613628,43561613:245816
x1,169:21760918,43561613
k1,169:22006735,43561613:245817
x1,169:24324844,43561613
k1,169:24570661,43561613:245817
x1,169:25546365,43561613
k1,169:25792181,43561613:245816
x1,169:28068587,43561613
k1,169:28314404,43561613:245817
x1,169:29005379,43561613
k1,169:29251196,43561613:245817
x1,169:32097793,43561613
k1,169:32343609,43561613:245816
x1,169:33522794,43561613
k1,169:33768611,43561613:245817
x1,169:34338077,43561613
k1,169:34338077,43561613:0
)
(1,170:5920357,44452903:28417720,489408,155358
x1,170:7923120,44452903
k1,169:8102214,44452903:179094
x1,169:9584271,44452903
k1,169:9763365,44452903:179094
x1,169:10564615,44452903
x1,169:10907277,44452903
x1,169:11730246,44452903
k1,169:11909341,44452903:179095
x1,169:15314838,44452903
k1,169:15493932,44452903:179094
x1,169:16535349,44452903
k1,169:16714444,44452903:179095
x1,169:18096258,44452903
k1,169:18318614,44452903:222356
x1,169:21443552,44452903
x1,169:23085722,44452903
k1,169:23264817,44452903:179095
x1,169:24466332,44452903
k1,169:24645426,44452903:179094
x1,169:28731725,44452903
k1,169:28910820,44452903:179095
x1,169:33157958,44452903
k1,169:33337052,44452903:179094
x1,169:34338077,44452903
k1,169:34338077,44452903:0
)
(1,170:5920357,45344193:28417720,489408,155358
x1,170:6597784,45344193
k1,169:6777976,45344193:180192
x1,169:8970285,45344193
k1,169:9150477,45344193:180192
x1,169:10744987,45344193
x1,169:11821405,45344193
k1,169:12001597,45344193:180192
x1,169:13118197,45344193
k1,169:13298390,45344193:180193
x1,169:14015999,45344193
x1,169:14367633,45344193
k1,169:14547825,45344193:180192
x1,169:15983043,45344193
k1,169:16163235,45344193:180192
x1,169:17318580,45344193
x1,169:19241063,45344193
k1,169:19465887,45344193:224824
x1,169:22893205,45344193
k1,169:23073397,45344193:180192
x1,169:24149806,45344193
k1,169:24329998,45344193:180192
x1,169:25286571,45344193
k1,169:25466764,45344193:180193
x1,169:29572201,45344193
k1,169:29752393,45344193:180192
x1,169:31147430,45344193
k1,169:31327622,45344193:180192
x1,169:32204540,45344193
k1,169:32384732,45344193:180192
x1,169:34338077,45344193
k1,169:34338077,45344193:0
)
(1,170:5920357,46235483:28417720,489408,155358
x1,170:7345545,46235483
k1,169:7524379,46235483:178834
x1,169:8078771,46235483
k1,169:8257605,46235483:178834
x1,169:10434543,46235483
k1,169:10613377,46235483:178834
x1,169:12077737,46235483
k1,169:12256571,46235483:178834
x1,169:13879133,46235483
k1,169:14057967,46235483:178834
x1,169:14770561,46235483
k1,169:14949395,46235483:178834
x1,169:16255561,46235483
k1,169:16434395,46235483:178834
x1,169:17146989,46235483
x1,169:18805860,46235483
k1,169:18984694,46235483:178834
x1,169:23060665,46235483
k1,169:23239499,46235483:178834
x1,169:24545673,46235483
k1,169:24724507,46235483:178834
x1,169:25318087,46235483
k1,169:25496921,46235483:178834
x1,169:28683615,46235483
k1,169:28862563,46235483:178948
x1,169:29099854,46235483
x1,169:30219991,46235483
k1,169:30398939,46235483:178948
x1,169:33130261,46235483
k1,169:33309095,46235483:178834
x1,169:34338077,46235483
k1,169:34338077,46235483:0
)
]
(1,170:5920357,48201563:28417720,446948,0
(1,170:5920357,48201563:28417720,446948,0
k1,170:19965377,48201563:14045020
x1,170:20293057,48201563
k1,170:34338077,48201563:14045020
)
)
]
]
]
!41434
}4
!10
{5
[1,187:4736286,48201563:29601791,43465277,9168
[1,187:4736286,4736286:0,0,0
(1,187:4736286,2302362:0,0,0
k1,187:4736286,2302362:-1118290
)
]
[1,187:4736286,48201563:29601791,43465277,9168
h1,187:4736286,4736286:0,0,0
[1,187:5920357,48201563:28417720,45833420,9168
[1,187:5920357,3154575:28417720,786432,0
(1,187:5920357,3154575:28417720,444988,8188
(1,187:5920357,3154575:28417720,444988,8188
k1,187:13171428,3154575:7251071
x1,187:15265284,3154575
x1,187:16743097,3154575
g1,187:16906937,3154575
x1,187:19925480,3154575
g1,187:20089320,3154575
x1,187:21006160,3154575
x1,187:23981443,3154575
g1,187:24145283,3154575
x1,187:25262002,3154575
g1,187:25425842,3154575
x1,187:26907602,3154575
g1,187:27087006,3154575
k1,187:34338077,3154575:7251071
)
)
]
[1,187:5920357,46235483:28417720,40258437,0
(1,170:5920357,6697942:28417720,494436,155358
x1,170:9116680,6697942
k1,169:9339896,6697942:223216
x1,169:11046697,6697942
k1,169:11226353,6697942:179656
x1,169:14283296,6697942
k1,169:14462952,6697942:179656
x1,169:15335648,6697942
k1,169:15515304,6697942:179656
x1,169:16587426,6697942
x1,169:17442905,6697942
k1,169:17622561,6697942:179656
x1,169:18217934,6697942
k1,169:18397590,6697942:179656
x1,169:19195572,6697942
x1,169:22374587,6697942
k1,169:22554243,6697942:179656
x1,169:23869616,6697942
k1,169:24049272,6697942:179656
x1,169:28653459,6697942
k1,169:28876675,6697942:223216
x1,169:29988103,6697942
k1,169:30167759,6697942:179656
x1,169:32152598,6697942
k1,169:32332254,6697942:179656
x1,169:33563039,6697942
k1,169:33742695,6697942:179656
x1,169:34338077,6697942
k1,169:34338077,6697942:0
)
(1,170:5920357,7589232:28417720,494436,155358
x1,170:9303728,7589232
k1,169:9482806,7589232:179078
x1,169:10551697,7589232
x1,169:11404544,7589232
k1,169:11583541,7589232:178997
x1,169:12177121,7589232
k1,169:12356118,7589232:178997
x1,169:13831527,7589232
x1,169:15607613,7589232
k1,169:15786609,7589232:178996
x1,169:17101982,7589232
k1,169:17280979,7589232:178997
x1,169:21884628,7589232
k1,169:22063706,7589232:179078
x1,169:22933773,7589232
k1,169:23112770,7589232:178997
x1,169:25091621,7589232
k1,169:25270617,7589232:178996
x1,169:28516454,7589232
k1,169:28695451,7589232:178997
x1,169:31288557,7589232
k1,169:31467635,7589232:179078
x1,169:33209203,7589232
k1,169:33388200,7589232:178997
x1,169:34338077,7589232
k1,169:34338077,7589232:0
)
(1,170:5920357,8480522:28417720,489408,155358
x1,170:7290115,8480522
x1,169:8968364,8480522
k1,169:9147224,8480522:178860
x1,169:10598212,8480522
k1,169:10777072,8480522:178860
x1,169:12106924,8480522
k1,169:12285783,8480522:178859
x1,169:12890123,8480522
k1,169:13068983,8480522:178860
x1,169:13431739,8480522
x1,169:14807454,8480522
k1,169:14986423,8480522:178969
x1,169:17827494,8480522
k1,169:18006463,8480522:178969
x1,169:18369219,8480522
x1,169:19272505,8480522
k1,169:19451473,8480522:178968
x1,169:19814229,8480522
x1,169:20129177,8480522
x1,169:21932182,8480522
x1,169:22247130,8480522
k1,169:22425990,8480522:178860
x1,169:25206847,8480522
k1,169:25385707,8480522:178860
x1,169:26433342,8480522
k1,169:26612202,8480522:178860
x1,169:28224278,8480522
k1,169:28403137,8480522:178859
x1,169:31183994,8480522
k1,169:31362854,8480522:178860
x1,169:31927295,8480522
k1,169:32106155,8480522:178860
x1,169:34363194,8480522
k1,169:34338077,8480522:0
)
(1,170:5920357,9371812:28417720,489408,155358
x1,170:8949393,9371812
g1,169:9128797,9371812
x1,169:10603480,9371812
g1,169:10782884,9371812
x1,169:12177921,9371812
g1,169:12357325,9371812
x1,169:15367694,9371812
k1,170:34338077,9371812:19095966
g1,170:34338077,9371812
)
(1,173:5920357,10263102:28417720,489408,155358
h1,171:5920357,10263102:1114112,0,0
x1,171:7478624,10263102
k1,171:7658422,10263102:179798
x1,171:8143281,10263102
k1,171:8323079,10263102:179798
x1,171:8847933,10263102
x1,171:10011861,10263102
k1,171:10191659,10263102:179798
x1,171:12615281,10263102
k1,171:12795079,10263102:179798
x1,171:13724111,10263102
k1,171:13903910,10263102:179799
x1,171:14994312,10263102
k1,171:15174110,10263102:179798
x1,171:17233521,10263102
k1,171:17413319,10263102:179798
x1,171:18301637,10263102
k1,171:18481435,10263102:179798
x1,171:21711959,10263102
k1,171:21891757,10263102:179798
x1,171:22497302,10263102
k1,171:22677100,10263102:179798
x1,171:23404048,10263102
x1,171:26590991,10263102
k1,171:26770789,10263102:179798
x1,171:30021649,10263102
k1,171:30201546,10263102:179897
x1,171:31978192,10263102
k1,171:32157990,10263102:179798
x1,171:34338077,10263102
k1,171:34338077,10263102:0
)
(1,173:5920357,11154392:28417720,489408,155358
x1,173:9439840,11154392
k1,171:9618248,11154392:178408
x1,171:11753131,11154392
k1,171:11931538,11154392:178407
x1,171:15964984,11154392
k1,171:16143392,11154392:178408
x1,171:18575837,11154392
k1,171:18754444,11154392:178607
x1,171:19624347,11154392
x1,171:19969528,11154392
k1,171:20147936,11154392:178408
x1,171:22204525,11154392
k1,171:22382932,11154392:178407
x1,171:24398947,11154392
k1,171:24577355,11154392:178408
x1,171:27424829,11154392
k1,171:27603237,11154392:178408
x1,171:28631184,11154392
k1,171:28809592,11154392:178408
x1,171:30786441,11154392
k1,171:30964848,11154392:178407
x1,171:32743820,11154392
x1,171:33605835,11154392
k1,171:33784243,11154392:178408
x1,171:34338077,11154392
k1,171:34338077,11154392:0
)
(1,173:5920357,12045682:28417720,489408,155358
x1,173:7215951,12045682
k1,171:7395735,12045682:179784
x1,171:9258571,12045682
k1,171:9438355,12045682:179784
x1,171:12272339,12045682
k1,171:12452123,12045682:179784
x1,171:13343072,12045682
k1,171:13522856,12045682:179784
x1,171:14251956,12045682
x1,171:17448348,12045682
k1,171:17628132,12045682:179784
x1,171:19935699,12045682
k1,172:20115483,12045682:179784
x1,172:20722820,12045682
k1,172:20902604,12045682:179784
x1,172:22583155,12045682
k1,172:22806754,12045682:223599
x1,172:25074947,12045682
k1,172:25254731,12045682:179784
x1,172:26490533,12045682
k1,172:26670412,12045682:179879
x1,172:28856964,12045682
k1,172:29036748,12045682:179784
x1,172:31872895,12045682
k1,172:32052679,12045682:179784
x1,172:32660016,12045682
k1,172:32839800,12045682:179784
x1,172:34338077,12045682
k1,172:34338077,12045682:0
)
(1,173:5920357,12936972:28417720,489408,155358
x1,173:9135266,12936972
k1,172:9314785,12936972:179519
x1,172:9791507,12936972
k1,172:9971026,12936972:179519
x1,172:11043130,12936972
k1,172:11222650,12936972:179520
x1,172:12096061,12936972
x1,172:12442677,12936972
k1,172:12622196,12936972:179519
x1,172:13494892,12936972
k1,172:13674411,12936972:179519
x1,172:16651312,12936972
k1,172:16830831,12936972:179519
x1,172:18101646,12936972
k1,172:18281165,12936972:179519
x1,172:19630601,12936972
k1,172:19810121,12936972:179520
x1,172:20326158,12936972
k1,172:20505677,12936972:179519
x1,172:21379088,12936972
k1,172:21558607,12936972:179519
x1,172:22233325,12936972
x1,172:24406823,12936972
k1,172:24586342,12936972:179519
x1,172:25181724,12936972
k1,172:25361243,12936972:179519
x1,172:26670649,12936972
k1,172:26850169,12936972:179520
x1,172:29093727,12936972
k1,172:29273275,12936972:179548
x1,172:30305367,12936972
k1,172:30484886,12936972:179519
x1,172:31556990,12936972
x1,172:32333124,12936972
k1,172:32512643,12936972:179519
x1,172:34338077,12936972
k1,172:34338077,12936972:0
)
(1,173:5920357,13828262:28417720,489408,155358
x1,173:7831521,13828262
k1,172:8012778,13828262:181257
x1,172:8907234,13828262
k1,172:9088492,13828262:181258
x1,172:10145435,13828262
k1,172:10326692,13828262:181257
x1,172:10936420,13828262
k1,172:11117678,13828262:181258
x1,172:12012134,13828262
k1,172:12193391,13828262:181257
x1,172:14308019,13828262
k1,172:14489277,13828262:181258
x1,172:16726155,13828262
k1,172:16907412,13828262:181257
x1,172:17598387,13828262
x1,172:17953614,13828262
k1,172:18134871,13828262:181257
x1,172:20126541,13828262
k1,172:20307799,13828262:181258
x1,172:24312342,13828262
k1,172:24540362,13828262:228020
x1,172:25841790,13828262
k1,172:26023048,13828262:181258
x1,172:27283489,13828262
k1,172:27464746,13828262:181257
x1,172:28440459,13828262
x1,172:29690142,13828262
k1,172:29871400,13828262:181258
x1,172:30765856,13828262
k1,172:30947113,13828262:181257
x1,172:34363194,13828262
k1,172:34338077,13828262:0
)
(1,173:5920357,14719552:28417720,489408,155358
x1,173:6761278,14719552
k1,172:6939805,14719552:178527
x1,172:7620619,14719552
k1,172:7799147,14719552:178528
x1,172:10363725,14719552
k1,172:10542252,14719552:178527
x1,172:11103343,14719552
k1,172:11281871,14719552:178528
x1,172:12163173,14719552
k1,172:12341700,14719552:178527
x1,172:14183628,14719552
k1,172:14362155,14719552:178527
x1,172:14923246,14719552
k1,172:15101774,14719552:178528
x1,172:15421985,14719552
k1,172:15600512,14719552:178527
x1,172:17642946,14719552
k1,172:17821474,14719552:178528
x1,172:19905005,14719552
k1,172:20083532,14719552:178527
x1,172:21124949,14719552
k1,172:21303476,14719552:178527
x1,172:22825192,14719552
x1,172:23167854,14719552
x1,172:23477307,14719552
k1,172:23655835,14719552:178528
x1,172:25499197,14719552
x1,172:25841859,14719552
x1,172:26151312,14719552
k1,172:26329839,14719552:178527
x1,172:29735336,14719552
k1,172:29913864,14719552:178528
x1,172:31315877,14719552
k1,172:31494404,14719552:178527
x1,172:34338077,14719552
k1,172:34338077,14719552:0
)
(1,173:5920357,15610842:28417720,489408,155358
x1,173:6595752,15610842
x1,172:8226936,15610842
k1,172:8449164,15610842:222228
x1,172:8846958,15610842
x1,172:9432180,15610842
k1,172:9610887,15610842:178707
x1,172:11081146,15610842
k1,172:11259853,15610842:178707
x1,172:14321273,15610842
k1,172:14499981,15610842:178708
x1,172:15095961,15610842
k1,172:15274668,15610842:178707
x1,172:15990134,15610842
x1,172:19126687,15610842
k1,172:19305394,15610842:178707
x1,172:22702396,15610842
k1,172:22881243,15610842:178847
x1,172:23915071,15610842
k1,172:24093778,15610842:178707
x1,172:25206313,15610842
k1,172:25385021,15610842:178708
x1,172:25981001,15610842
k1,172:26159708,15610842:178707
x1,172:27113421,15610842
k1,172:27292128,15610842:178707
x1,172:28524150,15610842
x1,172:28831054,15610842
x1,172:29178029,15610842
k1,172:29356736,15610842:178707
x1,172:29833938,15610842
k1,172:30012646,15610842:178708
x1,172:31919345,15610842
k1,172:32098052,15610842:178707
x1,172:32654678,15610842
x1,172:33153301,15610842
x1,172:34338077,15610842
k1,172:34338077,15610842:0
)
(1,173:5920357,16502132:28417720,489408,155358
x1,173:6485357,16502132
x1,172:6819774,16502132
x1,172:8180838,16502132
x1,172:9629695,16502132
k1,172:9809919,16502132:180224
x1,172:10697360,16502132
k1,172:10877584,16502132:180224
x1,172:12895017,16502132
k1,172:13075241,16502132:180224
x1,172:14164567,16502132
k1,172:14344791,16502132:180224
x1,172:16160347,16502132
x1,172:16516287,16502132
k1,172:16696511,16502132:180224
x1,172:18067623,16502132
x1,172:19747547,16502132
k1,172:19927771,16502132:180224
x1,172:22993866,16502132
k1,172:23174090,16502132:180224
x1,172:24020869,16502132
k1,172:24201093,16502132:180224
x1,172:25410977,16502132
k1,172:25591201,16502132:180224
x1,172:29705965,16502132
k1,172:29886189,16502132:180224
x1,172:32649471,16502132
k1,172:32874391,16502132:224920
x1,172:34427779,16502132
k1,172:34338077,16502132:0
)
(1,173:5920357,17393422:28417720,489408,155358
x1,173:6518121,17393422
k1,172:6697418,17393422:179297
x1,172:7574336,17393422
k1,172:7753634,17393422:179298
x1,172:9866262,17393422
k1,172:10045559,17393422:179297
x1,172:10643332,17393422
k1,172:10822630,17393422:179298
(1,172:10822630,17393422:0,0,0
(1,172:10822630,16502132:0,0,0
)
)
x1,172:11660085,17393422
x1,172:12529828,17393422
k1,172:12709125,17393422:179297
x1,172:14224007,17393422
k1,172:14403305,17393422:179298
x1,172:15001078,17393422
k1,172:15180375,17393422:179297
x1,172:17332493,17393422
k1,172:17511791,17393422:179298
x1,172:17750755,17393422
(1,172:17750755,17393422:1435938,489408,10039
x1,172:19186693,17393422
)
x1,172:19425657,17393422
k1,172:19604954,17393422:179297
x1,172:20083591,17393422
k1,172:20262889,17393422:179298
x1,172:20821189,17393422
k1,172:21000486,17393422:179297
x1,172:23272449,17393422
k1,172:23451747,17393422:179298
x1,172:23770365,17393422
k1,172:23949662,17393422:179297
x1,172:25304516,17393422
x1,172:26964349,17393422
k1,172:27143647,17393422:179298
x1,172:29455775,17393422
k1,172:29635072,17393422:179297
x1,172:30193372,17393422
k1,172:30372670,17393422:179298
x1,172:32365470,17393422
k1,172:32544767,17393422:179297
x1,172:34338077,17393422
k1,172:34338077,17393422:0
)
(1,173:5920357,18284712:28417720,489408,155358
x1,173:6489823,18284712
k1,172:6717427,18284712:227604
x1,172:8303592,18284712
k1,172:8531196,18284712:227604
x1,172:10197884,18284712
x1,172:10443149,18284712
k1,172:10670753,18284712:227604
x1,172:12337423,18284712
k1,172:12565027,18284712:227604
x1,172:14292456,18284712
k1,172:14532110,18284712:239654
x1,172:15426566,18284712
k1,172:15654170,18284712:227604
x1,172:18988978,18284712
k1,172:19216582,18284712:227604
x1,172:20843008,18284712
k1,172:21070612,18284712:227604
x1,172:21965068,18284712
k1,172:22192672,18284712:227604
x1,172:22924642,18284712
x1,172:26133631,18284712
k1,172:26361235,18284712:227604
x1,172:30508525,18284712
k1,172:30736129,18284712:227604
x1,172:33216750,18284712
k1,172:33444354,18284712:227604
x1,172:34338077,18284712
k1,172:34338077,18284712:0
)
(1,173:5920357,19176002:28417720,489408,8247
x1,173:8670239,19176002
g1,172:8849643,19176002
x1,172:10244680,19176002
g1,172:10424084,19176002
x1,172:12376703,19176002
g1,172:12556107,19176002
x1,172:15964038,19176002
k1,173:34338077,19176002:18499622
g1,173:34338077,19176002
)
(1,176:5920357,20067292:28417720,489408,155358
h1,174:5920357,20067292:1114112,0,0
x1,174:7634633,20067292
k1,174:7813469,20067292:178836
x1,174:10594507,20067292
k1,174:10773457,20067292:178950
x1,174:12174786,20067292
k1,174:12353622,20067292:178836
x1,174:12953786,20067292
k1,174:13132622,20067292:178836
x1,174:14013047,20067292
k1,174:14191883,20067292:178836
x1,174:14712073,20067292
x1,174:15945569,20067292
k1,174:16124405,20067292:178836
x1,174:16844893,20067292
k1,174:17023729,20067292:178836
x1,174:18384001,20067292
x1,174:20050530,20067292
k1,174:20229366,20067292:178836
x1,174:21429685,20067292
k1,174:21608521,20067292:178836
x1,174:25690754,20067292
k1,174:25869590,20067292:178836
x1,174:27871081,20067292
k1,174:28049917,20067292:178836
x1,174:29610480,20067292
k1,175:29789316,20067292:178836
x1,175:30509804,20067292
k1,175:30688640,20067292:178836
x1,175:31048884,20067292
x1,175:31958182,20067292
k1,175:32137018,20067292:178836
x1,175:33617598,20067292
x1,175:34338077,20067292
k1,175:34338077,20067292:0
)
(1,176:5920357,20958582:28417720,489408,155358
x1,176:8670948,20958582
g1,175:8850352,20958582
x1,175:10503720,20958582
g1,175:10726180,20958582
x1,175:11125171,20958582
x1,175:11712186,20958582
g1,175:11891590,20958582
x1,175:12210208,20958582
x1,175:14491499,20958582
k1,176:34338077,20958582:19936280
g1,176:34338077,20958582
)
(1,178:5920357,23012820:28417720,541848,160032
(1,178:5920357,23012820:668472,541848,11006
g1,178:5920357,23012820
x1,178:6510181,23012820
g1,178:6588829,23012820
)
g1,178:6785437,23012820
x1,178:7353238,23012820
g1,178:7549846,23012820
x1,178:10346353,23012820
g1,178:10542961,23012820
x1,178:11460721,23012820
x1,178:12020659,23012820
g1,178:12217267,23012820
x1,178:13746853,23012820
g1,178:13943461,23012820
x1,178:14511262,23012820
x1,178:15715274,23012820
x1,178:17273977,23012820
k1,178:25806027,23012820:8532050
k1,178:34338077,23012820:8532050
)
(1,186:5920357,24377767:28417720,489408,155358
x1,186:6759632,24377767
k1,180:6948450,24377767:188818
x1,180:7842906,24377767
k1,180:8031725,24377767:188819
x1,180:9658125,24377767
x1,180:11854008,24377767
k1,180:12042826,24377767:188818
x1,180:14420969,24377767
k1,180:14612141,24377767:191172
x1,180:14937131,24377767
k1,180:15125949,24377767:188818
x1,180:18135050,24377767
k1,180:18323868,24377767:188818
x1,180:19543314,24377767
k1,180:19732132,24377767:188818
x1,180:21806515,24377767
k1,180:21995334,24377767:188819
x1,180:23052294,24377767
k1,180:23241112,24377767:188818
x1,180:25720999,24377767
k1,181:25909817,24377767:188818
x1,181:28308457,24377767
k1,181:28497275,24377767:188818
x1,181:29636207,24377767
k1,181:29825026,24377767:188819
x1,181:31979923,24377767
k1,181:32168741,24377767:188818
x1,181:34363911,24377767
k1,181:34338077,24377767:0
)
(1,186:5920357,25269057:28417720,489408,155358
x1,186:6423003,25269057
x1,181:7025547,25269057
k1,181:7233568,25269057:208021
x1,181:8575257,25269057
k1,181:8783279,25269057:208022
x1,181:9352745,25269057
k1,181:9560766,25269057:208021
x1,181:11105212,25269057
k1,181:11313233,25269057:208021
x1,181:11882699,25269057
k1,181:12090721,25269057:208022
x1,181:14529614,25269057
k1,182:14737635,25269057:208021
x1,182:15632091,25269057
k1,182:15840112,25269057:208021
x1,182:19823451,25269057
k1,182:20031473,25269057:208022
x1,182:20641201,25269057
k1,182:20849222,25269057:208021
x1,182:21743678,25269057
k1,182:21951699,25269057:208021
x1,182:23578099,25269057
x1,182:25021524,25269057
k1,182:25329836,25269057:308312
x1,182:27525006,25269057
k1,182:27732999,25269057:207993
x1,182:28221209,25269057
k1,182:28429230,25269057:208021
x1,182:29486190,25269057
k1,182:29694211,25269057:208021
x1,182:30588667,25269057
k1,182:30796689,25269057:208022
x1,182:32219634,25269057
k1,183:32427655,25269057:208021
x1,183:34338077,25269057
k1,183:34338077,25269057:0
)
(1,186:5920357,26160347:28417720,489408,155358
x1,186:8908810,26160347
k1,183:9088819,26160347:180009
x1,183:10502710,26160347
k1,183:10682719,26160347:180009
x1,183:11773121,26160347
k1,183:11953130,26160347:180009
x1,183:12437989,26160347
k1,183:12617999,26160347:180010
x1,183:13950482,26160347
k1,183:14130491,26160347:180009
x1,183:16109221,26160347
k1,183:16289230,26160347:180009
x1,183:16854788,26160347
k1,183:17034797,26160347:180009
x1,183:18610078,26160347
k1,183:18790087,26160347:180009
x1,183:20041879,26160347
k1,184:18790087,26160347:-10758
x1,184:20394595,26160347
k1,184:20574604,26160347:180009
x1,184:21664279,26160347
k1,184:21844288,26160347:180009
x1,184:22369142,26160347
x1,184:23533070,26160347
k1,184:23713079,26160347:180009
x1,184:26418749,26160347
k1,184:26598759,26160347:180010
x1,184:27931242,26160347
k1,184:28111251,26160347:180009
x1,184:28716786,26160347
k1,184:28896795,26160347:180009
x1,184:31723848,26160347
k1,184:31903857,26160347:180009
x1,184:34427779,26160347
k1,184:34338077,26160347:0
)
(1,186:5920357,27051637:28417720,489408,155358
x1,186:9109412,27051637
g1,185:9288816,27051637
x1,185:12098974,27051637
g1,185:12278378,27051637
x1,185:13793251,27051637
g1,185:13972655,27051637
x1,185:16424723,27051637
g1,185:16604127,27051637
x1,185:17640363,27051637
g1,185:17819767,27051637
x1,185:19333931,27051637
g1,185:19513335,27051637
x1,185:22323493,27051637
x1,185:22591881,27051637
k1,186:34338077,27051637:11873932
g1,186:34338077,27051637
)
]
(1,187:5920357,48201563:28417720,446948,9168
(1,187:5920357,48201563:28417720,446948,9168
k1,187:19965377,48201563:14045020
x1,187:20293057,48201563
k1,187:34338077,48201563:14045020
)
)
]
]
]
!19052
}5
Input:128:C:\Users\ni484792\Desktop\RBC\RBC-Niloo-Litreview\Online-To-Batch.aux
!90
Postamble:
Count:3346
!26
Post scriptum:

